Conjunctive Queries with Negation and Aggregation: A Linear Time Characterization

In this paper, we study the complexity of evaluating Conjunctive Queries with negation (\cqneg). First, we present an algorithm with linear preprocessing time and constant delay enumeration for a class of CQs with negation called free-connex signed-acyclic queries. We show that no other queries admit such an algorithm subject to lower bound conjectures. Second, we extend our algorithm to Conjunctive Queries with negation and aggregation over a general semiring, which we call Functional Aggregate Queries with negation (\faqneg). Such an algorithm achieves constant delay enumeration for the same class of queries, but with a slightly increased preprocessing time which includes an inverse Ackermann function. We show that this surprising appearance of the Ackermmann function is probably unavoidable for general semirings, but can be removed when the semiring has specific structure. Finally, we show an application of our results to computing the difference of CQs.

==> aggregation-colored.tex <==
\newpage
\section{Enumeration Algorithms for $\nestfaqneg$} \label{sec:preprocessing}

\myparagraph{Context-free Grammar ($\CFG$)}
If $u, v, w$ are strings of terminals and non-terminals, and $\nonterm ::= w$ is a rule of the $\CFG$, we say that $u \nonterm v$ \emph{yields} $uwv$ in the $\CFG$ (written as $u \nonterm v \yield uwv$). We say that $u$ \emph{derives} $v$ (written as $u \derive v$) in the $\CFG$ if $u = v$ or if there is a sequence $u_1, \dots, u_k$ for $k \geq 0$ such that 
$$ u \yield u_1 \yield u_2 \yield \cdots \yield u_k \yield v.
$$
A \emph{derivation} of a string for a grammar is a sequence of grammar rule applications that transform the start symbol into the string. A derivation proves that the string belongs to the grammar's language.

\medskip

\myparagraph{$\nestfaqneg$ Grammar \& Expression} 
We formally introduce \textit{nested functional aggregate queries with negation} ($\nestfaqneg$) over a single semiring $\bS = (\boldsymbol{D}, \oplus, \otimes, \mathbf{0}, \mathbf{1})$. As motivated in Section~\ref{sec:enum-faqneg}, $\nestfaqneg$ is a generalization of $\faqneg$ that is essential for our enumeration algorithms. 

For any $i \in [n]$, let $x_i$ denote a variable, and $a_i$ denote a value in the discrete domain $\dom(x_i)$ of the variable $x_i$. 
Overloading notation, we also refer to $[n]$ as the set of variables. 
For any subset $K \subseteq [n]$, we define $\bx_K = (x_i)_{i \in K}$ and $\ba_K = (a_i)_{i \in K} \in \prod_{i \in K} \dom(\bx_K)$, where $\dom(\bx_K) = \prod_{i \in K} \dom(x_i)$. In other words, $\bx_K$ is a tuple of variables, and $\ba_K$ is a tuple of specific values with support $K$.

% \highlight{Btw, we should define a signed hypergraph to have no $\emptyset$ hyperedge.}

\smallskip
Let $\mH = ([n], \mE^+, \mE^-)$ be a signed hypergraph. To each $K\in \mE^+$ (and $K \in \mE^-$), we associate a distinct function $R_K: \dom(\bx_K) \rightarrow \boldsymbol{D}$, called a \emph{factor}. We assume that all factors are represented via the \textit{listing representation}: each factor $R_K$ is a table of all tuples of the form $\langle \ba_K, R_K(\ba_K) \rangle$, where $R_K(\ba_K) \in \boldsymbol{D}$ is the \emph{weight} of the tuple $\ba_K$. For entries not in the table, the factor implicitly encodes their weights as $\zerobf$. Under set-theoretic context, we also use $R_K$ to denote the set of tuples of schema $\bx_K$ explicitly stored in the factor table and $\neg R_K = \dom (\bx_K) \setminus R_K$. Our definition of listing representation is slightly more general than \cite{ DBLP:conf/pods/KhamisNR16, FAQ-AI} in that we allow $R_K(\bx_K) = \mathbf{0}$ for some $\bx_K$ in the table (i.e. $\bx_K \in R_K$). A factor $R_K$ where $K \in \mE^+$ (resp. $R_N$ where $N \in \mE^-$) is called a \emph{positive} (resp. \emph{negative}) \emph{factor}. 

Over a single semiring $\bS = (\boldsymbol{D}, \oplus, \otimes, \mathbf{0}, \mathbf{1})$, a $\nestfaqneg$ expression $\formula(\bx_{[n]})$ associated with $\mH = ([n], \mE^+, \mE^-)$ is a string recognized by the following context-free grammar ($\CFG$):

\begin{equation}\label{def:cfg}
    \begin{aligned}
        \framebox{\CFG} \qquad \qquad \quad \; \\
        \text{ for all } S \subseteq [n], \\
        \nonterm(\bx_{\emptyset}) &::= \; e 
        && \text{ where } S = \emptyset \text{ and } e \in \boldsymbol{D} \setminus \{\zerobf\} \\
        \nonterm(\bx_{S}) &::= \; R_K(\bx_K) \otimes \nonterm(\bx_{S^-})
        && \text{ where } S = K \cup S^-, K \in \mE^+ \text{ and } S^- \subseteq S  \\
        & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-})
        && \text{ where } S = N \cup S^-, N^- \subseteq N \in \mE^- \text{ and } S^- \subseteq S
    \end{aligned}
\end{equation}

where
\begin{itemize}
    \item (terminals) $e, R_K(\bx_K)$ and $R_N(\bx_N)$, where $e \in \boldsymbol{D} \setminus \{\zerobf\}, K \in \mE^+$ and $N \in \mE^-$, the semiring operators $\otimes$ and $\vdash$, and the parenthesis are terminals of the $\CFG$. On its semantics, $R_N(\bx_N) \vdash \nonterm(\bx_{N^-})$ is a shorthand for $R_N(\bx_N) \oplus (\indicator{\neg R_N}(\bx_N) \otimes \nonterm(\bx_{N^-}))$, where $N^- \subseteq N$ and
    $\indicator{R_N}$ is an indicator factor defined as the following (also defined in \cite{FAQ-AI}):
    $$
    \indicator{R_N}(\bx_N)= 
    \begin{cases} \onebf & \text { if } \bx_K \in R_K \\ \zerobf & \text { otherwise. } \end{cases}
    $$
    Here, $\vdash$ is the non-commutative operator that takes a negative factor as its left operand and a $\nestfaqneg$ subexpression as its right operand.
    \item (non-terminals) $\nonterm(\bx_{S})$, where $S \subseteq [n]$, are the non-terminals of the $\CFG$, and in particular ($S = [n]$), $\nonterm(\bx_{[n]})$ is the start symbol of the $\CFG$. {A $\nestfaqneg$ subexpression is a string $\formula(\bx_S)$ derived from the $\nonterm(\bx_S)$ non-terminal, following a sequence of grammar rule applications of $\CFG$ as defined in \eqref{def:cfg}.}
    \item (size measure) the \emph{size} of a $\nestfaqneg$ subexpression $\formula(\bx_{[n]})$ is defined as $|\formula| = \sum_{i \in [n]} d(i)$, where $d(i)$ is the number of hyperedges in $\mH$ that contain $i$;
    %%%%%%%%%%%%%%%% the size of subexpression - could be redundant %%%%%%%%%%%%%%%%%%%%
    % the \emph{size} of a $\nestfaqneg$ subexpression $\formula(\bx_{S})$ in $\formula(\bx_{[n]})$, where $S\subseteq [n]$ is defined as $|\formula(\bx_S)| = \sum_{i \in S} d(i)$, where $d(i)$ is the number of factors (or hyperedges) in $\formula(\bx_{S})$ that contain $i$.
    \item (our assumptions) in our work, we assume that each factor $R_K, R_N$, where $K \in \mE^+, N \in \mE^-$, shows up precisely once in $\formula(\bx_{[n]})$, i.e., a one-to-one mapping from the hyperedges of $\mH$ to factors in $\formula(\bx_{[n]})$. Moreover, we assume that a $\nestfaqneg$ expression $\formula(\bx_{[n]})$ is {\em safe}, that is, every $i \in [n]$ appears in some $K \in \mE^+$ (i.e. $\bigcup_{{K \in \mE^+} } K = [n]$). \highlight{Indeed, the ``unsafest'' case occurs when every branch takes the right child of $\vdash$ operator (thus more propensity to have un-guarded variables), because if takes the left child $R_N$, then the right sub-tree is immediately guarded by $R_N$; otherwise, the $\neg R_N$ can possibly be un-guarded.} Another assumption is that for constant factors, we assume $e \in \boldsymbol{D} \setminus \{\zerobf\}$. 
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%% some comments %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \highlight{Indeed, the ``unsafest'' case occurs when every branch takes the right child of $\vdash$ operator (thus more propensity to have un-guarded variables), because if takes the left child $R_N$, then the right sub-tree is immediately guarded by $R_N$; otherwise, the $\neg R_N$ can possibly be un-guarded. After aggregation out $x_n$, the syntax is preserved as $\CFG_n$ and only the hyperedges are changed. The removed positive factors are never guards, but the pivot factor is.} Another assumption is that for constant factors, we assume $e \in \boldsymbol{D} \setminus \{\zerobf\}$. 


A $\nestfaqneg$ expression $\formula(\bx_{[n]})$ can be depicted pictorially as a \emph{abstract syntax tree} ($\AST$) drawn below, where
\begin{figure}[h]
    \centering
    \begin{tikzpicture} 
        \centering
        %% root is \bigotimes, 2nd level are \bigooplus nodes, 3rd level are \bigotimes nodes, 4th level are relation nodes
        %% root at the center
        \node (root) at (0, 0) {$\bigotimes$}; %% root node
    
        %% 2nd level
        %% draw \bigoplus operation nodes from the right of RN onwards, one for each negative factor (4 of them)
        \node[draw,circle,inner sep=1.5pt] (oplus0) at (-6, -1) {$\vdash$};
        \node[draw,circle,inner sep=1.5pt] (oplus1) at (-2.5, -1) {$\vdash$};
    
        \node[draw,circle,inner sep=1.5pt] (oplus3) at (1.25, -1) {$\vdash$};

        %%% add a node for positive factor
        \node (e) at (3, -1.25) {$e$};
        \node (rk1) at (5, -1.25) {$R_{K_1}$};
        \node (rkt) at (7, -1.25) {$R_{K_t}$};

        %% draw ... between oplus0 and oplus1 to indicate that there are more negative factors in between
        \node (dots1) at (-0.5, -1.15) {$\cdots$};
        \node (dots2) at (6, -1.25) {$\cdots$};
    
        %% 3rd level are \bigotimes nodes, each oplus node has two \bigotimes nodes as children
        %% draw \bigotimes nodes for oplus0 (put oplus0 at the center of its children)
        \node (otimes00) at (-7, -2) {$R_{N_k}$};
        \node (otimes01) at (-5, -2) {$\bigotimes$}; %% e is any element in \boldsymbol{D}
    
        %% draw \bigotimes nodes for oplus1 
        \node (otimes10) at (-3.5, -2) {$R_{N_{k-1}}$};
        \node (otimes11) at (-1.5, -2) {$\bigotimes$};

        %% draw \bigotimes nodes for oplus2 
        \node (otimes20) at (0.25, -2) {$R_{N_{1}}$};
        \node (otimes21) at (2.25, -2) {$\bigotimes$};

        %% 4th level are subproblems for each otimes on the upper level, draw a subtree for the 2nd otime
        %% add a ... node for otimes11 (directly below)
        \node (dots2) at (-1.5, -4) {$\cdots$};

        %% draw a subtree for otimes11
        \node (dots2) at (-5, -4) {$\cdots$};

        %% draw a subtree for otimes21
        \node (dots3) at (2.25, -4) {$\cdots$};
    
        %% draw all the edges
        \draw (root) -- (oplus0);
        \draw (root) -- (oplus1);
        \draw (root) -- (oplus3);

        \draw (oplus0) -- (otimes00);
        \draw (oplus0) -- (otimes01);

        \draw (oplus1) -- (otimes10);
        \draw (oplus1) -- (otimes11);

        \draw (oplus3) -- (otimes20);
        \draw (oplus3) -- (otimes21);

        %% draw two edges from otimes11 to the left and right of dots2 using dashed lines
        \draw[dashed] (otimes11) -- (-2.25, -4);
        \draw[dashed] (otimes11) -- (-0.75, -4);
        
        %% draw two edges from otimes21 to the left and right of dots3 using dashed lines
        \draw[dashed] (otimes21) -- (1.5, -4);
        \draw[dashed] (otimes21) -- (3, -4);

        %% draw two edges from otimes01 to the left and right of dots3 using dashed lines
        \draw[dashed] (otimes01) -- (-5.75, -4);
        \draw[dashed] (otimes01) -- (-4.25, -4);

        %% draw edges from root to e, rk1 and rkt
        \draw (root) -- (e);
        \draw (root) -- (rk1);
        \draw (root) -- (rkt);

        %% draw an underbrace to indicate that the negative factors are from $\mM(\mE^-)$ from the left of R0 to the right of R3 and immediately below the 4th level
        % \draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
        % (-1.3, -3.2) -- (4.1, -3.2) node [black,midway,yshift=-0.8cm] {\footnotesize $\mM(\mE^-)$};
    \end{tikzpicture}
    %% add a caption
    \caption{The $\AST$ for a general $\nestfaqneg$ expression $\formula(\bx_{[n]})$ recognized by the $\CFG$ in \eqref{def:cfg}.}
\end{figure}

\begin{itemize}
    \item $\bigotimes$ and $\vdash$ are the intermediate nodes, and they are show up on alternating levels, starting from the root being a $\bigotimes$ node. The $\bigotimes$ node takes at least one child, but the  $\vdash$ node always takes two children. 
    \item $e, R_K(\bx_K)$ and $R_N(\bx_N)$, where $e \in \boldsymbol{D} \setminus \{\zerobf\}, K \in \mE^+$ and $N \in \mE^-$, are the leaves of the $\AST$.
\end{itemize}

\myparagraph{The $\nestfaqneg$ Queries.} 
A $\nestfaqneg$ query $\varphi$ (with free variables $F \subseteq [n]$) associated with a signed hypergraph $\mH = ([n], \mE^+, \mE^-)$ is defined as:
\begin{align}\label{def:nestfaqneg}
    \varphi(\bx_F) = \bigoplus_{\bx_{[n] \setminus F} \in \dom(\bx_{[n] \setminus F})} \; \formula(\bx_{[n]})
\end{align}
where
\begin{itemize}
    \item $\formula(\bx_{[n]})$ is a safe $\nestfaqneg$ expression recognized by the $\CFG$ in \eqref{def:cfg}. Sometimes we call $\formula(\bx_{[n]})$ a \emph{full} $\nestfaqneg$ query (i.e. $F = [n]$).
    \item $F = [f]\subseteq [n]$ is the set of \emph{free variables} for some integer $0 \leq f \leq n$.
    % Variables in $[n]\setminus F$ are called \emph{bound variables}.
    %%%%%%%% safe faqneg
    % \item We assume that a $\nestfaqneg$ is {\em safe}, that is, every variable of $\varphi$ appears in at least one positive factor ($\bigcup_{{K \in \dedup{\mE^+}} } K = [n]$). Moreover, we assume that factors associated with every hyperedge in multi-sets $\mE^+$ and $\mE^-$ show up exactly once in the body of $\varphi$.
    \item (query input and output) The input to a $\nestfaqneg$ query $\varphi$ is a database instance $\db$ that contains the constants $e \in \boldsymbol{D} \setminus \{\zerobf\}$ and a list representation for every factor in $\formula(\bx_{[n]})$. {The size of a database instance $|\db|$ is defined as the total number of rows to store the constants and the list representations.} An {\em answer} (or {\em output}) of $\varphi$ is a tuple $\langle \ba_F, \varphi(\ba_F)\rangle \in \dom(\bx_F)$ such that $\ba_F \in \dom(\bx_F)$ and $\varphi(\ba_F) \neq \zerobf$. The set of all answers of $\varphi$ is denoted by $\varphi(\db)$. 
    \item (complexity measure) {In this work, we measure the combined (and data) complexity of evaluating a $\nestfaqneg$ query $\varphi$ on a database instance $\db$ by the query size $|\varphi| = |\formula| = \sum_{i \in [n]} d(i)$ and the database size $|\db|$.} 
\end{itemize}

% \highlight{If $K = \emptyset$, then we simply use $e$ to denote the factor $R_{\emptyset}$ (also its single-row list representation) that always maps to the constant $e \in \boldsymbol{D}$.} 
A fragement of $\nestfaqneg$ queries is the $\faqneg$ queries, where the corresponding $\AST$ is flat: the right child of the $\vdash$ nodes are $\bc_N \neq \zerobf$, that is, the default values of $R_N$. Indeed, the query can be compactly written as 
\begin{align*}
    \varphi(\bx_F) = \bigoplus_{\bx_{[n] \setminus F} \in \dom(\bx_{[n] \setminus F})} \; \bigotimes_{K \in \mE^+} R_K(\bx_K) \otimes \bigotimes_{N \in \mE^-} ( R_N(\bx_N) \vdash \bc_N ) 
\end{align*}
that coincides with the definition of $\faqneg$ queries in \eqref{def:faqneg} by letting $\overline{R}_N(\bx_N) = ( R_N(\bx_N) \vdash \bc_N )$. 

% A speical case of $\nestfaqneg$ queries is the \emph{conjunctive queries with negation} ($\cqneg$) over the Boolean semiring, where the input is
% \begin{itemize}
%     \item the constant $e = \mathsf{true}$, and
%     \item a list representation for every factor in $\formula(\bx_{[n]})$, where $R_K(\ba_K) = \mathsf{true}$ for any $\ba_K \in R_K$ and $R_N(\ba_N) = \mathsf{false}$ for any $\ba_N \in R_N$.
% \end{itemize}
% After simplifying the $\nestfaqneg$ expression, we degenerate into a $\cqneg$ query $Q$: % $R_K(\bx_K) = \textsf{true}$ for all $\bx_K \in R_K$ and $R_N(\bx_N) = \textsf{false}$ for all $\bx_N \in R_N$. 
% \begin{align}\label{def:nestfaqneg-boolean}
%     Q(\bx_F) = \bigvee_{\bx_{[n] \setminus F} \in \dom(\bx_{[n] \setminus F})} \; \bigwedge_{K \in \mE^+} R_K(\bx_K) \wedge \bigwedge_{N \in \mE^-} \neg R_N(\bx_N),
% \end{align}
% where $R_K, R_N$ now represent input relations. A $\cqneg$ \eqref{def:nestfaqneg-boolean} is also called the signed conjunctive queries, as coined in \cite{BBThesis, DBLP:journals/sigmod/Segoufin15}. 

\begin{definition}[Free-connex $\pn$-acyclicity]
\label{defn:free-connex-pn-acyclic}
A $\nestfaqneg$ query $\varphi$ \eqref{def:nestfaqneg} is \emph{free-connex $\pn$-acyclic} if the signed hypergraph $\mH = ([n], \mE^+, \mE^- \cup \{F\})$ is $\pn$-acyclic. 
%In other words, $\varphi$ is free-connex $\pn$-acyclic if the signed hypergraph $\mH' = ([n], \mE^+ \cup \mE')$ is $\alpha$-acyclic for every multi-set $\mE' \subseteq \mE^- \cup \{F\}$.
\end{definition}

In the following sections, we will show the following main theorem for free-connex $\pn$-acyclic $\nestfaqneg$ queries, which subsumes Theorem~\ref{conj:main-upper} as a special case.

\begin{theorem}\label{thm:faqneg-main}
    Let $\varphi$ be a free-connex $\pn$-acyclic $\nestfaqneg$ query with free variables $F$ over a commutative semiring $\bS$. Then, there is an algorithm that can enumerate the answers of $\varphi$ in $O(|\varphi|)$ delay, after a $O(|\varphi|^3 + |\varphi| \cdot |\db| \cdot \alpha(14 \cdot |\db|, |\db|))$ preprocessing time. 
\end{theorem}

Before jumping to the general case of free-connex $\pn$-acyclicity, we dedicate the next section to a special case, where $\varphi$ is a \emph{full} $\pn$-acyclic $\nestfaqneg$ query, i.e. $F = [n]$.


\subsection{Enumeration of full $\nestfaqneg$} \label{sec:enum-full-faqneg}

In this section, we study the enumeration problem $\Enum(\varphi, \db)$ for $\pn$-acyclic \emph{full} $\nestfaqneg$ queries. First, we recall the definition \eqref{def:nestfaqneg} and \eqref{def:cfg} that: a $\nestfaqneg$ query associated with a signed hypergraph $\mH = ([n], \mE^+, \mE^-)$ is full if $F = [n]$, that is, $\varphi(\bx_{[n]}) = \formula(\bx_{[n]})$, where $\formula(\bx_{[n]})$ is a safe $\nestfaqneg$ expression associated with $\mH$. The enumeration algorithm can be summarized as follows. 
\begin{enumerate}
    \item (pre-processing phase) we first reduce the $\Enum(\varphi, \db)$ problem into a $\Enum(Q^*, \db^*)$ problem, where $Q^*$ is a $\pn$-acyclic \emph{full} $\cqneg$ query that evaluates on a new database instance $\db^*$; then, we follow the pre-processing algorithm for $\pn$-acyclic \emph{full} $\cqneg$ queries presented in Section~\ref{sec:enumeration-full}.
    \item (enumeration phase) we enumerate the output tuples of $Q^*$ via the enumeration algorithm for $\pn$-acyclic \emph{full} $\cqneg$ queries presented in Section~\ref{sec:enumeration-full}; then we plug the tuples into $\varphi$ to get its corresponding weight.
\end{enumerate}

Now we present the construction of $Q^*$ and $\db^*$. First, the desired $Q^*$ is the following full $\cqneg$ query associated with $\mH$:
\begin{align} \label{eq:q-for-full-faqneg}
    Q^*(\bx_{[n]}) &= \bigwedge_{K \in \mE^+} R^*_K(\bx_{K}) \wedge \bigwedge_{N \in \mE^-} \neg R^*_N(\bx_{N}),
\end{align}
where for every $K \in \mE^+$, we add a positive atom $R^*_K(\bx_{K})$, and for every $N \in \mE^-$, we add a negative atom $R^*_N(\bx_{N})$ (and place a $\neg$ symbol in front) into the body of $Q^*$. It is easy to see that \eqref{eq:q-for-full-faqneg} is a full $\pn$-acyclic \emph{full} $\cqneg$ query associated with $\mH$. Next, we construct the corresponding database instance $\db^*$ for every atom in $Q^*$ defined as follows: 
\begin{equation}\label{eq:db-for-full-faqneg}
    \begin{aligned} 
        R^*_K &= \{\ba_K \in R_K \mid R_K(\ba_K) \neq \zerobf\},  && \text{ for every } K \in \mE^+, \\
        R^*_N &= \{\ba_N \in R_N \mid R_N(\ba_N) = \zerobf\}, && \text{ for every } N \in \mE^-.
    \end{aligned}
\end{equation}
Thus, $\db^*$ is of size $O(|\db|)$ and can be constructed in $O(|\db|)$ time by scanning over the list representation of every factor in $\db$. We reason about the such a construction of $\Enum(Q^*, \db^*)$ through the following theorem:

\begin{theorem}
\label{thm:enum-full-faqneg}
Let $\varphi$ be a $\pn$-acyclic full $\nestfaqneg$ query associated with a signed hypergraph $\mH = ([n], \mE^+, \mE^-)$ over a commutative semiring $\bS$, and $\db$ be a corresponding database instance. Then, a tuple $\ba_{[n]}$ is an answer of $\varphi$ (i.e. $\varphi(\ba_{[n]}) \neq \zerobf$) if and only if $\ba_{[n]}$ is an answer of $Q^*(\db^*)$ (i.e. $\ba_{[n]} \in Q^*(\db^*)$, or $Q^*(\ba_{[n]}) = \mathsf{true}$), where $Q^*$ and $\db^*$ are defined in \eqref{eq:q-for-full-faqneg} and \eqref{eq:db-for-full-faqneg}, respectively. 
\end{theorem}

\begin{proof}
    We first prove the ``if'' direction. Suppose $\ba = \ba_{[n]} \in Q^*(\db^*)$. Then, we have $\Pi_K \ba \in R^*_K$, for every $K \in \mE^+$, and $\Pi_N \ba \notin R^*_N$, for every $N \in \mE^-$. This implies that $R_K(\Pi_K \ba) \neq \zerobf$, for every $K \in \mE^+$. However, for every $N \in \mE^-$, either $\Pi_N \ba \notin R_N$, or $\Pi_N \ba \in R_N \wedge R_N(\Pi_N \ba) \neq \zerobf$. We prove that $\ba \in \varphi(\db)$, or in other words, $\formula(\ba) \neq \zerobf$, by induction on the $\nestfaqneg$ subexpression $\formula(\bx_{S})$ following the rules of the $\CFG$ \eqref{def:cfg} in a bottom-up fashion. The base case $S = \emptyset$ is trivial, because $\formula(\Pi_{\emptyset} \ba) = e$, where $ e \in \boldsymbol{D} \setminus \{\zerobf\}$. We argue the inductive step. If $\nonterm(\bx_S) \derive \formula(\bx_S)$ uses the production $\nonterm(\bx_{S}) ::= \; R_K(\bx_K) \otimes \nonterm(\bx_{S^-})$ next, and by induction hypothesis $\formula(\Pi_{S^-}\ba) \neq \zerobf$, then $\formula(\Pi_{S}\ba) = R_K(\Pi_{K}\ba) \otimes \formula(\Pi_{S^-}\ba) \neq \zerobf$. Otherwise, $\nonterm(\bx_S) \derive \formula(\bx_S)$ uses the production $(R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-})$ as the next yield step, and by induction hypothesis $\formula(\Pi_{S^-}\ba) \neq \zerobf$ and $\formula(\Pi_{N^-}\ba) \neq \zerobf$. We distinguish the following two cases:
    \begin{itemize}
        \item If $\Pi_N \ba \notin R_N$, then 
        \begin{align*}
            R_N(\Pi_N \ba) \vdash \formula(\Pi_{N^-} \ba) = R_N(\Pi_N \ba) \oplus \indicator{\neg R_N} (\Pi_N \ba) \otimes \formula(\Pi_{N^-} \ba) = \zerobf \oplus \onebf \otimes \formula(\Pi_{N^-} \ba) = \formula(\Pi_{N^-} \ba) \neq \zerobf
        \end{align*}
        \item If $\Pi_N \ba \in R_N$ and $R_N(\Pi_N \ba) \neq \zerobf$, then 
        \begin{align*}
            R_N(\Pi_N \ba) \vdash \formula(\Pi_{N^-} \ba) = R_N(\Pi_N \ba) \oplus \indicator{\neg R_N} (\Pi_N \ba) \otimes \formula(\Pi_{N^-} \ba) = R_N(\Pi_N \ba) \oplus \zerobf \otimes \formula(\Pi_{N^-} \ba) = R_N(\Pi_N \ba) \neq \zerobf
        \end{align*}
    \end{itemize} 
    In both cases, we have $\formula(\Pi_{S}\ba) = (R_N(\Pi_N \ba) \vdash \formula(\bx_{N^-})) \otimes \formula(\Pi_{S^-}\ba) \neq \zerobf$. Therefore, $\varphi(\ba) \neq \zerobf$.

    \medskip
    We then prove the ``only if'' direction. Suppose $\varphi(\ba) \neq \zerobf$. We prove that $\ba \in Q^*(\db^*)$, or in other words, $\Pi_K \ba \in R^*_K$, for every $K \in \mE^+$, and $\Pi_N \ba \notin R^*_N$, for every $N \in \mE^-$. We prove by induction on the $\nestfaqneg$ subexpression $\formula(\bx_{S})$ following the rules of the $\CFG$ \eqref{def:cfg} in a top-down fashion, i.e. tracing the derivation from the start symbol $\nonterm(\bx_{[n]})$ of the $\CFG$ \eqref{def:cfg}. The base case is simply $\varphi(\ba)  = \formula(\ba) \neq \zerobf$. We now argue the inductive step and suppose $\nonterm(\bx_S)$ ($S \neq \emptyset$) is an intermediate non-terminal along the derivation of $\formula(\bx_{[n] })$. By inductive hypothesis, we have that $\formula(\Pi_{S} \ba) \neq \zerobf$. We then distinguish the following two cases:
    \begin{itemize}
        \item If $\nonterm(\bx_S) \derive \formula(\bx_S)$ uses the production $\nonterm(\bx_{S}) ::= R_K(\bx_K) \otimes \nonterm(\bx_{S^-})$ next, then $\formula(\ba_{S^-}) \neq \zerobf$ and $R_K(\Pi_K \ba) \neq \zerobf$. Therefore, $\Pi_K \ba \in R^*_K$.
        \item If $\nonterm(\bx_S) \derive \formula(\bx_S)$ uses the production $\nonterm(\bx_{S}) ::= (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-})$ next, then $\formula(\ba_{S^-}) \neq \zerobf$ and $(R_N(\Pi_N \ba) \vdash \formula(\Pi_{N^-} \ba)) \neq \zerobf$. The latter further implies that $\Pi_N \ba \notin R^*_N$ because if not, then 
        \begin{align*}
            R_N(\Pi_N \ba) \vdash \formula(\Pi_{N^-} \ba) = \zerobf \oplus \zerobf \otimes \formula(\Pi_{N^-} \ba) = \zerobf
        \end{align*}
        and we get a contradiction. Thus, we have proven that $\ba \in Q^*(\db^*)$ and close the proof.
    \end{itemize}
\end{proof}

An immediate corrollary from \autoref{thm:enum-full-faqneg} is the following, as a special case of \autoref{thm:faqneg-main}.
\begin{corollary} \label{cor:enum-full-faqneg}
    Let $\varphi$ be a \emph{full} $\pn$-acyclic $\nestfaqneg$ query over a commutative semiring $\bS$. Then, there is an algorithm that can enumerate the answers of $\varphi$ in $O(|\varphi|)$ delay, after a $O(|\varphi|^3 + |\varphi| \cdot |\db|)$ preprocessing time.
\end{corollary}

From the next section onwards, we study the enumeration problem of free-connex $\pn$-acyclic $\nestfaqneg$ queries.


\subsection{Enumeration of free-connex $\pn$-acyclic $\nestfaqneg$} \label{sec:enum-free-connex-faqneg}
In the following sections, we let $\varphi$ be a free-connex $\pn$-acyclic $\nestfaqneg$ query \eqref{def:nestfaqneg} with free variables $F = [f]$ and $\mH = ([n], \mE^+, \mE^-)$ be its associated signed hypergraph. We let $\formula(\bx_{[n]})$ be the $\nestfaqneg$ expression of $\varphi$, recognized by the $\CFG$ defined in \eqref{def:cfg}. As $\mH$ is $\pn$-acyclic, W.L.O.G, it accepts a $\pn$-elimination sequence $(1, 2, \dots, f \dots, n)$. 

On a high level, our preprocessing algorithm takes as input $(i)$ the $\nestfaqneg$ expression $\formula(\bx_{[n]})$, and $(ii)$ its database instance $\db$, and for each $i = n-1, n-2, \dots, f$ (following the $\pn$-elimination order), it executes a \textbf{$\pn$-elimination step on $i$}, that constructs an intermediate $\nestfaqneg$ expression $\formula_{i}(\bx_{[i]})$ and its database instance $\db_i$, where 
\begin{itemize}
    \item $\formula_{i}(\bx_{[i]})$ is associated with the signed hypergraph $\mH_i = \removeleaf{\mH_{i+1}}{i+1}$, i.e. the signed hypergraph after eliminating $n, n-1, \dots, i+1$ from $\mH$, (if $i = n-1$, then $\mH_{n-1} = \removeleaf{\mH}{n}$)
    \item $\db_{i}$ is an intermediate database instance of $\formula_{i}(\bx_{[i]})$ such that $\formula_{i}(\bx_{[i]}) = \bigoplus_{x_{i+1} \in \dom(x_{i+1})} \formula_{i+1}(\bx_{[i+1]}) $. Here, $\formula_{i}(\bx_{[i]}) = \bigoplus_{x_{i+1} \in \dom(x_{i+1})} \formula(\bx_{[i+1]})$ indicates: for any $\ba_{[i]} \in \dom(\bx_{[i]})$, we have $\formula_{i}(\ba_{[i]}) = \bigoplus_{x_{i+1} \in \dom(x_{i+1})} \formula(x_{i+1}, \ba_{[i]})$, where $\formula(\bx_{[i+1]})$ is evaluated on $\db_{{i+1}}$ and $\formula_{i}(\bx_{[i]})$ is evaluated on $\db_{i}$.
\end{itemize}
The last $\nestfaqneg$ expression $\formula_f(\bx_{[f]})$, after the sequence of $\pn$-elimination steps on $n-1, n-2, \dots, f$, becomes a full $\nestfaqneg$ query whose associated signed hypergraph $\mH_f$ accepts a $\pn$-elimination sequence $(1, 2, \dots, f)$ and 
        \begin{align*}
            \varphi(\bx_F) = \bigoplus_{\bx_{[n] \setminus F} \in \dom(\bx_{[n] \setminus F})} \; \formula(\bx_{[n]}) = \bigoplus_{\bx_{[n-1] \setminus F} \in \dom(\bx_{[n-1] \setminus F})} \; \formula_{n-1}(\bx_{[n-1]}) = \cdots = \formula_f(\bx_{[f]}).
        \end{align*}

Thus, we degenerate to the case where $\varphi$ is a full $\pn$-acyclic $\nestfaqneg$ query and our algorithm simply follows our discussion in the last section (Appendix~\ref{sec:enum-full-faqneg}): reduce $\Enum(\formula_f(\bx_{[f]}), \db_{f})$ into $\Enum(Q^*_{f}(\bx_{[f]}), \db^*_{f})$, where $Q^*_{f}$ is a full $\pn$-acyclic $\cqneg$ and apply the preprocessing algorithm for full $\cqneg$. At the enumeration phase, we emit each answer $\ba_{F}$ of $Q^*_{f}(\db_{f})$ (applying the enumeration algorithm for full $\cqneg$) and plug the emitted tuple $\ba_{F}$ into $\formula_f$ to get recover its weight $\formula_f(\ba_{F}) = \varphi(\ba_{F})$.

% \hangdong{very important assumptions:  \\
% 1. postive factors contain only positive weights -> the algorithm will mimic $\alpha$-elimiation as Yannakakis or InsideOut alg by only operating on the topmost level of ASTs. \\
% 2. the query must be safe - every variable must appear in some positive factor that shows up in the AST. 
% }

%%%%%%%%%%%%%%%%%%%%%%%%%% finished todos %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hangdong{todo:
% 1. preprocessing phase alg (elimination step -> new sub-faq query and new relations)
% 	\begin{enumerate}
% 		\item $\varphi, \db, (x_1, x_2, \dots, x_f \dots, x_n) \rightarrow \varphi', \db', (x_1, x_2, \dots, x_f \dots, x_{n-1}) \rightarrow \cdots \rightarrow \varphi^*, \db^*, (x_1, x_2, \dots, x_f)$: for each elimination step of $v_n$ (or call it aggregation step of $v_n$, aka $\bigoplus_{v_n}$),
% 		\item syntax on ASTs (how to maintain the ASTs?) -> this tells us how to get $\varphi'$ -> \textcolor{blue}{$O(|\varphi|)$ time}
% 			\begin{enumerate}
% 				\item \textcolor{blue}{factor out those atoms that doesn't contain $n$ (some are nested in the ASTs, they are to be factored out in sub ASTs}
% 				\item ($\alpha$-step at each subtree) choose a biggest positive factor $R_U(\bx_U)$ containing $n$ -> eat some smaller positive (leaves) and negative subtrees immediately -> some smaller negatives will be eaten as $R_U(\bx_U)$ gets pushed downward the AST (on the fly) + make a ghost copy of the biggest positive factor $I_{U \setminus \{n\}}(\bx_{U \setminus \{n\}})$ without $n$ as a future guard; keep pushing $R_U(\bx_U)$ down to the right order and swallow the rightmost positive subtree -> it leads to an ordered AST structure
% 				\item ($\beta$-step at the negative subtree (if there is any) for $n$) after all $\alpha$ steps -> AST structure:
% 					\begin{enumerate} 
% 						\item the task $\bigoplus_{n} $
% 						\item sub AST = the root $\bigotimes$ and children are a bunch of sub-ASTs
% 						\item a refactoring algorithm (strip off $n$ with no change on the (linear nested) query structure) + a bottom-up interval range sum
% 					\end{enumerate}
% 			\end{enumerate}
% 		\item accumulative range sum -> this tells us how to get $\db'$ (with the aggregated weights) -> \textcolor{blue}{$\cdelay$ time}
% 		\item reduce from full faq into enumeration of a full scq 
% 	\end{enumerate}
% 2. enumeration phase alg (call scq enumeration alg + plug-in for faq weights)
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\medskip
\introparagraph{$\pn$-elimination step}
% Recall that a $\nestfaqneg$ query $\varphi$, associated with a signed hypergraph $\mH = ([n], \mE^+, \mE^-)$, is an aggregation over a $\nestfaqneg$ expression $\formula(\bx_{[n]})$ recognized by the $\CFG$ \eqref{def:cfg} (i.e. $\nonterm(\bx_{[n]}) \derive \formula(\bx_{[n]})$). 
W.L.O.G, we let $n$ be the given $\pn$-leaf of $\mH$ and appoint $U$ to be a pivot hyperedge, breaking ties arbitrarily. We call the factor $R_U(\bx_U)$ corresponding to $U$ the \emph{pivot factor}. A $\pn$-elimination step runs the following 3 algorithms consecutively:

\begin{enumerate}
    \item \textbf{the refactoring algorithm (Appendix~\ref{sec:rewriting})} The refactoring algorithm takes the given $\nestfaqneg$ expression $\formula(\bx_{[n]})$ and database instance $\db$ as input and returns $(\formula_n(\bx_{[n]}), \db_n)$ as output where 
    \begin{itemize}
        \item $\formula_n(\bx_{[n]})$ is a new $\nestfaqneg$ expression recognized by the following (more restrictive) $\CFG_n$ associated with the signed hypergraph $\mH_n = ([n], \mE^+_n, \mE^-_n)$, where $\mE^+_n = \{K \in \mE^+ \mid n \notin K\} \cup \{U \} \subseteq \mE^+$ and $\mE^-_n = \{N \in \mE^- \mid n \notin N \vee n \in U \subset N \} \subseteq \mE^-$,
        %%%%%%%%%%%%%%%%%%%%%%%%%% the old CFG_n %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            % \begin{equation}
            %     \begin{aligned}
            %         \CFG_n: \qquad \qquad \; \\
            %         \text{ for all } S \subseteq [n], \\
            %         \nonterm_n(\bx_{\emptyset}) &::= \; e  
            %         && \text{ where } e \in \boldsymbol{D} \\
            %         \nonterm_n(\bx_{S}) &::= \; R_K(\bx_K) \otimes \nonterm_n(\bx_{S^-}),  
            %         && \text{ where } K \in \mE^+_n \text{ and } S^- \subseteq S \text{ such that } S = K \cup S^- \\
            %         & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_n(\bx_{N^-})) \otimes \nonterm_n(\bx_{S^-}), 
            %         && \text{ where } N \in \mE^-_n, N^- \subseteq N \text{ and } S^- \subseteq S \text{ such that } S = N \cup S^- 
            %     \end{aligned}
            % \end{equation}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \begin{equation} \label{eq:cfg_n}
                \begin{aligned}
                    \framebox{$\CFG_n$} \qquad \qquad \; \\
                    \text{ for all } S \subseteq [n], \\
                    \nonterm_n(\bx_{\emptyset}) &::= \; e  
                    && \text{ where } S = \emptyset \text{ and } e \in \boldsymbol{D} \setminus \{\zerobf\} \\
                    \nonterm_n(\bx_{S}) &::= \; R_U(\bx_U) 
                    && \text{ where } S = U \\
                    & \; \; \mid \; R_K(\bx_K) \otimes \nonterm_n(\bx_{S^-})
                    && \text{ where } S = K \cup S^- \text{ and } K \in \{K \in \mE^+ \mid n \notin K\}   \\
                     & \; \; \mid \; (R_{N}(\bx_{N}) \vdash \nonterm_n(\bx_{N^-}))
                    && \text{ where } S = N \text{ and }  N^- \subseteq N \in \{N \in \mE^- \mid n \in U \subset N \}  \\
                    & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_n(\bx_{N^-})) \otimes \nonterm_n(\bx_{S^-})
                    && \text{ where } S = N \cup S^- \text{ and } N^- \subseteq N \in \{N \in \mE^- \mid n \notin N\} 
                \end{aligned}
            \end{equation}
        \item $\db_n$ is the corresponding database instance of $\formula_n(\bx_{[n]})$ such that $\formula_n(\bx_{[n]}) = \formula(\bx_{[n]})$. We observe that $\CFG_n$ is more restrictive than $\CFG$ \eqref{def:cfg} in that it has strictly less productions for the non-terminals $\nonterm_n(\bx_S)$ where $n \in S$. The refactoring algorithm uses the pivot factor $R_U$ to ``absorb'' the factors $R_K$ and $R_N$ where $n \in K \subseteq U$, $n \in N \subseteq U$. By the properties of a $\pn$-leaf $n$, the only hyperedges containing $n$ left in $\mH_n$ are $U$ and $N_1, \dots, N_k \in \mE^-$ for some $k$ such that $U \subseteq N_1 \subseteq \dots \subseteq N_k$.
    \end{itemize}
    \item \textbf{the oracle-construction algorithm (Appendix~\ref{sec:oracle})} The oracle-construction algorithm takes the $\nestfaqneg$ expression $\formula_n(\bx_{[n]})$ recognized by $\CFG_n$ \eqref{eq:cfg_n}, and the database instance $\db_n$ from the refactoring algorithm and constructs an oracle data structure for the following $\nestfaqneg$ subexpressions show up in $\formula_n(\bx_{[n]})$: $\formula_n(\bx_{U})$ and $\formula_n(\bx_{N_i})$, where $i \in [k]$. The oracle-construction algorithm is analogous to the $\beta$-step in the enumeration of full $\cqneg$ queries, but instead of linked lists, it builds arrays and \textsf{RangeSum} data structures that support fast aggregation in the upcoming aggregation algorithm.
    \item \textbf{the aggregation algorithm (Appendix~\ref{sec:aggregation})} The aggregation algorithm takes $(\formula_n(\bx_{[n]}), \db_n)$ and uses the constructed oracles 
    to finally constructs the desired $(\formula_{n-1}(\bx_{n-1}), \db_{n-1})$, where 
    \begin{itemize}
        \item $\formula_{n-1}(\bx_{n-1})$ is a new $\nestfaqneg$ expression recognized by the grammar $\CFG_{n-1}$ associated with $\mH_{n-1} = \removeleaf{\mH}{n}$, or equivalently, $\mH_{n-1} = ([n-1], \mE^+_{n-1}, \mE^-_{n-1})$, where $\mE^+_{n-1} = \{K \setminus \{n\} \mid K \in \mE^+_n \}$ and $\mE^-_{n-1} = \{N \setminus \{n\} \mid N \in \mE^-_n\}$. The grammar $\CFG_{n-1}$ is defined as follows:
        %%%%%%%%%%%%%%%%%%%%%%%%% the old CFG_n-1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{equation} \label{eq:cfg_n-1}
            \begin{aligned}
                \framebox{$\CFG_{n-1}$} \qquad \qquad \; \\
                \text{ for all } S \subseteq [n-1], \\
                    \nonterm_{n-1}(\bx_{\emptyset}) &::= \; e  
                    && \text{ where } S = \emptyset \text{ and } e \in \boldsymbol{D} \setminus \{\zerobf\}  \\
                    \nonterm_{n-1}(\bx_{S}) &::= \; R_K(\bx_K) \otimes \nonterm_{n-1}(\bx_{S^-}),  
                    && \text{ where } S = K \cup S^- \text{ and } K \in \mE^+_{n-1}, S^- \subseteq S  \\
                    & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_{n-1}(\bx_{N^-})) \otimes \nonterm_{n-1}(\bx_{S^-}), 
                    && \text{ where } S = N \cup S^-, N^- \subseteq N \in \mE^-_{n-1} \text{ and } S^- \subseteq S 
            \end{aligned}
        \end{equation}
        % \begin{equation} \label{eq:cfg_n-1}
        %     \begin{aligned}
        %         \CFG_{n-1} \qquad \qquad \; \\
        %         \text{ for all } S \subseteq [n-1], \\
        %         \nonterm_{n-1}(\bx_{\emptyset}) &::= \; e  
        %         && \text{ where }  S = \emptyset \text{ and } e \in \boldsymbol{D} \setminus \{\zerobf\}   \\
        %         \nonterm_{n-1}(\bx_{S}) &::= \; R_U(\bx_U) 
        %         && \text{ where } S = U \setminus \{n\} \\
        %         & \; \; \mid \; R_K(\bx_K) \otimes \nonterm_{n-1}(\bx_{S^-}) 
        %         && \text{ where } S = K \cup S^- \text{ and } K \in \{K \in \mE^+ \mid n \notin K\}   \\
        %         & \; \; \mid \; (R_{N}(\bx_{N}) \vdash \nonterm_{n-1}(\bx_{N^-}))
        %         && \text{ where } S = N \text{ and } N^- \subseteq N \in \{N \setminus \{n\} \mid N \in \mE^-, n \in U \subset N \}  \\
        %         & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_{n-1}(\bx_{N^-})) \otimes \nonterm_{n-1}(\bx_{S^-}) 
        %         && \text{ where } S = N \cup S^- \text{ and } N^- \subseteq N \in \{N \in \mE^- \mid n \notin N\} 
        %     \end{aligned}
        % \end{equation}
        \item $\db_{n-1}$ is the corresponding database instance of $\formula_{n-1}(\bx_{n-1})$ such that $\formula_{n-1}(\db_{n-1}) = \bigoplus_{x_n \in \dom(x_n)} \formula_n(\bx_{[n]})$.
    \end{itemize}
\end{enumerate}

As a recap, a $\pn$-elimination step on $n$ aggregates out $x_n$ from the $\nestfaqneg$ expression $\formula(\bx_{[n]})$ and outputs a $\nestfaqneg$ expression $\formula_{n-1}(\bx_{[n-1]})$ associated with $\mH_{n-1}= \removeleaf{\mH}{n}$ and its database instance $\db_{n-1}$ such that $\formula_{n-1}(\bx_{[n-1]}) = \bigoplus_{x_n \in \dom(x_n)} \formula(\bx_{[n]})$. Now, we can keep applying the $\pn$-elimination step on the next $\pn$-leaf $n-1$ and so on, untill all variables in $[n] \setminus F$ have been removed. 

\subsection{The refactoring algorithm} \label{sec:rewriting}
In this section, we present the refactoring algorithm that refactors $\formula(\bx_{[n]})$ into $\formula_n(\bx_{[n]})$, a $\nestfaqneg$ expression associated with $\mH_n$. We start from $\nonterm(\bx_{[n]}) \derive \formula(\bx_{[n]})$, the derivation in $\CFG$ \eqref{def:cfg}, and refactor it step-by-step into a derivation of $\formula_n(\bx_{[n]})$ in $\CFG_n$ \eqref{eq:cfg_n}, i.e. $\nonterm_n(\bx_{[n]}) \derive \formula_n(\bx_{[n]})$. Along the way, we will also update the database instance $\db$ accordingly, leading to $\db_n$ at the end. In particular, we let 
$$
\formula_n(\bx_{[n]}) = \Rewrite \left(\nonterm(\bx_{\emptyset}) \yield \onebf, \nonterm(\bx_{[n]}) \derive \formula(\bx_{[n]}) \right),
$$
where $\Rewrite \left(\nonterm(\bx_{M}) \derive \mu(\bx_{M}) , \nonterm(\bx_{S}) \derive \formula(\bx_{S}) \right)$, for some $M, S \subseteq [n]$, is an invokation of a recursive algorithm $\Rewrite$ that takes the following inputs: 
\begin{enumerate}
    \item a stashed derivation of a $\nestfaqneg$ subexpression $\mu(\bx_{M})$, i.e. $\nonterm(\bx_{M}) \derive \mu(\bx_{M})$, such that its first yield step will be maintained to be one of the followings:
    \begin{itemize}
        \item if $n \notin M$, then it follows that $M = \emptyset$ and $\mu(\bx_{M}) \yield \onebf$; or 
        \item otherwise $n \in M$, then it applies the production of $\CFG$ that uses the largest hyperedge among all productions that can be used as the next yield step, if there is any (an arbitrary choice otherwise)
    \end{itemize}
    \item a derivation of a $\nestfaqneg$ subexpression $\formula(\bx_{S})$, i.e. $\nonterm(\bx_{S}) \derive \formula(\bx_{S})$, for some $S \subseteq [n]$;
    \item a database instance $\db$ of $\formula(\bx_{[n]})$ as a global input,
\end{enumerate}
and returns a $\nestfaqneg$ subexpression $\formula_n(\bx_{M \cup S})$ recognized by $\CFG_n$ and a database instance $\db_n$ corresponding to $\formula_n(\bx_{[n]})$, such that $\nonterm_n(\bx_{M \cup S}) \derive \formula_{n}(\bx_{M  \cup S}) = \mu(\bx_{M}) \otimes \formula(\bx_{S})$. The refactoring algorithm $\Rewrite$ is illustrated in Algorithm~\ref{alg:rewrite} and formally, we prove the following lemma. 


\begin{algorithm}[t]
    \KwIn{two derivations in $\CFG$, $\nonterm(\bx_{M}) \derive \mu(\bx_{M})$ and $\nonterm(\bx_{S}) \derive \formula(\bx_{S})$, for some $M, S \subseteq [n]$ }
    \KwIn{a global database instance $\db$ of $\formula(\bx_{[n]})$}
    \KwOut{an expression $\formula_n(\bx_{M \cup S})$ recognized by $\CFG_n$ such that $\nonterm_n(\bx_{M \cup S}) \derive \formula_n(\bx_{M \cup S}) = \mu(\bx_{M}) \otimes \formula(\bx_{S})$.}
    \BlankLine
    \If{$\nonterm(\bx_{S}) \yield \onebf$}{
        \If(\Comment{base case} \label{alg:rewrite:base-case}){$\nonterm(\bx_{M}) \yield \onebf$}{
            \Return $\onebf$   \;
        }
        \ElseIf(\Comment{(2.2)} \label{alg:rewrite:2.2}){$\nonterm(\bx_{M}) \yield R_U(\bx_U) \otimes \nonterm(\bx_{M^-})$}{
            $\absorb{R_U}(\bx_U) \leftarrow R_U(\bx_U) \otimes \mu(\bx_{M^-})$  \;
            \Return $\absorb{R_U}(\bx_U)$ \label{alg:rewrite:2.2} \;
        }
        \ElseIf(\Comment{(2.1)} \label{alg:rewrite:2.1}){$\nonterm(\bx_{M}) \yield (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{M^-})$}{
            $\absorb{R_N}(\bx_N) \leftarrow R_N(\bx_N) \otimes \mu(\bx_{M^-})$  \label{alg:rewrite:2.1} \;
            \Return $\left( \absorb{R_N}(\bx_N) \vdash \Rewrite \left(\nonterm(\bx_{M^-}) \derive \mu(\bx_{M^-}), \nonterm(\bx_{N^-}) \derive \formula(\bx_{N^-}) \right) \right)$ \label{alg:rewrite:case-pos-base} \;
        }
    }
    \ElseIf(\Comment{(3.3)} \label{alg:rewrite:3.3}){$\nonterm(\bx_{S}) \yield e$}{
            \Return $e \otimes e_{\emptyset} \otimes \Rewrite(\widetilde{\nonterm}(\bx_{M}) \derive \widetilde{\mu}(\bx_{M}), \nonterm(\bx_{S}) \derive \onebf)$  \label{alg:rewrite:case-e} \;
    } 

    \ElseIf(\Comment{$K \in \mE^+, S^- \subseteq [n]$ such that $S = K \cup S^-$} \label{alg:rewrite:3.1} ){$\nonterm(\bx_{S}) \yield R_K(\bx_K) \otimes \nonterm(\bx_{S^-})$}{    
        \If(\Comment{(3.1)}){$n \notin K$}{
            \Return $R_K(\bx_K) \otimes \Rewrite(\nonterm(\bx_{M}) \derive \mu(\bx_{M}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))$   \label{alg:rewrite:case-pos1} \;
        }
        \Else(\Comment{(4.1)} \label{alg:rewrite:4.1}){
            \textbf{augment} the stash derivation $\nonterm(\bx_{M}) \derive \mu(\bx_{M})$ into 
            $\nonterm(\bx_{M \cup K}) \yield R_K(\bx_K) \otimes \nonterm(\bx_{M}) \derive \mu(\bx_{M \cup K})$  \;
            \Return $\Rewrite(\nonterm(\bx_{M \cup K}) \derive \mu(\bx_{M \cup K}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))$ \label{alg:rewrite:case-pos2} \;
        }
    }
    \ElseIf(\Comment{$N \in \mE^-, N^- \subseteq N, S^- \subseteq [n]$ such that $S = N \cup S^-$}  \label{alg:rewrite:case-neg}) {$\nonterm(\bx_{S}) \yield (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-})$ }  
    {  
        \If(\Comment{(3.2)} \label{alg:rewrite:3.2} ){$n \notin N$}{
            \Return $(R_N(\bx_N) \vdash \mu(\bx_{N^-})) \otimes \Rewrite(R_U(\bx_U), \nonterm(\bx_{M}) \derive \mu(\bx_{M}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))$  \label{alg:rewrite:case-neg1} \;
        }
        \Else(\Comment{(4.2)} \label{alg:rewrite:4.2} ){
            \textbf{augment} the stash derivation $\nonterm(\bx_{M}) \derive \mu(\bx_{M})$ into 
            $\nonterm(\bx_{M \cup N}) \yield  \left(R_N(\bx_N) \vdash \nonterm(\bx_{N^-}) \right) \otimes \nonterm(\bx_{M}) \derive \mu(\bx_{M \cup N})$  \;
            \Return $\Rewrite(\nonterm(\bx_{M \cup N}) \derive \mu(\bx_{M \cup N}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))$ \label{alg:rewrite:case-neg2.2} \;
        }
    }
    \caption{The refactoring algorithm $\Rewrite(\nonterm(\bx_{M}) \derive \mu(\bx_{M}), \nonterm(\bx_{S}) \derive \formula(\bx_{S}))$}
    \label{alg:rewrite}
\end{algorithm}


\begin{lemma} \label{lem:rewrite}
    Let $\mH = ([n], \mE^+, \mE^-)$ be a signed hypergraph, $n$ be a $\pn$-leaf of $\mH$ and $U$ be a pivot hyperedge. Let $\varphi$ be a free-connex $\pn$-acyclic $\nestfaqneg$ query \eqref{def:nestfaqneg} associated with $\mH$ and $\db$ be a (global) database instance of $\varphi$. There is an algorithm that takes the following as input
    \begin{enumerate}
        \item a derivation of a $\nestfaqneg$ subexpression $\mu(\bx_{M})$, i.e. $\nonterm(\bx_{M}) \derive \mu(\bx_{M})$, for some $M \subseteq [n]$ such that if $n \notin M$, then $M = \emptyset$ and $\mu(\bx_{M}) \yield \onebf$;
        \item a derivation of a $\nestfaqneg$ subexpression $\formula(\bx_{S})$, i.e. $\nonterm(\bx_{S}) \derive \formula(\bx_{S})$, for some $S \subseteq [n]$;
        \item a global database instance $\db$ of $\formula(\bx_{[n]})$
    \end{enumerate}
    and then returns a subexpression $\formula_n(\bx_{M \cup S})$ of $\CFG_n$ \eqref{eq:cfg_n} such that $\nonterm_n(\bx_{M \cup S}) \derive \formula_n(\bx_{M \cup S})$ and a corresponding (global) database instance $\db_n$ such that
    \begin{enumerate}
        \item $\nonterm_n(\bx_{M \cup S}) \derive \formula_n(\bx_{M \cup S}) = \mu(\bx_{M}) \otimes \formula(\bx_{S})$,
        \item $|\db_n| = O(\dbsize)$,
        \item the length of the derivation $\nonterm_n(\bx_{M \cup S}) \derive \formula_n(\bx_{M \cup S})$ is at most $|\eta|$, where $|\eta|$ is the length of the derivation $\nonterm(\bx_{S}) \derive \formula(\bx_{S})$ plus the length of the derivation $\nonterm(\bx_{M}) \derive \mu(\bx_{M})$.
        \item runs in time $O(|\eta|^2  + d(n) \cdot \dbsize)$, where $d(n)$ is the number of hyperedges in $\mH$ that contains $n$.
    \end{enumerate}
\end{lemma}


\begin{proof}
    We prove the lemma by induction on $|\eta| \geq 2$ for every if-else branch in $\Rewrite$. We first examine the case where \textcolor{blue}{the next yield step of $\nonterm(\bx_{S})$ is $\nonterm(\bx_{\emptyset}) \yield \formula(\bx_{\emptyset})  = \onebf$, so $S = \emptyset$}. We divide into $2$ main cases (case (1) and (2)), one for each next yield step of $\nonterm(\bx_{M})$: 
    \begin{enumerate}
        \item (\autoref{alg:rewrite:base-case}) the base case is when $M = \emptyset$ and $\nonterm(\bx_{M}) \yield \mu(\bx_{\emptyset}) = \onebf$, in which case ($M = S = \emptyset, |\mu| = |\formula|  = 1$) we simply return \highlight{$\onebf$} and the lemma is trivially true. Indeed, it uses the production \textcolor{orange}{$\nonterm_n(\bx_{\emptyset}) ::= \onebf$ in $\CFG_n$}.
        \item otherwise, ($n \in M)$, \highlight{recall $S = \emptyset$ now, so there must be one largest hyperedge in $\mu(\bx_M)$, by the $\beta$-property of the $\pn$-leaf $n$} and we have the following cases:
        \begin{enumerate}
            \item [(2.1)] (\autoref{alg:rewrite:2.1}) let the next yield step of $\nonterm(\bx_{M})$ be 
               \begin{align*}
                    \nonterm(\bx_{M}) \yield (R_{N}(\bx_{N}) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{M^-}) \derive (R_{N}(\bx_{N}) \vdash \mu(\bx_{N^-})) \otimes \mu(\bx_{M^-})
                \end{align*}
                where $N \in \mE^-$, $N^- \subseteq N$ and $M^- \subseteq M$ such that $M = N \cup M^-$. As $N$ is the largest hyperedge used among the next yield steps of $\nonterm(\bx_{M})$, we have $M^- \subseteq N$. Then we have
                \begin{align*}
                    \nonterm(\bx_{M}) \otimes \nonterm(\bx_{S}) & \derive (R_{N}(\bx_{N}) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{M^-})  \otimes \onebf\\
                    & \derive (R_{N}(\bx_{N}) \vdash \mu(\bx_{N^-})) \otimes \mu(\bx_{M^-}) \otimes \onebf \\
                    & = \; \absorb{R_{N}}(\bx_{N}) \vdash \left(\mu(\bx_{N^-}) \otimes \mu(\bx_{M^-}) \right)
                \end{align*}
                where $\absorb{R_{N}}(\bx_{N}) = R_{N}(\bx_{N}) \otimes \mu(\bx_{M^-})$ is an updated negative factor that can be computed in $O(|R_N|)$ time. Recall that we return in this case
                \begin{align*}
                    \textcolor{red}{\left(\absorb{R_{N}}(\bx_{N}) \vdash \Rewrite \left(\nonterm(\bx_{M^-}) \derive \mu(\bx_{M^-}), \nonterm(\bx_{N^-}) \derive \mu(\bx_{N^-}) \right)\right)}.
                \end{align*}
                Now, we observe that the first yield step in the stashed derivation $\nonterm(\bx_{M}) \yield (R_{N}(\bx_{N}) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{M^-})  \derive \formula(\bx_{M}) $ is trimmed off in this inner recursive call. That is, $|\eta|$ decrements by 1 in the recursion. By the induction hypothesis,
                \begin{align*}
                    \nonterm_n(\bx_{M^- \cup N^-}) & \derive \formula_n(\bx_{M^- \cup N^-}) = \mu(\bx_{M^-}) \otimes \mu(\bx_{N^-})  = \Rewrite \left(\nonterm(\bx_{M^-}) \derive \mu(\bx_{M^-}), \nonterm(\bx_{N^-}) \derive \mu(\bx_{N^-}) \right).
                \end{align*}
                Thus, we get
            \begin{align*}
                \mu(\bx_{M}) \otimes \formula(\bx_{S}) & = (R_{N}(\bx_{N}) \vdash \mu(\bx_{N^-})) \otimes \mu(\bx_{M^-}) \otimes \onebf \\
                & = \absorb{R_{N}}(\bx_{N}) \vdash \left(\mu(\bx_{M^-}) \otimes \mu(\bx_{N^-})\right) \\
                & = \left(\absorb{R_{N}}(\bx_{N}) \vdash \Rewrite \left(\nonterm(\bx_{M^-}) \derive \mu(\bx_{M^-}), \nonterm(\bx_{N^-}) \derive \mu(\bx_{N^-}) \right)\right).
            \end{align*}
            and $\nonterm_n(\bx_{M \cup S})$ indeed derives this subexpression in $\CFG_n$ because (now $S = \emptyset$ and $M = N$, so $M \cup S = N$)
            \begin{align*}
                \nonterm_n(\bx_{M \cup S}) & \; \yield \absorb{R_{N}}(\bx_{N}) \vdash \nonterm_n(\bx_{M^- \cup N^- })  \\
                & \; \yield \absorb{R_{N}}(\bx_{N}) \vdash \nonterm_n(\bx_{M^- \cup N^- })  \\
                & \; \derive \absorb{R_{N}}(\bx_{N}) \vdash \formula_n(\bx_{M^- \cup N^-})  && \text{ (induction hypothesis) }\\
                & \; = \absorb{R_{N}}(\bx_{N}) \vdash \left(\mu(\bx_{M^-}) \otimes \mu(\bx_{N^-})\right) \\
                & \; =  \mu(\bx_{M}) \otimes \formula(\bx_{S})  
            \end{align*}
            where \textcolor{orange}{the first yield step here uses the production $\nonterm_n(\bx_{N}) ::= R_{N}(\bx_{N}) \vdash \nonterm_n(\bx_{N^-})$, where $S = N$ and $N^- \subseteq N \in \{N \in \mE^- \mid n \in U \subset N\}$}.
            \item [(2.2)] (\autoref{alg:rewrite:2.2}) \highlight{if there is no $N \supseteq U$ (only $N \subset U$ lower), then in the children of the root, there must be $R_U$, because $R_U$ can no longer hide lower in any subtrees of the AST}, thus let the next yield step of $\nonterm(\bx_{M})$ be 
             \begin{align*}
                \nonterm(\bx_{M}) \yield R_U(\bx_U) \otimes \nonterm(\bx_{M^-}) \derive R_U(\bx_U) \otimes \mu(\bx_{M^-})
             \end{align*}
             where $M^- \subseteq M$. As $U$ is the largest hyperedge used among the next yield steps of $\nonterm(\bx_{M})$, we have $M^- \subseteq U$. Then we have
                \begin{align*}
                    \nonterm(\bx_{M}) \otimes \nonterm(\bx_{S}) & \derive R_U(\bx_U) \otimes \nonterm(\bx_{M^-}) \otimes \onebf \\
                    & \derive R_U(\bx_U) \otimes \mu(\bx_{M^-})  \otimes \onebf  \\
                    & = \; \absorb{R_U}(\bx_U) 
                \end{align*}
                where $\absorb{R_U}(\bx_U) = R_U(\bx_U) \otimes \mu(\bx_{M^-})$ is an updated positive factor that can be computed in $O(|R_U|)$ time.Recall that we simply return in this case \textcolor{red}{$\absorb{R_U}(\bx_U)$} and the lemma is trivially true. Indeed, the next production of $\CFG_n$ to be used is \textcolor{orange}{$\nonterm_n(\bx_{U}) ::= R_U(\bx_U)$}.
        \end{enumerate}    
    \end{enumerate}
    Next, we examine the case where \textcolor{blue}{the next yield step of $\nonterm(\bx_{S})$ is not $\nonterm(\bx_{S}) \yield \onebf$}. Now, $\Rewrite$ prioritizes processing the next yield steps of $\nonterm(\bx_{S})$ over those of $\nonterm(\bx_{M})$. We distinguish the following two cases: one for $n$ not being contained in the hyperedge used in the next yield step, and the other for the opposite.
    
    \begin{enumerate}
        \item [(3)] First, we examine the case where $n$ is not contained in the hyperedge in the next yield step of $\nonterm(\bx_{S})$. There are 3 subcases, one for each next yield step of $\nonterm(\bx_{M})$:
            \begin{enumerate}
                \item [(3.1)] (\autoref{alg:rewrite:3.1}) $\nonterm(\bx_{S}) \yield  R_K(\bx_K) \otimes \nonterm(\bx_{S^-}) \derive R_K(\bx_K) \otimes \formula(\bx_{S^-})$, for some $K \in \mE^+, S^- \subseteq [n]$ such that $S = K \cup S^-$. If $n \notin K$, then by the induction hypothesis, 
                \begin{align*}
                    \nonterm_n(\bx_{M \cup S^-}) \derive \formula_n(\bx_{M \cup S^-}) = \Rewrite(\nonterm(\bx_{M}) \derive \mu(\bx_{M}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))
                \end{align*}
                since $|\eta|$ decrements by 1 (the first yield step $\nonterm(\bx_{S}) \yield  R_K(\bx_K) \otimes \nonterm(\bx_{S^-})$ is trimmed off in the recursive call). In the $\CFG$, we have
                \begin{align*}
                    \nonterm(\bx_{M}) \otimes \nonterm(\bx_{S}) & \yield \; \nonterm(\bx_{M}) \otimes \left( R_K(\bx_K) \otimes \nonterm(\bx_{S^-}) \right) \\
                    & \derive \; R_K(\bx_K) \otimes \left( \mu(\bx_{M}) \otimes \formula(\bx_{S^-}) \right) \\
                    &= \; R_K(\bx_K) \otimes \Rewrite(\nonterm(\bx_{M}) \derive  \mu(\bx_{M}), \nonterm(\bx_{S^-}) \derive  \formula(\bx_{S^-}))
                \end{align*}
                (recall that we return \highlight{$R_K(\bx_K) \otimes \Rewrite(\nonterm(\bx_{M}) \derive \mu(\bx_{M}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))$}). Moreover, $\nonterm_n(\bx_{M \cup S})$ derives this expression in $\CFG_n$ because 
                \begin{align*}
                    \nonterm_n(\bx_{ M \cup S}) \yield R_K(\bx_K) \otimes \nonterm_n(\bx_{M \cup S^-}) \derive R_K(\bx_K) \otimes \formula_n(\bx_{M \cup S^-}) 
                \end{align*}
                where \textcolor{orange}{the first yield step here uses the production $\nonterm_n(\bx_{S}) ::= R_K(\bx_K) \otimes \nonterm_n(\bx_{S^-})$, where $S = K \cup S^-$ and $K \in \{K \in \mE^+ \mid n \notin K\} $}.
                \item [(3.2)] (\autoref{alg:rewrite:3.2}) $\nonterm(\bx_{S}) \yield (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-}) \derive (R_N(\bx_N) \vdash \mu(\bx_{N^-})) \otimes \formula(\bx_{S^-}) $, for some $N \in \mE^-, N^- \subseteq N$, and $S^- \subseteq [n]$ such that $S = N \cup S^-$. If $n \notin N$, then by the induction hypothesis,
                \begin{align*}
                    \nonterm_n(\bx_{M \cup S^-}) \derive \formula_n(\bx_{M \cup S^-}) = \Rewrite(\nonterm(\bx_{M}) \derive \mu(\bx_{M}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))
                \end{align*}
                since $|\eta|$ decrements by 1 (the first yield step $\nonterm(\bx_{S}) \yield (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-})$ is trimmed off). Indeed, in the $\CFG$, we have
                \begin{align*}
                    \nonterm(\bx_{M}) \otimes \nonterm(\bx_{S}) & \yield \; \nonterm(\bx_{M}) \otimes (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-}) \\
                    & = \; (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{M}) \otimes  \nonterm(\bx_{S^-})   \\
                    & \derive \; (R_N(\bx_N) \vdash \mu(\bx_{N^-})) \otimes \left( \mu(\bx_{M}) \otimes \formula(\bx_{S^-}) \right) \\
                    & = \; (R_N(\bx_N) \vdash \mu(\bx_{N^-})) \otimes \Rewrite(\nonterm(\bx_{M}) \derive  \mu(\bx_{M}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))
                \end{align*}
                (recall that we return \highlight{$(R_N(\bx_N) \vdash \mu(\bx_{N^-})) \otimes \Rewrite(\nonterm(\bx_{M}) \derive \mu(\bx_{M}) , \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}))$}). Moreover, $\nonterm_n(\bx_{M \cup S})$ derives this expression in $\CFG_n$ because 
                \begin{align*}
                    \nonterm_n(\bx_{ M \cup S}) \yield (R_N(\bx_N) \vdash \nonterm_n(\bx_{N^-}) ) \otimes \nonterm_n(\bx_{M \cup S^-}) \derive (R_N(\bx_N) \vdash \mu_n(\bx_{N^-}) ) \otimes \nonterm_n(\bx_{M \cup S^-}) \derive (R_N(\bx_N) \vdash \mu_n(\bx_{N^-}) ) \otimes \formula_n(\bx_{M \cup S^-}) .
                \end{align*}
                where \textcolor{orange}{(i) the first yield step here uses the production $\nonterm_n(\bx_{M \cup S}) ::= (R_N(\bx_N) \vdash \nonterm_n(\bx_{N^-})) \otimes \nonterm_n(\bx_{M \cup S^-})$, where $S = N \cup S^-$ and $N^- \subseteq N \in \{N \in \mE^- \mid n \notin N\}$}, (ii) the second step is valid because $\nonterm_n(\bx_{N^-}) \derive \mu_n(\bx_{N^-}) $ in $\CFG_n$ as $n \notin N^-$ and (iii) the last derivation follows from the induction hypothesis. 
            \item [(3.3)] (\autoref{alg:rewrite:3.3}) Lastly, if $\nonterm(\bx_{S}) \yield e$ (so $S = \emptyset$). In the $\CFG$, let $\nonterm(\bx_{M}) \yield \widetilde{\nonterm}(\bx_{M}) \otimes \nonterm(\bx_{\emptyset})$, where $\widetilde{\nonterm}(\bx_{M}) \derive \widetilde{\mu}(\bx_{M})$ and $\nonterm(\bx_{\emptyset}) \yield e_{\emptyset} \in \boldsymbol{D} \setminus \{\zerobf\}$, we have
            \begin{align*}
                \nonterm(\bx_{M}) \otimes \nonterm(\bx_{S}) & \yield \; \left(\widetilde{\nonterm}(\bx_{M}) \otimes \nonterm(\bx_{\emptyset})\right) \otimes e \\
                & \yield \; \left(\widetilde{\nonterm}(\bx_{M}) \otimes e_{\emptyset} \right) \otimes e \\
                & \derive \; (e \otimes  e_{\emptyset}) \otimes \widetilde{\mu}(\bx_{M})  && \text{ where } \mu(\bx_{M}) = \widetilde{\mu}(\bx_{M}) \otimes e_{\emptyset} \\
                & = \; (e \otimes  e_{\emptyset}) \otimes \Rewrite(\widetilde{\nonterm}(\bx_{M}) \derive \widetilde{\mu}(\bx_{M}), \nonterm(\bx_{\emptyset}) \yield \onebf)
            \end{align*}
            Recall that we return in this case \highlight{$e \otimes e_{\emptyset} \otimes \Rewrite(\widetilde{\nonterm}(\bx_{M}) \derive \widetilde{\mu}(\bx_{M}), \nonterm(\bx_{\emptyset}) \yield \onebf)$}. The yield step $\nonterm(\bx_{S}) \yield e$ is trimmed off, so $|\eta|$ decrements by 1 in the recursive call. 
            Moreover, $\nonterm_n(\bx_{M \cup S})$ derives this expression in $\CFG_n$ because
            \begin{align*}
                \nonterm_n(\bx_{M \cup S}) = \widetilde{\nonterm_n}(\bx_{M \cup S}) \otimes \nonterm_n(\bx_{\emptyset}) \yield \widetilde{\nonterm_n}(\bx_{M \cup S}) \otimes (e \otimes  e_{\emptyset})  \derive \widetilde{\mu_n}(\bx_{M}) \otimes (e \otimes  e_{\emptyset})  = \mu(\bx_{M}) \otimes e
            \end{align*}
            where \textcolor{orange}{the first yield step here uses the production $ \nonterm_n(\bx_{\emptyset}) ::= e \in \boldsymbol{D} \setminus \{\zerobf\}$ in $\CFG_n$}.
            \end{enumerate}
        \item [(4)] otherwise, $n$ is contained in the hyperedge in the next yield step of $\nonterm(\bx_{S})$. In this case, we apply a `stash' step that temporarily `stashes' this yield step into $\nonterm(\bx_{M})$ and then keep processing the next yield step of $\nonterm(\bx_{S})$.
            \begin{enumerate}
                \item [(4.1)] (\autoref{alg:rewrite:4.1}) $\nonterm(\bx_{S}) \yield  R_K(\bx_K) \otimes \nonterm(\bx_{S^-}) \derive R_K(\bx_K) \otimes \formula(\bx_{S^-})$, for some $K \in \mE^+, S^- \subseteq [n]$ such that $S = K \cup S^-$. Now $n \in K$. Let $\mu(\bx_{M \cup K})  = R_K(\bx_K) \otimes \mu(\bx_{M})$, we have
                \begin{align*}
                    \nonterm(\bx_{M}) \otimes \nonterm(\bx_{S}) & \yield \; \nonterm(\bx_{M}) \otimes R_K(\bx_K) \otimes \nonterm(\bx_{S^-}) \\
                    & \derive \; \mu(\bx_{M}) \otimes R_K(\bx_K) \otimes \formula(\bx_{S^-}) \\
                    &= \;  \mu(\bx_{M \cup K}) \otimes \formula(\bx_{S^-})
                \end{align*}
                We insert a new yield step for $R_K$ into the stashed derivation $\nonterm(\bx_{M}) \derive \mu(\bx_{M})$ and keep track of the largest hyperedge to be used as the next yield step of $\nonterm(\bx_{M})$ in the augmented derivation. W.L.O.G, the agumented derivation becomes
                $$
                \nonterm(\bx_{M \cup K}) \yield R_K(\bx_K) \otimes \nonterm(\bx_{M}) \derive R_K(\bx_K) \otimes \mu(\bx_{M}) = \mu(\bx_{M \cup K})
                $$
                and then we return \highlight{$\Rewrite \left(\nonterm(\bx_{M \cup K}) \derive \mu(\bx_{M \cup K}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}) \right)$}. 
                
                \item [(4.2)] (\autoref{alg:rewrite:4.2}) $\nonterm(\bx_{S}) \yield (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-}) \derive (R_N(\bx_N) \vdash \mu(\bx_{N^-})) \otimes \formula(\bx_{S^-}) $, for some $N \in \mE^-, N^- \subseteq N$, and $S^- \subseteq [n]$ such that $S = N \cup S^-$. Now $n \in N$. Let $\mu(\bx_{M \cup N})  = \left(R_N(\bx_N) \vdash \mu(\bx_{N^-}) \right) \otimes \mu(\bx_{M})$, we have
                    \begin{align*}
                        \nonterm(\bx_{M}) \otimes \nonterm(\bx_{S}) & \yield \; \nonterm(\bx_{M}) \otimes \left(R_N(\bx_N) \vdash \nonterm(\bx_{N^-}) \right) \otimes \nonterm(\bx_{S^-}) \\
                        & \derive \; \mu(\bx_{M}) \otimes \left(R_N(\bx_N) \vdash \mu(\bx_{N^-}) \right) \otimes \formula(\bx_{S^-}) \\
                        &= \;  \left[\left(R_N(\bx_N) \vdash \mu(\bx_{N^-}) \right) \otimes \mu(\bx_{M})\right] \otimes \formula(\bx_{S^-})  \\
                        &= \; \mu(\bx_{M \cup N}) \otimes \mu(\bx_{S^-})  
                    \end{align*}
                    $$
                    \nonterm(\bx_{M \cup N}) \yield \left(R_N(\bx_N) \vdash \nonterm(\bx_{N^-}) \right) \otimes \nonterm(\bx_{M}) \derive \left(R_N(\bx_N) \vdash \mu(\bx_{N^-}) \right) \otimes \mu(\bx_{M}) = \mu(\bx_{M \cup N}) 
                    $$
                    and then we return \highlight{$\Rewrite \left(\nonterm(\bx_{M \cup N}) \derive \mu(\bx_{M \cup N}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}) \right)$}. 
            \end{enumerate}
            Case (4) is the only if-else branch where $|\eta|$ stays the same in the recursive call, because this step essentially `stashes' the next yield step of $\nonterm(\bx_{S})$ into the  derivation for $\nonterm(\bx_{M})$. Therefore, the length of the derivation for $\formula(\bx_S)$ decrements by 1 but that of $\mu(\bx_M)$ increments by 1 in the recursive call. However, in the worst-case, this if-else branch can be visited at most $O(|\eta|)$ times, each visit incurs an $O(|\eta|)$ time overhead to place the yield step of $R_N$ into the stashed derivation $\nonterm(\bx_{M \cup N}) \derive \mu(\bx_{M \cup N})$ so that the largest hyperedge can be directly accessed upon request. Eventually, $\Rewrite$ will recurse back to one of the previous cases and $|\eta|$ will decrement by 1 in that subsequent recursive call. As a result, the correctness of the lemma in this case simply follows through from the correctness of $\Rewrite \left(\nonterm(\bx_{M \cup N}) \derive \mu(\bx_{M \cup N}), \nonterm(\bx_{S^-}) \derive \formula(\bx_{S^-}) \right)$. 
    \end{enumerate}
    % \hangdong{idea. stash for e, Rk, Rn, that has x + skipping if Rk, Rn has no x}
    Lastly, we justify that $\Rewrite$ runs in time $O(|\eta|^2 + d(n) \cdot \dbsize)$. The $\Rewrite$ algorithm recursively visits each yield step in both derivations $\nonterm(\bx_{M}) \derive \mu(\bx_{M})$ and $\nonterm(\bx_{S}) \derive \formula(\bx_{S})$ at most twice (accounting for ``stashes''). For each visit, if it does not fall into the last stash case (4), $|\eta|$ decrements by 1, and $\Rewrite$ takes $O(\dbsize)$ time to update the global database instance $\db$. Furthermore, every such update (on the database instance of $\db$) leverages the $\alpha$ or $\beta$ properties of the $\pn$-leaf $n$ to guarantee that $|\db_n| \leq |\db|$ and the update can only happen once for each hyperedge containing $n$ (since that corresponding factor does not appear in the subsequent recursive call). Thus, all updates leading to $\db_n$ take $O(d(n) \cdot \dbsize)$ time in total.
    
    For the last case (4), as discussed in paragraph of case (4), $\Rewrite$ can fall into it for at most $O(|\eta|)$ times, each time with a $O(|\eta|)$ time overhead before the next recursive call (for the `stashes'). Therefore, the total time complexity of $\Rewrite$ is $O(|\eta|^2 + d(n) \cdot \dbsize)$.
\end{proof}
    
The following theorem is a direct consequence of Lemma~\ref{lem:rewrite}.
\begin{theorem}
    \label{thm:rewrite}
    There is an algorithm that takes as input an $\nestfaqneg$ expression $\formula(\bx_{[n]})$ associated with $\mH$, thus recognized by $\CFG$ \eqref{def:cfg}, and a database instance $\db$, and then returns a $\nestfaqneg$ expression $\formula_n(\bx_{[n]})$ associated with $\mH_n$, thus recognized by $\CFG_n$ \eqref{eq:cfg_n}, and a new database instance $\db_n$ such that $\formula(\bx_{[n]}) = \formula_n(\bx_{[n]})$, $|\formula_n| \leq |\formula|$ and $|\db_n| \leq |\db|$. Moreover, the algorithm runs in time $O(|\formula|^2 + d(n) \cdot \dbsize)$, where $d(n)$ is the number of hyperedges containing $n$ in $\mH$.
\end{theorem}

\begin{proof}
    We simply call $\formula(\bx_{[n]}) = \formula_n(\bx_{[n]}) = \Rewrite \left(\nonterm(\bx_{\emptyset}) \yield \onebf, \nonterm(\bx_{[n]}) \derive \formula(\bx_{[n]}) \right)$ and trace the recursive call steps of $\Rewrite$ to construct the derivation $\nonterm_n(\bx_{[n]}) \derive \formula_n(\bx_{[n]})$ using production rules of $\CFG_n$ \eqref{eq:cfg_n}. As $\Rewrite$ (Algorithm~\ref{alg:rewrite}) only recurses on $\nonterm_n(\bx_S)$ where $n \in S$, and if not, it just follows from the original derivations in $\CFG$ (those derivations can be attached to the end of the derivation for every $\nestfaqneg$ subexpression $\nonterm_n(\bx_S) \derive \formula_n(\bx_S)$ where $n \notin S$). We therefore close the proof by invoking Lemma~\ref{lem:rewrite}. 
\end{proof}




\subsection{The aggregation algorithm} \label{sec:aggregation}
We assume in this section that we have obtained $(\formula_n(\bx_{[n]}), \db_n)$ from the call of $\Rewrite$ as in Theorem~\ref{thm:rewrite}. We now shift our focus directly to the aggregation algorithm that eliminates $x_n$, where $n$ is the $\pn$-leaf of the signed hypergraph $\mH$. We defer the oracle-construction algorithm to Appendix~\ref{sec:oracle} for now because the aggregation algorithm will provide an intuitive motivation that necessitates the oracles to be constructed.

The aggregation algorithm takes as input $\formula_n(\bx_{[n]})$ recognized by $\CFG_n$ \eqref{eq:cfg_n} and a database instance $\db_n$ and returns a new $\nestfaqneg$ expression $\formula_{n-1}(\bx_{[n-1]})$ recognized by $\CFG_{n-1}$ \eqref{eq:cfg_n-1}, and a corresponding database instance $\db_{n-1}$ such that $\bigoplus_{x_n \in \dom(x_n)}\formula_n(\bx_{[n]}) = \formula_{n-1}(\bx_{[n-1]})$. As a recap, the production rules of $\CFG_n$ are: for all $S \subseteq [n]$,
\begin{align}
    \qquad \qquad \nonterm_n(\bx_{\emptyset}) &::= \; e  
    && \text{ where } S = \emptyset \text{ and } e \in \boldsymbol{D} \setminus \{\zerobf\}\label{eq:cfg_n:rule1} \\
    \qquad \qquad \nonterm_n(\bx_{S}) &::= \; R_U(\bx_U)
    && \text{ where } S = U \label{eq:cfg_n:rule2} \\
    & \; \; \mid \; R_K(\bx_K) \otimes \nonterm_n(\bx_{S^-})
    && \text{ where } S = K \cup S^- \text{ and } K \in \{K \in \mE^+ \mid n \notin K\}  \label{eq:cfg_n:rule3} \\
    \qquad \qquad & \; \; \mid \; (R_{N}(\bx_{N}) \vdash \nonterm_n(\bx_{N^-}))
    && \text{ where } S = N \text{ and }  N^- \subseteq N \in \{N \in \mE^- \mid n \in U \subset N \} \label{eq:cfg_n:rule4} \\
    \qquad \qquad & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_n(\bx_{N^-})) \otimes \nonterm_n(\bx_{S^-})
    && \text{ where } S = N \cup S^- \text{ and } N^- \subseteq N \in \{N \in \mE^- \mid n \notin N\} \label{eq:cfg_n:rule5} 
\end{align}

The main upside of turning the $\nestfaqneg$ expression $\formula(\bx_{[n]})$ (recognized by $\CFG$) into $\formula_n(\bx_{[n]})$ (recognized by $\CFG_n$) is that the productions of $\CFG_n$ are layed out in a principled way: $x_n$ is only contained in one terminal (or non-terminal). From an $\AST$ standpoint, after refactoring, $x_n$ only resides in at most one subtree at every intermediate $\bigotimes$ node. 


We safely assume that $R_{N_k}, R_{N_{k-1}}, \cdots, R_{N_1}, R_U$ are the only factors of $\formula_n(\bx_{[n]})$ that contain $x_n$ in $\formula_n(\bx_{[n]})$ and $N_k \supseteq N_{k-1} \supseteq \cdots \supseteq N_1 \supseteq U$ (we let $N_0 = U$ for convenience), gifted by the $\beta$-property of the $\pn$-leaf $n$. A convenient way to derive $\formula_n(\bx_{[n]})$ in $\CFG_n$ is as follows (let $N_{i} \supseteq N^-_{i} = S_{i-1} \cup N_{i-1}$ for $i \in [k]$)
\begin{equation} \label{eq:derivation}
    \begin{aligned}
        \nonterm_n(\bx_{[n]}) & \derive \formula_n(\bx_{S_k}) \otimes \nonterm_n(\bx_{N_k})  \\
    & \yield \formula_n(\bx_{S_k}) \otimes \left( R_{N_k}(\bx_{N_k}) \vdash \nonterm_n(\bx_{N^-_k}) \right) \\
    & \derive \formula_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \nonterm_n(\bx_{N_{k-1}}) \right) \\
    & \yield \formula_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1}}(\bx_{N_{k-1}}) \vdash \nonterm_n(\bx_{N^-_{k-1}}) \right) \right) \\
    & \; \vdots \\
    & \yield \formula_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1}}(\bx_{N_{k-1}}) \vdash  \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash\left(\formula_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \nonterm_n(\bx_{N^-_1})) \right) \cdots  \right) \right)   \\
    & \derive \formula_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1}}(\bx_{N_{k-1}}) \vdash \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash \left(\formula_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \formula_n(\bx_{S_{0}}) \otimes \nonterm_n(\bx_U)) \right) \cdots  \right) \right) \\
    & \yield \formula_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1}}(\bx_{N_{k-1}}) \vdash \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash \left(  \formula_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \formula_n(\bx_{S_{0}}) \otimes R_U(\bx_U)) \right)  \cdots   \right) \right) \\
    & = \; \formula_n(\bx_{[n]})
    \end{aligned}
\end{equation}
where every $\derive$ (a derive step) in \eqref{eq:derivation} applies the productions \eqref{eq:cfg_n:rule1}, \eqref{eq:cfg_n:rule3} and \eqref{eq:cfg_n:rule5} to factor out all the terms ($e, R_K(\bx_K)$ or $R_N(\bx_N) \vdash \nonterm_n(\bx_{N^-})$) that does not contain $x_n$ and wrap them in some $\formula_n(\bx_{S_i})$ such that $\nonterm_n(\bx_{S_i}) \derive \formula_n(\bx_{S_i})$, where $i \in [k]$ and $n \notin S_i$. Then it is followed by $\yield$ (a yield step) that applies the production \eqref{eq:cfg_n:rule4} that produces the negative factors $R_{N_k}, R_{N_{k-1}}, \cdots, R_{N_1}$ from $\nonterm_n(\bx_{N_k}), \nonterm_n(\bx_{N_{k-1}}), \cdots, \nonterm_n(\bx_{N_1})$, except for the last yield step where we use the production \eqref{eq:cfg_n:rule2} to produce the pivot factor $R_U(\bx_U)$ from $\nonterm_n(\bx_U)$.


On a high level, our aggregation algorithm will follow the derivation \eqref{eq:derivation} of $\formula_n(\bx_{[n]})$ line-by-line and ``push-in'' the aggregation operator $\bigoplus_{x_n \in \dom(x_n)}$ into the more and more nested subexpressions. For succinctness, we use $\bigoplus_{x_n}$ as an abbreviation of $\bigoplus_{x_n \in \dom(x_n)}$ in the following. This ``push-in'' step for every derive step is immediate: we can simply push the aggregation operator $\bigoplus_{x_n}$ by factoring out the term $\formula_n(\bx_{S_i})$ that does not contain $x_n$. That is, for $i = 0, 1, \ldots, k$,
\begin{align*}
    \bigoplus_{x_n} \formula_n(\bx_{S_i}) \otimes \left(R_{N_i}(\bx_{N_i}) \vdash \formula_n(\bx_{N^-_{i}})  \right) & = \formula_n(\bx_{S_i}) \otimes \bigoplus_{x_n}  \left(R_{N_i}(\bx_{N_i}) \vdash \formula_n(\bx_{N^-_{i}})  \right) \\
    \bigoplus_{x_n} \formula_n(\bx_{S_0}) \otimes R_U(\bx_U) & = \formula_n(\bx_{S_0}) \otimes \bigoplus_{x_n} R_U(\bx_U) \\
    & = \formula_n(\bx_{S_0}) \otimes R_{U \setminus \{n\}}(\bx_{U \setminus \{n\}}) 
\end{align*}
Here, in the last yield step (applying the production \eqref{eq:cfg_n:rule2}), $\bigoplus_{x_n} R_U(\bx_U)$ is straightforward: we can scan the list representation of the pivot factor $R_U$ once and get a new factor $R_{U \setminus \{n\}}(\bx_{U \setminus \{n\}})$ in time $O(|R_U|)$. 

Now we turn to the tricky yield steps in the derivation \eqref{eq:derivation} that applies the production \eqref{eq:cfg_n:rule4} of the $\CFG_n$. What we want here is to ``push-in'' the aggregation operator $\bigoplus_{x_n}$ after the $\vdash$ operator so that the aggregation algorithm can proceed with the subexpression $\formula_n(\bx_{N^-})$. To that end, first we recall the semantics of the $\vdash$ operator: 
\begin{equation*}
    \bigoplus_{x_n} R_N(\bx_N) \vdash \formula_n(\bx_{N^-})  = \bigoplus_{x_n} \left( R_N(\bx_N) \oplus \indicator{\neg R_N}(\bx_N) \otimes \formula_n(\bx_{N^-}) \right).
    % R_{N \setminus \{n\}}(\bx_{N \setminus \{n\}}) \vdash \bigoplus_{x_n}  \nonterm_n(\bx_{N^-})
\end{equation*}
We distinguish the following two disjoint cases:
\begin{enumerate}
    \item if $\ba_{N \setminus \{n\}} \notin \Pi_{N \setminus \{n\}} R_N$, then the aggreation simply becomes $\bigoplus_{x_n} \formula_n(\bx_{N^-})$, because $R_N(x_n, \ba_{N \setminus \{n\}}) = \zerobf$ and $\indicator{\neg R_N}(x_n, \ba_{N \setminus \{n\}}) = \onebf$, for all $x_n \in \dom(x_n)$. Thus, for such tuples $\ba_{N \setminus \{n\}}$, the push-in step is trivial.
    \item otherwise, we have $\ba_{N \setminus \{n\}} \in \Pi_{N \setminus \{n\}} R_N(\bx_N)$. In this case, we define a new factor $R_{N \setminus \{n\}}$ as follows:
    \begin{align*}
        R_{N \setminus \{n\}}(\ba_{N \setminus \{n\}})  = 
        \begin{cases} \bigoplus_{x_n} R_N({x_n, \ba_{N \setminus \{n\}}}) \oplus \indicator{\neg R_N}({x_n, \ba_{N \setminus \{n\}}}) \otimes \formula_n({x_n, \ba_{N^- \setminus \{n\}}}) & \text { if } \ba_{N \setminus \{n\}} \in \Pi_{N \setminus \{n\}} R_N(\bx_N) \\ \zerobf & \text { otherwise. } \end{cases}
    \end{align*}
    It is easy to see that the list representation of $R_{N \setminus \{n\}}$ is of size $O(|R_N|)$.
\end{enumerate}
Therefore, if we can obtain (the list representation of) this new factor $R_{N \setminus \{n\}}$ efficiently, the ``push-in'' of the aggregation operator becomes immediate because
\begin{align*}
    \bigoplus_{x_n} \formula_n(\bx_{N}) & = \bigoplus_{x_n} \left( R_N(\bx_N) \vdash \formula_n(\bx_{N^-}) \right) \\
    & = \bigoplus_{x_n} \left( R_N(\bx_N) \oplus \indicator{\neg R_N}(\bx_N) \otimes \formula_n(\bx_{N^-}) \right) \\
    & = R_{N \setminus \{n\}}(\bx_{N \setminus \{n\}}) \oplus \indicator{\neg R_{N \setminus \{n\}}}(\bx_{N \setminus \{n\}}) \otimes \bigoplus_{x_n}  \formula_n(\bx_{N^-}) \\
    & = R_{N \setminus \{n\}}(\bx_{N \setminus \{n\}}) \vdash \bigoplus_{x_n}  \formula_n(\bx_{N^-}) 
\end{align*}

Back to our big picture, the aggregation step ``pushes-in'' the aggregation operator $\bigoplus_{x_n}$ one line at a time following the derivation \eqref{eq:derivation}:
\begin{equation} \label{eq:derivation-aggregate}
    \begin{aligned}
        \bigoplus_{x_n} \formula_n(\bx_{[n]}) & = \formula_n(\bx_{S_k}) \otimes \bigoplus_{x_n} \formula_n(\bx_{N_k})  \\
        & = \formula_n(\bx_{S_k}) \otimes \left( R_{N_k \setminus \{n\}}(\bx_{N_k \setminus \{n\}}) \vdash \bigoplus_{x_n} \formula_n(\bx_{N^-_k}) \right) \\
        & = \formula_n(\bx_{S_k}) \otimes \left(R_{N_k \setminus \{n\}}(\bx_{N_k \setminus \{n\} } ) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \bigoplus_{x_n} \formula_n(\bx_{N_{k-1}}) \right) \\
        & = \formula_n(\bx_{S_k}) \otimes \left(R_{N_k\setminus \{n\}}(\bx_{N_k \setminus \{n\} }) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1} \setminus \{n\} }(\bx_{N_{k-1} \setminus \{n\} }) \vdash \bigoplus_{x_n}  \formula_n(\bx_{N^-_{k-1}}) \right) \right) \\
        & \; \vdots \\
        & = \formula_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \left(  \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash\left(\formula_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \bigoplus_{x_n} \formula_n(\bx_{N^-_1})) \right) \cdots  \right) \right)   \\
        & = \formula_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \left( \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash \left(\formula_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \formula_n(\bx_{S_{0}}) \otimes \bigoplus_{x_n} \formula_n(\bx_U)) \right) \cdots  \right) \right) \\
        & = \formula_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{S_{k-1}}) \otimes \left( \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash \left(  \formula_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \formula_n(\bx_{S_{0}}) \otimes \bigoplus_{x_n} R_U(\bx_U)) \right)  \cdots   \right) \right) \\
        & =: \formula_{n-1}(\bx_{[n-1]})
    \end{aligned}
\end{equation}

As one can see from the comparison with \eqref{eq:derivation}, the derivation of $\formula_{n-1}(\bx_{[n-1]})$ exactly follows the derivation of $\formula_{n}(\bx_{[n]})$ except that $x_n$ has been peeled off from the set of variables and every $\nestfaqneg$ subexpression show up in $\formula_{n}(\bx_{[n]})$. So, $\formula_{n-1}(\bx_{[n-1]})$ is a $\nestfaqneg$ expression recognized by the following intermediate context-free grammar, obtained by directly removing $x_n$ from every non-terminal of the grammar $\CFG_n$: for all $S \subseteq [n-1]$,
\begin{align*}
        \nonterm_{n-1}(\bx_{\emptyset}) &::= \; e  
        && \text{ where }  S = \emptyset \text{ and } e \in \boldsymbol{D} \setminus \{\zerobf\}   \\
        \nonterm_{n-1}(\bx_{S \setminus \{n\}}) &::= \; R_{U \setminus \{n\}}(\bx_{U \setminus \{n\}}) 
        && \text{ where } S = U \\
        & \; \; \mid \; R_{K}(\bx_{K}) \otimes \nonterm_{n-1}(\bx_{S^- \setminus \{n\}})  \label{eq:nonterm-1}
        && \text{ where } S = K \cup S^- \text{ and } K \in \{K \in \mE^+ \mid n \notin K\}   \\
        & \; \; \mid \; (R_{N \setminus \{n\}}(\bx_{N \setminus \{n\}}) \vdash \nonterm_{n-1}(\bx_{N^- \setminus \{n\}}))
        && \text{ where } S = N \setminus \{n\} \text{ and } N^-  \subseteq N \in \{N \in \mE^-  \mid n \in U \subset N \}  \\
        & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_{n-1}(\bx_{N^-})) \otimes \nonterm_{n-1}(\bx_{S^- \setminus \{n\}}) 
        && \text{ where } S = N \cup S^- \text{ and } N^- \subseteq N \in \{N \in \mE^- \mid n \notin N\} 
\end{align*}


% \begin{equation} 
%     \begin{aligned}
%         \CFG_{n-1} \qquad \qquad \; \\
%         \text{ for all } S \subseteq [n-1], \\
%             \nonterm_{n-1}(\bx_{\emptyset}) &::= \; e  
%             && \text{ where } S = \emptyset \text{ and } e \in \boldsymbol{D} \setminus \{\zerobf\}  \\
%             \nonterm_{n-1}(\bx_{S}) &::= \; R_K(\bx_K) \otimes \nonterm_{n-1}(\bx_{S^-}),  
%             && \text{ where } S = K \cup S^- \text{ and } K \in \mE^+_{n-1}, S^- \subseteq S  \\
%             & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_{n-1}(\bx_{N^-})) \otimes \nonterm_{n-1}(\bx_{S^-}), 
%             && \text{ where } S = N \cup S^-, N^- \subseteq N \in \mE^-_{n-1} \text{ and } S^- \subseteq S 
%     \end{aligned}
% \end{equation}

In spite of its discrepencies to $\CFG_{n-1}$ \eqref{eq:cfg_n-1}, every production of the above grammar can be derived from $\CFG_{n-1}$. Indeed, recall that $\CFG_{n-1}$ is associated with the signed hypergraph $\mH_{n-1} = \removeleaf{\mH}{n} = ([n-1], \mE_{n-1}^+, \mE_{n-1}^-)$. Then, $U \setminus \{n\} \in \mE_{n-1}^+$, $\{K \in \mE^+ \mid n \notin K\} \subseteq \mE_{n-1}^+$ and $\{N \setminus \{n\} \mid N \in \mE^-, n \notin N \vee n \in U \subset N  \}  \subseteq \mE_{n-1}^-$. Therefore, the $\nestfaqneg$ expression $\formula_{n-1}(\bx_{[n-1]})$ is also recognized by $\CFG_{n-1}$ at the end of the elimination step for the $\pn$-leaf $n$ and the $\pn$-elimination step for $n$ now completes.


The only missing (and tricky) piece is how to compute the list representation of the new factor $R_{N \setminus \{n\}}$ efficiently. In the next section, we will introduce an efficient algorithm for this task using \textsf{RangeSum} data structures and it then to the following main theorem. Its proof is deferred to Appendix~\ref{sec:putting_things_together}, after the introduction of \textsf{RangeSum} data structures.

\begin{theorem} \label{thm:aggregation-main}
    Let $\mH_n$ be a signed hypergraph with a $\pn$-leaf $n$. Let $\formula_n(\bx_{[n]})$ be a $\nestfaqneg$ expression associated with $\mM_n$ (thus recognized by $\CFG_n$ \eqref{eq:cfg_n}) and $\db_n$ be its database instance. There is an (aggregation) algorithm that takes $(\formula_n(\bx_{[n]}), \db_n)$ as input and outputs $(\formula_{n-1}(\bx_{[n-1]}), \db_{n-1})$ where
    \begin{enumerate}
        \item $\formula_{n-1}(\bx_{[n-1]})$ is the $\nestfaqneg$ expression associated with $\mH_{n-1} = \removeleaf{\mH}{n}$ obtained by directly peeling off in $x_n$ from $\formula_n(\bx_{[n]})$, thus it is recognized by $\CFG_{n-1}$ \eqref{eq:cfg_n-1} and $|\formula_{n-1}| = O(|\formula_n|)$,
        \item $\db_{n-1}$ is a database instance of $\formula_{n-1}(\bx_{[n-1]})$ such that $\bigoplus_{x_n \in \dom(x_n)}\formula_n(\bx_{[n]}) = \formula_{n-1}(\bx_{[n-1]})$ and $|\db_{n-1}| = O(|\db_n|)$.
    \end{enumerate}
    and the algorithm runs in $O(|\formula_n| + d(n) \cdot |\db_n| \cdot \ackfunc{\db_n})$ time, where $d(n)$ is the number of hyperedges containing $n$ in $\mH_n$.
\end{theorem}

\highlight{The inverse Ackermann factor $\ackfunc{\db_n}$ in the aggregation algorithm is inherited from the algorithm supporting \textsf{RangeSum} queries. Thus, the guarantee of the \textsf{RangeSum} problem carries over to our aggregation algorithm: for semigroups that accepts additive inverse, or for the semigroup with minimum (or maximum) as the operation (\textsf{RMQ} as in \cite{GBT84}), the aggregation algorithm runs in $O(|\formula_n| \cdot |\db_n|)$ time, without the additional inverse Ackermann overhead.}


\subsection{The oracle-construction algorithm} \label{sec:oracle}
\myparagraph{\textsf{RangeSum}} Chazelle and Rosenberg \cite{10.1145/73833.73848} studied the range query problem \textsf{RangeSum} in the semigroup model defined as follows. Preprocess a array $A$ of $\arraysize$ elements from a semigroup $\bS = (\boldsymbol{D}, \oplus)$, and then support the following query: given a query range $[\open, \close]$, return the range sum $\bigoplus_{\interval \in [\open, \close]} A[\interval]$, i.e. $\bigoplus_{\open \leq \interval \leq \close} A[\interval]$. In particular, they proved the following theorem.

\begin{theorem}[\cite{10.1145/73833.73848}] \label{thm:range-sum}
	There is a data structure of size $O(\arraysize)$ that works in the word RAM, and support a \textsf{RangeSum} query in $O(\alpha(14 \arraysize, \arraysize))$ time, where $\alpha$ is the inverse Ackermann function, after spending $O(\arraysize)$ preprocessing time. 
\end{theorem}
It is the absence of additive inverse for general semirings that results in the hardness of $\mathsf{RangeSum}$ and an unconditional hard instance can be recursively constructed that mimics the definition of the inverse Ackermann function $\alpha(\cdot, \cdot)$ as in~\cite{10.1145/73833.73848}. It is easy to see that \textsf{RangeSum} queries can be answered in $O(1)$ time after $O(\arraysize)$ preprocessing, if the underlying semigroup $\bS$ allows for additive inverse: one candidate algorithm can precompute the partial sums $\bigoplus_{\interval \in [1, \close]} A[\interval]$ and represent each \textsf{RangeSum} query $[\open, \close]$ as the semigroup sum of $\bigoplus_{ \interval \in [1, \close]} A[\interval]$ and the additive inverse of $\bigoplus_{\interval \in [1, \open-1]} A[\interval]$.  

The \textsf{RangeSum} problem with minimum as the semigroup operation, is studied intensively and typically known as \textsf{RangeMinimumQuery} (\textsf{RMQ}). In their influential paper \cite{GBT84}, Gabow, Bentley and Tarjan shown that there is an algorithm that works in the word RAM and supports a \textsf{RMQ} query in $O(1)$ time, after spending $O(\arraysize)$ preprocessing time and space. They recognized the Cartesian tree as the instrumental data structure that was introduced by Vuillemin \cite{Vuillemin80} in the context of average time analysis of searching.

% \cite{BerlinHeidelberg}, Bender and Farach-Colton that there is an algorithm that works in the word RAM and supports a \textsf{RMQ} query in $O(1)$ time, after spending $O(\arraysize)$ preprocessing time and space, using Cartesian tree as an instrumental data structure. The first optimal \textsf{RangeMinimumQuery} structure is due to Harel and Tarjan \cite{10.1137/0213024} in the context of the Level Ancestor Problem.

In this section, we introduce a key oracle (called \textsf{RangeSumOrcale}) that supports efficient computation of the new negative factors $R_{N \setminus \{n\}}$ in the aggregation algorithm introduced in \eqref{eq:derivation-aggregate} of the last section. In particular, \textsf{RangeSumOrcale} uses the \textsf{RangeSum} data structures as a black-box, thus inherits the inverse Ackermann factor of Theorem~\ref{thm:range-sum} under general semirings. We first introduce the following definition.

\medskip
\myparagraph{\textsf{RangeSumOracle}}
Let $A$ be an an array of size $\arraysize$ over a semigroup $\bS = (\boldsymbol{D}, \oplus)$, where we implicitly assume that $A[\interval] = \zerobf$ if $\interval \notin [1, \arraysize]$. An \emph{array decomposition} of $A$ is an array of pairs as follows:
\begin{align*}
    \left([1, \interval_1], \bigoplus_{\interval \in [1, \interval_1]} A[\interval] \right), \;
    \left([\interval_1 + 1, \interval_2], \bigoplus_{\interval \in [\interval_1 + 1, \interval_2]} A[\interval] \right), \;
    \ldots, 
    \left([\interval_r + 1, \arraysize], \bigoplus_{\interval \in [\interval_p + 1, \arraysize]} A[\interval] \right), \;
    \left([w+1, \bot], \zerobf \right)
\end{align*}
where $1 \leq \interval_1 \leq \interval_2 \leq \cdots \leq \interval_{p} = \arraysize$ ($\interval_i$, where $i \in [p]$, and $0, \bot$, are called the \emph{break points} of the array decomposition) and  
each pair contains a range and a semigroup sum over that range. For convenience, we add a dummy pair $([w + 1, \bot], \zerobf)$ indicating the end of the array decomposition. A \emph{trivial} array decomposition of $A$ is the array of pairs 
\begin{align*}
    \left([1, 1], A[1] \right), \;
    \left([2, 2], A[2] \right), \;
    \ldots,
    \left([\arraysize, \arraysize], A[\arraysize] \right), \;
    \left([w+1, \bot], \zerobf \right).
\end{align*}
whose set of break points is $\{1, 2, \ldots, \arraysize\}$.

An $\RangeSumOracle$ of the array $A$ is a $\RangeSum$ data structure built on an array decomposition of $A$ such that: given a query range $[\interval_i + 1, \interval_j]$, where $\interval_i < \interval_j$ are two break points of the array decomposition (so that the query range aligns with the smaller range sums stored in the array decomposition), it returns the range sum over the query range
$$
\bigoplus_{i \leq k < j }  \bigoplus_{\interval \in [\interval_k + 1, \interval_{k+1}]} A[\interval] = \bigoplus_{\interval \in [\interval_i + 1, \interval_j]} A[\interval]
$$
It is easy to see from \autoref{thm:range-sum} that there is a data structure of size $O(\arraysize)$ and support a $\RangeSumOracle$ query in $O(\alpha(14 \arraysize, \arraysize))$ time, where $\alpha(\cdot, \cdot)$ is the inverse Ackermann function, after spending $O(\arraysize)$ preprocessing time.
Indeed, for a trivial array decomposition, the $\RangeSumOracle$ is essentially a $\RangeSum$ data structure of $A$. 



\medskip
Now we formally describe our $\RangeSumOracle$(s). To better identify $\nestfaqneg$ subexpressions show up in $\formula_n(\bx_{[n]})$, we let $\nonterm_n(\bx_{N_i}) \derive \formula_n(\bx_{N_i})$ for $n \in U = N_0 \subseteq N^-_1 \subseteq N_1 \subseteq \cdots \subseteq N^-_k \subseteq N_k$ and $\nonterm_n(\bx_S) \derive \mu_n(\bx_S)$ for all $n \notin S \subseteq [n]$. Then, \eqref{eq:derivation} can be equivalently written as:

\begin{equation} \label{eq:derivation-oracle}
    \begin{aligned}
    \formula_n(\bx_{[n]}) & = \mu_n(\bx_{S_k}) \otimes \formula_n(\bx_{N_k})  \\
    & = \mu_n(\bx_{S_k}) \otimes \left( R_{N_k}(\bx_{N_k}) \vdash \formula_n(\bx_{N^-_k}) \right) \\
    & = \mu_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \mu_n(\bx_{S_{k-1}}) \otimes \formula_n(\bx_{N_{k-1}}) \right) \\
    & = \mu_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \mu_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1}}(\bx_{N_{k-1}}) \vdash \formula_n(\bx_{N^-_{k-1}}) \right) \right) \\
    & \; \vdots \\
    & = \mu_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \mu_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1}}(\bx_{N_{k-1}}) \vdash  \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash\left(\mu_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \formula_n(\bx_{N^-_1})) \right) \cdots  \right) \right)   \\
    & = \mu_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \mu_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1}}(\bx_{N_{k-1}}) \vdash \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash \left(\mu_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \mu_n(\bx_{S_{0}}) \otimes \formula_n(\bx_U)) \right) \cdots  \right) \right) \\
    & = \mu_n(\bx_{S_k}) \otimes \left(R_{N_k}(\bx_{N_k}) \vdash \mu_n(\bx_{S_{k-1}}) \otimes \left(R_{N_{k-1}}(\bx_{N_{k-1}}) \vdash \cdots R_{N_{1}}(\bx_{N_{1}}) \vdash \left(  \mu_n(\bx_{S_1}) \otimes (R_{N_{1}}(\bx_{N_{1}}) \vdash \mu_n(\bx_{S_{0}}) \otimes R_U(\bx_U)) \right)  \cdots   \right) \right) 
    \end{aligned}
\end{equation}
We will construct a $\RangeSumOracle$ for the $\nestfaqneg$ subexpression $\formula_n(\bx_{U})$ (let $U = N_0$) and then $\formula_n(\bx_{N_1}), \formula_n(\bx_{N_2}), \ldots, \formula_n(\bx_{N_k})$, in a bottom-up order as layed out in \eqref{eq:derivation-oracle}. Indeed, the $\BuildOracle$ algorithm described in Algorithm~\ref{alg:oracle} takes as input the $\nestfaqneg$ expression $\formula_n(\bx_{[n]})$ recognized by $\CFG_n$ and the corresponding database instance $\db_n$ and returns a $\RangeSumOracle$ for the every $\nestfaqneg$ subexpression $\formula_n(\bx_{N_i})$, where $i = 0, 1, \ldots, k$. Now we walk through its steps, starting from the inner-most $\formula_n(\bx_{U}) = R_U(\bx_U)$ in \eqref{eq:derivation-oracle}, $R_U$ being the pivot factor. 


\begin{algorithm}
    \caption{$\BuildOracle(\formula_n(\bx_{[n]}), \db_n)$} \label{alg:oracle}
    \KwIn{a $\nestfaqneg$ expression $\formula_n(\bx_{[n]})$ recognized by $\CFG_n$ and a global database instance $\db_n$}
    \KwOut{An $\RangeSumOracle$ $\Oracle_i(\bx_{N_i \setminus \{n\}})$ for each $\formula_n(\bx_{N_i})$, where $i = 0, 1, \ldots, k$ and $U = N_0 \subseteq N_1 \subseteq \cdots \subseteq N_k$ are the only hyperedges containing $n$}

    \ForEach(\Comment{base case for $\formula_n(\bx_U)$} \label{line:oracle-base-start}
    ){$\ba_{U \setminus \{n\}} \in \bigcup_{0 \leq i \leq k} \Pi_{U \setminus \{n\}} R_{N_i}$}{
         \textbf{init} $A_0(\ba_{U \setminus \{n\}}) \gets []$, $\Oracle_0(\ba_{U \setminus \{n\}}) \gets []$, $\interval_{\ba_{U \setminus \{n\}}} \gets 1$ \\
    }
    
    \ForEach{$\ba_{U} \in \bigcup_{0 \leq i \leq k} \Pi_{U} R_{N_i}$}{
        $A_0(\ba_{U \setminus \{n\}})[\interval_{\ba_{U \setminus \{n\}}}] \gets \Pi_{\{n\}} \ba_{U}$ \\
        % \textbf{append} $\Pi_{\{n\}} \ba_{U}$ \textbf{to} $A_0(\ba_{U \setminus \{n\}})$ \\
        \textbf{append} $\left([\interval_{\ba_{U \setminus \{n\}}}, \interval_{\ba_{U \setminus \{n\}}}], R_U(\ba_{U}) \right)$ \textbf{to} $\Oracle_0(\ba_{U \setminus \{n\}})$ \\
        $\interval_{\ba_{U \setminus \{n\}}} \gets \interval_{\ba_{U \setminus \{n\}}} + 1$ \\
    }
    \ForEach{$\ba_{U \setminus \{n\}} \in \bigcup_{0 \leq i \leq k} \Pi_{U \setminus \{n\}} R_{N_i}$}{
        \textbf{append} $\left([\interval_{\ba_{U \setminus \{n\}}} + 1, \bot], \; \zerobf \right)$ \textbf{to} $\Oracle_0(\ba_{U \setminus \{n\}})$ \label{line:oracle-base-end} \\
        \textbf{construct} $\RangeSum$ data structures \textbf{on} $\Oracle_0(\ba_{U \setminus \{n\}})$ \\
    }
    
    \ForEach(\Comment{inductive case for $\formula_n(\bx_{N_i})$}){$i = 1, 2, \ldots k$ (in order) \label{line:oracle-inductive}}{
        \ForEach{$\ba_{N_i \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_i \setminus \{n\}} R_{N_s}$}{ 
            \textbf{init} $\Oracle_i(\ba_{N_i \setminus \{n\}}) \gets []$, $\open_{\ba_{N_i \setminus \{n\}}} \gets 0$  \\
        }
        
        \ForEach{$\ba_{N_{i-1} \setminus \{n\}} \in \bigcup_{i-1 \leq s \leq k} \Pi_{N_{i-1} \setminus \{n\}} R_{N_s} $}{
            $\close \gets 1$ \\
            \While{$\close \neq \bot$ }{
                $a_n \gets A_0(\Pi_{U \setminus \{n\}}\ba_{N_{i-1} \setminus \{n\}})[\close]$ \\
                \ForEach{$\ba_{N_i \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_{i} \setminus \{n\}} R_{N_s}(a_n, \ba_{N_{i-1} \setminus \{n\}}, \bx_{N_s \setminus N_{i-1}})  $}{
                    %% implicit hashtable here
                    % $\mathsf{hash}(\bx_{N_{i-1}}, \bx_{N_{i} \setminus N_{i-1}}) \gets \Pi_{N_{i} \setminus \{n\}} R_{N_s}(x_n, \bx_{N_{i-1} \setminus \{n\}}, \bx_{N_s \setminus N_{i-1}})$
                    $M_1 \gets \bigoplus_{\interval \in [\open_{\ba_{N_i \setminus \{n\}}} + 1, \close -1]}\formula_n \left(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval],  \ba_{N_{i-1} \setminus\{n\}} \right)$ \label{line:oracle-set-breakpt-true-start} \\
                    $M_2 \gets \formula_n(a_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})$ \\
                    \textbf{append} 
                    $\left( [\open_{\ba_{N_i \setminus \{n\}}} + 1, \close -1 ], \; \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes M_1 \right)$ \textbf{to} $\Oracle_i(\ba_{N_i \setminus \{n\}})$ \\
                    \textbf{append} 
                    $\left( [\close, \close], \; R_{N_i}(a_n, \ba_{N_i \setminus \{n\}}) \oplus \indicator{\neg R_{N_i} } (a_n, \ba_{N_i \setminus \{n\}}) \otimes \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes M_2 \right)$ \textbf{to} $\Oracle_i(\ba_{N_i \setminus \{n\}})$   \label{line:oracle-set-breakpt-true-end}  \\
                    $\open_{\ba_{N_i \setminus \{n\}}} \gets \close + 1$ \\
                }
                \textbf{move} $\close$ to the next break point of $\Oracle_{i-1}(\ba_{N_{i-1} \setminus \{n\}})$ \\
            }
        }
        \ForEach{$\ba_{N_i \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_i \setminus \{n\}} R_{N_s}$}{
            \textbf{append} $([\open_{\ba_{N_i \setminus \{n\}}} + 1, \bot], \; \zerobf)$ into $\Oracle_i(\ba_{N_i \setminus \{n\}} )$ \\
            \textbf{construct} $\RangeSum$ data structures \textbf{on} $\Oracle_i(\ba_{N_i \setminus \{n\}} )$ \\
        }
    }
    \Return $\left(\Oracle_i(\bx_{N_i \setminus \{n\}})\right)_{i = 0, 1, \ldots, k}$
\end{algorithm}

\medskip
\introparagraph{\textcolor{blue}{the base case of $\formula_n(\bx_{U}) = R_U(\bx_U)$}}
The base case first sets up the indices for accessing all $x_n$ values for $\RangeSum$ data structures constructed later. More precisely, we first build a hashtable $A_0(\bx_{U \setminus \{n\}})$ from $\bigcup_{0 \leq i \leq k} \Pi_{U} R_{N_i}$, where $\bx_{U \setminus \{n\}}$ is its key and each entry $\bx_{U \setminus \{n\}} = \ba_{U \setminus \{n\}} \in \Oracle_0(\bx_{U \setminus \{n\}})$ stores an array of $x_n$ values where $(x_n, \ba_{U \setminus \{n\}}) \in \bigcup_{0 \leq i \leq k} \Pi_{U} R_{N_i}$. The array is identified as $A_0(\ba_{U \setminus \{n\}})$ and the ordering of $x_n$ values in the array can be posited arbitrarily but fixed afterwards. Thus, $A_0(\bx_{U \setminus \{n\}})$ is of size $|\bigcup_{0 \leq i \leq k} \Pi_{U} R_{N_i}| = O(|\db_n|)$ and allows for every tuple $\ba_{U \setminus \{n\}} \in \bigcup_{0 \leq i \leq k} \Pi_{U \setminus \{n\}} R_{N_i}$, a direct (array) access to all possible $x_n$ values that could appear alongside $\ba_{U \setminus \{n\}}$ in the database instance $\db_n$. It is easy to see that this construction costs $O(|\db_n|)$ time and space.

Now we start constructing the base-case oracle $\Oracle_0(\bx_{U \setminus \{n\}})$ for $\formula_n(\bx_{U}) = R_U(\bx_U)$. It follows exactly as $A_0(\bx_{U \setminus \{n\}})$ except that each entry $\bx_{U \setminus \{n\}} = \ba_{U \setminus \{n\}} \in \Oracle_0(\bx_{U \setminus \{n\}})$ stores instead a trivial array decomposition of $A_0(\ba_{U \setminus \{n\}})$, replacing each value of $x_n$ in $A_0(\ba_{U \setminus \{n\}})$ by its weight $R_U(x_n, \ba_{U \setminus \{n\}}) \in \boldsymbol{D}$. So the $\interval$-th element in $A_0(\ba_{U \setminus \{n\}})$, say $a_n = A_0(\ba_{U \setminus \{n\}})[\interval]$, corresponds to 
the $\interval$-th entry in the array decomposition $\Oracle_0(\ba_{U \setminus \{n\}})$, i.e. $\left([\interval, \interval], R_U(a_n , \ba_{U \setminus \{n\}}) \right) = \left([\interval, \interval], \formula_n(a_n, \ba_{U \setminus \{n\}}) \right)$. Thus, $\Oracle_0(\bx_{U \setminus \{n\}})$ is of size $|A_0(\bx_{U \setminus \{n\}})| = O(|\db_n|)$. We recall that for $(a_n, \ba_{U \setminus \{n\}}) \notin R_U$, we have $R_U(a_n, \ba_{U \setminus \{n\}}) = \zerobf$. Applying \autoref{thm:range-sum}, we construct a $\RangeSumOracle$ on each array decomposition $\Oracle_0(\ba_{U \setminus \{n\}})$, after spending $O(|\db_n|)$ preprocessing time building the $\RangeSum$ data structures. Abusing notations, we denote the entire oracle as 
$\Oracle_0(\bx_{U \setminus \{n\}})$ to implicitly indicate that it is a hashtable of array decompositions equipped with the $\RangeSumOracle$ that supports the following query in $O(\ackfunc{\db_n})$ time:
\begin{description}
    \item[oracle] $\Oracle_0(\bx_{U \setminus \{n\}})$
    \item[input] a tuple $\ba_{U \setminus \{n\}} \in \bigcup_{0 \leq i \leq k} \Pi_{U \setminus \{n\}} R_{N_i}$ (to identity the array decomposition $\Oracle_i(\ba_{N_i \setminus \{n\}})$ to be queried) and a query range $[\open+1, \close]$, where $ 0 \leq \open < \close$ are two break points of the array decomposition.
    \item[output] a range sum $\bigoplus_{\interval \in [\open+1, \close]} \formula_n \left(A_0(\ba_{U \setminus \{n\}})[\interval], \; \ba_{U \setminus \{n\}} \right)$.
\end{description}


\introparagraph{\textcolor{blue}{the inductive case of $\formula_n(\bx_{N_i})$}}
For $\formula_n(\bx_{N_i})$, where $i \in [k]$, following \eqref{eq:derivation-oracle}, we have that $\formula_n(\bx_{N_i}) = R_{N_i}(\bx_{N_i }) \vdash  \formula_n(\bx_{N^-_i}) = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\bx_{S_{i-1}}) \otimes \formula_n(\bx_{N_{i-1}})$. Thus, for a fixing of $\bx_{N_i \setminus \{n\}} = \ba_{N_i \setminus \{n\}}$, we have

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% the full derivation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{equation} \label{eq:oracle-derivation}
%     \begin{aligned}
%     \formula_n(x_n, \ba_{N_i \setminus\{n\}}) & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \formula_n(x_n, \Pi_{N^-_{i} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \formula_n(x_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \left(R_{N_{i-1}}(x_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_{i}\setminus \{n\}}) \vdash \formula_n(x_n, \Pi_{N^-_{i-1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}}) \right)  \\
%     & \; \vdots \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \; \otimes    \\
%     & \qquad \left( \cdots R_{N_{1}}(x_n, \Pi_{N_{1} \setminus \{n\} } \ba_{N_{i} \setminus \{n\}}) \vdash \left(\mu_n(\Pi_{S_{1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes (R_{N_{1}}(x_n, \Pi_{N_{1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}}) \vdash \formula_n(x_n, \Pi_{N^-_{1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}})) \right) \cdots  \right)   \\
%     & =  R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \; \otimes  \\
%     & \qquad \left(\cdots  (R_{N_{1}}(x_n, \Pi_{N_{1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}}) \vdash  \mu_n(\Pi_{S_0 \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \formula_n(x_n, \Pi_{U \setminus \{n\}} \ba_{N_{i} \setminus\{n\}})) \cdots   \right) \\
%     & =  R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \; \otimes  \\
%     & \qquad \left(\cdots  (R_{N_{1}}(x_n, \Pi_{N_{1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}}) \vdash  \mu_n(\Pi_{S_0 \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes R_U(x_n, \Pi_{U \setminus \{n\}} \ba_{N_{i} \setminus\{n\}})) \cdots   \right) 
%     \end{aligned}
% \end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% the inductive derivation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation} \label{eq:oracle-derivation}
    \begin{aligned}
    \formula_n(x_n, \ba_{N_i \setminus\{n\}}) & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \formula_n(x_n, \Pi_{N^-_{i} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
    & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \formula_n(x_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) 
    \end{aligned}
\end{equation}

Following the bottom-up construction, for the $i$-th $(i > 0)$ time entering in the for-loop on \autoref{line:oracle-inductive}, we have constructed the $(i-1)$-th $\RangeSumOracle$(s) denoted as $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$ for $\formula_n(\bx_{N_{i-1}})$. Specifically, the $\RangeSumOracle$(s) $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$ is a hashtable of size $O(|\db_n|)$ containing array decompositions as entries that supports the following range query in $O(\ackfunc{\db_n})$ time:


\begin{description}
    \item[oracle] $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$
    \item[input] a tuple $\ba_{N_{i-1} \setminus \{n\}} \in \bigcup_{i-1 \leq s \leq k} \Pi_{N_{i-1} \setminus \{n\}} R_{N_s}$ (i.e. a query key to identity the array decomposition $\Oracle_{i-1}(\ba_{N_{i-1} \setminus \{n\}})$ to be queried) and a query range $[\open+1, \close]$, where $0 \leq \open \leq \close$ are two break points of the array decomposition $\Oracle_{i-1}(\ba_{N_{i-1} \setminus \{n\}})$. In particular, the break points of the array decomposition $\Oracle_i(\ba_{N_i \setminus \{n\}})$ are $\interval$ and $\interval-1$, where
    \begin{align*}
        \interval \in \left\{\interval \mid \left( A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus \{n\}})[\interval], \ba_{N_{i-1} \setminus \{n\}}\right) \in \bigcup_{i-1 \leq s\leq k} \Pi_{N_{i-1}} R_{N_s} \right\}
    \end{align*}
    \item[output] a range sum $\bigoplus_{\interval \in [\open+1, \close]} \formula_n\left(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus \{n\}})[\interval], \; \ba_{N_{i-1} \setminus \{n\}} \right)$, (or $\zerobf$ if $\open = \close$).
\end{description}

We now start constructing a new $\RangeSumOracle$ $\Oracle_{i}(\bx_{N_{i} \setminus \{n\}})$ for $\formula_n(\bx_{N_i})$, using the $\RangeSumOracle$ $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$. We initialize $\Oracle_i(\bx_{N_i \setminus \{n\}})$ as a hashtable with $\bx_{N_i \setminus \{n\}}$ as its key, where each entry $\bx_{N_i \setminus \{n\}} = \ba_{N_i \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_t \setminus \{n\}} R_{N_s}$ is intialized as an empty array decomposition, denoted as $\Oracle_i( \ba_{N_i \setminus \{n\}})$. Furthermore, we initialize a set of scanning iterators $\open_{\ba_{N_i \setminus \{n\}}} = 0$, one for each $\ba_{N_i \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_t \setminus \{n\}} R_{N_s}$ that pinpoints the last constructed break point throughout its ongoing construction process. 

Next, we will make one scan over every entry (array decomposition) stored in $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$ by iterating over its break points, and for each array decomposition $\Oracle_{i-1}(\ba_{N_i \setminus \{n\}})$, we construct the array decompositions $\Oracle_i(\ba_{N_i \setminus \{n\}})$ for all $\ba_{N_i \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_t \setminus \{n\}} R_{N_s}$ such that $\Pi_{N_{i-1} \setminus \{n\}} \ba_{N_i \setminus \{n\}} = \ba_{N_{i-1} \setminus \{n\}}$ simultaneously. Let us now describe the exact steps when scanning an array decomposition $\Oracle_{i-1}(\ba_{N_{i-1} \setminus \{n\}})$ in the oracle $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$. First, we initialize a scanning iterator $\close = 1$ to scan the array decomposition $\Oracle_{i-1}(\ba_{N_{i-1} \setminus \{n\}})$ by moving $\close$ forward to the next break point. 

As we are scanning at the break point $\close$ of the array decomposition $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$, we retrieve its corresponding $x_n$ value via $A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus \{n\}})[\close] = a_n$. For every ongoing construction of $\Oracle_i(\ba_{N_i \setminus \{n\}})$ (i.e. $\Pi_{N_{i-1} \setminus \{n\}} \ba_{N_i \setminus \{n\}} = \ba_{N_{i-1} \setminus \{n\}}$), if $(a_n, \ba_{N_{i} \setminus \{n\}}) \in \bigcup_{i \leq s \leq k} \Pi_{N_{i}} R_{N_s}$, we set both $\close-1$ and $\close$ as it new break points by appending the following two pairs to the array decomposition $\Oracle_i(\ba_{N_i \setminus \{n\}})$:
\begin{enumerate}
    \item the first pair to be appended is
    \begin{align*}
        \left( [\open_{\ba_{N_i \setminus \{n\}}} + 1, \close -1 ], \; \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes M_1 \right)
    \end{align*}
    where $M_1$ is a call to the $\RangeSumOracle$ $\Oracle_{i-1}(\ba_{N_{i-1} \setminus \{n\}})$ with the input parameters $\ba_{N_{i-1} \setminus\{n\}} = \Pi_{N_{i-1} \setminus\{n\}} \ba_{N_i \setminus \{n\}}$ (the query key) and $[\open_{\ba_{N_i \setminus \{n\}}} + 1, \close -1]$ (the query range). Therefore, by induction hypothesis, 
    \begin{align*}
        M_1 = \bigoplus_{\interval \in [\open_{\ba_{N_i \setminus \{n\}}} + 1, \close -1]}\formula_n \left(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval],  \ba_{N_{i-1} \setminus\{n\}} \right)
    \end{align*}
    and $M_1$ is returned by $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$ in time $O(\ackfunc{\db_n})$.
    \item the second pair to be appended is
    \begin{align*}
        \left( [\close, \close], \; R_{N_i}(a_n, \ba_{N_i \setminus \{n\}}) \oplus \indicator{\neg R_{N_i} } (a_n, \ba_{N_i \setminus \{n\}}) \otimes \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes M_2 \right)
    \end{align*}
    where $M_2$ is a call to the $\RangeSumOracle$ $\Oracle_{i-1}(\ba_{N_{i-1} \setminus \{n\}})$ with the input parameters $\ba_{N_{i-1} \setminus\{n\}} = \Pi_{N_{i-1} \setminus\{n\}} \ba_{N_i \setminus \{n\}}$ (the query key) and $[\close, \close]$ (the query range). Therefore, by induction hypothesis,
    \begin{align*}
        M_2 = \bigoplus_{\interval \in [\close, \close]}\formula_n \left(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \ba_{N_{i-1} \setminus \{n\}} \right) = \formula_n(a_n, \ba_{N_{i-1} \setminus \{n\}}) = \formula_n(a_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})
    \end{align*}
    and $M_2$ is returned by $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$ in time $O(\ackfunc{\db_n})$.
\end{enumerate}

The correctness of the second pair simply follows from \eqref{eq:oracle-derivation}, where we fix the value of $x_n$ to be $a_n = A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval]$. We now reason the correctness of the first pair as follows: by construction of break points, $\open_{\ba_{N_i \setminus \{n\}}}$ and $\close$ are two consecutive break points for $\Oracle_{i}(\bx_{N_{i} \setminus \{n\}})$, thus 
$(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \ba_{N_i \setminus\{n\} }) \notin R_{N_i}$, for all $\interval \in [\open_{\ba_{N_i \setminus \{n\}}} + 1, \close -1]$. Therefore, $R_{N_i} (A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval]) = \zerobf$ and 
$\indicator{R_{N_i}} (A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval]) = \onebf$ for all $\interval \in [\open_{\ba_{N_i \setminus \{n\}}} + 1, \close -1]$. Still following \eqref{eq:oracle-derivation}, we have that
\begin{equation*} 
    \begin{aligned}
    \formula_n(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \ba_{N_i \setminus\{n\}}) & = R_{N_i} (A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval]) \oplus \indicator{R_{N_i}} (A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \ba_{N_i \setminus\{n\}}) \\
    & \qquad \otimes \formula_n(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \Pi_{N^-_{i} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
    & = \zerobf \oplus \onebf \otimes \formula_n(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \; \Pi_{N^-_{i} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
    & = \formula_n(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \; \Pi_{N^-_{i} \setminus \{n\}} \ba_{N_i \setminus\{n\}})\\ 
    & =  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \formula_n(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \;\Pi_{N_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) 
    \end{aligned}
\end{equation*}
Hence, the correctness of the first pair follows because
\begin{align*}
    \bigoplus_{\interval \in [\open_{\ba_{N_i \setminus \{n\}}} + 1, \close -1]} \formula_n(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i-1} \setminus\{n\}})[\interval], \ba_{N_i \setminus\{n\}}) = \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes M_1.
\end{align*}

As a summary, one scan over the break points of every array decomposition stored in $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$ costs time $O(|\db_n|)$, i.e. the size of the oracle. Furthermore, for a fixed $\ba_{N_{i-1} \setminus \{n\}} \in \bigcup_{i-1 \leq s \leq k} \Pi_{N_{i-1} \setminus \{n\}} R_{N_s}$, we make break points across all the (constructing) array decompositions of $\Oracle_{i}(\ba_{N_{i} \setminus \{n\}})$ where $\ba_{N_{i} \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_{i}} R_{N_s}$ and $\Pi_{N_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}} = \ba_{N_{i-1} \setminus\{n\}}$ and by construction, the break points are $\interval$ and $\interval - 1$ where
\begin{align*}
    \interval \in \left\{\interval \mid \left( A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})[\interval], \ba_{N_{i} \setminus \{n\}}\right) \in \bigcup_{i \leq s\leq k} \Pi_{N_{i}} R_{N_s} \right\}
\end{align*}
Observe that the break points constructed in $\Oracle_{i}(\ba_{N_{i} \setminus \{n\}})$ is a subset of those of $\Oracle_{i-1}(\Pi_{N_{i-1} \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})$, thus we are free from the risk of asking the oracle $\Oracle_{i-1}(\Pi_{N_{i-1} \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})$ with mis-aligned intervals, when constructing $\Oracle_{i}(\ba_{N_{i} \setminus \{n\}})$. The number of break points to be constructed in the array decomposition $\Oracle_{i}(\ba_{N_{i} \setminus \{n\}})$ is at most $\sum_{i \leq s \leq k} \mathsf{deg}_{R_{N_s}}(\ba_{N_i \setminus \{n\}}) $, where $\mathsf{deg}_{R_{N_s}}(\ba_{N_i \setminus \{n\}})$ denotes the degree of $\ba_{N_i \setminus \{n\}}$ in $R_{N_s}$, i.e., the number of tuples in $R_{N_s}$ that coincide with $\ba_{N_i \setminus \{n\}}$ on the variables $\bx_{N_i \setminus \{n\}}$. Therefore, the total number of break points in the oracle $\Oracle_{i}(\bx_{N_{i} \setminus \{n\}})$ is at most 
%%%%%%%%%%%%%%%%% alternatively, use \left| R_{N_s}(x_n, \bx_{N_s \setminus N_i}, \ba_{N_i \setminus \{n\}})  \right| for degrees
\begin{align*}
    \sum_{\ba_{N_i \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_i \setminus \{n\}} R_{N_s}} \sum_{i \leq s \leq k} \mathsf{deg}_{R_{N_s}}(\ba_{N_i \setminus \{n\}}) \leq \sum_{i \leq s \leq k}|R_{N_s}| = O(|\db_n|).
\end{align*}
The new-built oracle $\Oracle_{i}(\bx_{N_{i} \setminus \{n\}})$ is thus of size $O(|\db_n|)$. Furthermore, for each break point, it costs $O(\ackfunc{\db_n})$ to get the two range sums $M_1, M_2$ from the oracle $\Oracle_{i-1}(\bx_{N_{i-1} \setminus \{n\}})$, thus the total time of the construction of $\Oracle_{i}(\bx_{N_{i} \setminus \{n\}})$ is $O(|\db_n| \cdot \ackfunc{\db_n})$. The $\RangeSumOracle$ $\Oracle_{i}(\bx_{N_{i} \setminus \{n\}})$ supports the following range query in time $O(\ackfunc{\db_n})$:

\begin{description}
    \item[oracle] $\Oracle_{i}(\bx_{N_{i} \setminus \{n\}})$
    \item[input] a tuple $\ba_{N_{i} \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_{i} \setminus \{n\}} R_{N_s}$ (i.e. a query key to identity the array decomposition $\Oracle_{i}(\ba_{N_{i} \setminus \{n\}})$ to be queried) and a query range $[\open+1, \close]$, where $0 \leq \open \leq \close$ are two break points of the array decomposition $\Oracle_{i}(\ba_{N_{i} \setminus \{n\}})$. In particular, the break points of the array decomposition $\Oracle_i(\ba_{N_i \setminus \{n\}})$ are $\interval$ and $\interval-1$, where
    \begin{align*}
        \interval \in \left\{\interval \mid \left( A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})[\interval], \ba_{N_{i} \setminus \{n\}}\right) \in \bigcup_{i \leq s\leq k} \Pi_{N_{i}} R_{N_s} \right\}
    \end{align*}
    \item[output] a range sum $\bigoplus_{\interval \in [\open+1, \close]} \formula_n\left(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})[\interval], \; \ba_{N_{i} \setminus \{n\}} \right)$, (or $\zerobf$ if $\open = \close$).
\end{description}

% \begin{equation} \label{eq:oracle-derivation-type-base}
%     \begin{aligned}
%     \formula_n(x_n, \ba_{N_i \setminus\{n\}}) & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \formula_n(x_n, \Pi_{N^-_{i} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \formula_n(x_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \left(\zerobf \oplus \formula_n(x_n, \Pi_{N^-_{i-1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}}) \right)  \\
%     & \; \vdots \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \left[\zerobf \oplus \cdots \zerobf \oplus \left[\mu_n(\Pi_{S_{1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes (\zerobf \oplus \formula_n(x_n, \Pi_{N^-_{1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}})) \right] \cdots  \right]   \\
%     & =  R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \left[\zerobf \oplus \cdots  (\zerobf \oplus  \mu_n(\Pi_{S_0 \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \formula_n(x_n, \Pi_{U \setminus \{n\}} \ba_{N_{i} \setminus\{n\}})) \cdots   \right] \\
%     & =  R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \left[\zerobf \oplus \cdots  (\zerobf \oplus  \mu_n(\Pi_{S_0 \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \zerobf) \cdots   \right] \\
%     & =  R_{N_i}(x_n, \ba_{N_i \setminus\{n\} })
%     \end{aligned}
% \end{equation}

% \begin{equation} \label{eq:oracle-derivation-type-i}
%     \begin{aligned}
%     \formula_n(x_n, \ba_{N_i \setminus\{n\}}) & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \formula_n(x_n, \Pi_{N^-_{i} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash  \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \formula_n(x_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \left(\zerobf \oplus \indicator{\neg R_{N_{i-1}}}(x_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_{i}\setminus \{n\}}) \otimes \formula_n(x_n, \Pi_{N^-_{i-1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}}) \right)  \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash \mu_n(\Pi_{S_{i-1} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \indicator{\neg R_{N_{i-1}}}(x_n, \Pi_{N_{i-1} \setminus \{n\}} \ba_{N_{i}\setminus \{n\}}) \otimes \formula_n(x_n, \Pi_{N^-_{i-1} \setminus \{n\}} \ba_{N_{i} \setminus\{n\}})  \\
%     & \; \vdots \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash \left( \bigotimes_{t+1 \leq j \leq i-1} \mu_n(\Pi_{S_{j} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \indicator{\neg R_{N_{j}}}(x_n, \Pi_{N_{j} \setminus \{n\}} \ba_{N_{i}\setminus \{n\}}) \right) \otimes \formula_n(x_n, \Pi_{N^-_{t+1} \setminus \{n\}}\ba_{N_i \setminus\{n\} })  \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash \left( \bigotimes_{t+1 \leq j \leq i-1} \mu_n(\Pi_{S_{j} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \onebf \right) \otimes \formula_n(x_n, \Pi_{N^-_{t+1} \setminus \{n\}}\ba_{N_i \setminus\{n\} })  \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash \left( \bigotimes_{t+1 \leq j \leq i-1} \mu_n(\Pi_{S_{j} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \onebf \right) \otimes \mu_n(\Pi_{S_{t} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \otimes \formula_n(x_n, \Pi_{N_{t} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \vdash \bigotimes_{t \leq j \leq i-1} \mu_n(\Pi_{S_{j} \setminus \{n\}} \ba_{N_i \setminus\{n\}})  \otimes \formula_n(x_n, \Pi_{N_{t} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) \\
%     & = R_{N_i}(x_n, \ba_{N_i \setminus\{n\} }) \oplus \indicator{\neg R_{N_i}}(x_n, \ba_{N_i \setminus\{n\} }) \otimes \bigotimes_{t \leq j \leq i-1} \mu_n(\Pi_{S_{j} \setminus \{n\}} \ba_{N_i \setminus\{n\}})  \otimes \formula_n(x_n, \Pi_{N_{t} \setminus \{n\}} \ba_{N_i \setminus\{n\}}) 
%     \end{aligned}
% \end{equation}

To conclude this section, we present the following theorem, whose proof is immediate from the prior discussion in this section. Here, $k = d(n)$, where we recall that $d(n)$ is number of hyperedges containing the $\pn$-leaf $n$ in $\mH_n$.

\begin{theorem} \label{thm:oracle-main}
    Let $\mH_n$ be a signed hypergraph with a $\pn$-leaf $n$. Let $\formula_n(\bx_{[n]})$ be a $\nestfaqneg$ expression \eqref{eq:derivation} associated with $\mH_n$ (thus recognized by $\CFG_n$ \eqref{eq:cfg_n}) and $\db_n$ be its database instance. Suppose that $U = N_0 \subseteq N_1 \subseteq \cdots \subseteq N_k$ are the only hyperedges containing the $\pn$-leaf $n$ in $\mH_n$. Then, there is an algorithm that takes $(\formula_n(\bx_{[n]}), \db_n)$ as input and constructs in $O(|\formula_n| + k \cdot |\db_n|)$ time, a $\RangeSumOracle$ $\Oracle_i(\bx_{N_i \setminus \{n\}})$, for every $i = 0, 1, \ldots, k$, and the oracle $\Oracle_i(\bx_{N_i \setminus \{n\}})$ is of size $O(|\db_n|)$ and supports the following range query in $O(\ackfunc{\db_n})$ time:
    \begin{description}
        \item[oracle] $\Oracle_{i}(\bx_{N_{i} \setminus \{n\}})$
        \item[input] a query key $\ba_{N_{i} \setminus \{n\}} \in \bigcup_{i \leq s \leq k} \Pi_{N_{i} \setminus \{n\}} R_{N_s}$ to identity the array decomposition $\Oracle_{i}(\ba_{N_{i} \setminus \{n\}})$ to be queried, and a query range $[\open+1, \close]$, where $0 \leq \open \leq \close$ are two break points of the array decomposition $\Oracle_{i}(\ba_{N_{i} \setminus \{n\}})$. In particular, the break points of the array decomposition $\Oracle_i(\ba_{N_i \setminus \{n\}})$ are $\interval$ and $\interval-1$, where
        \begin{align*}
            \interval \in \left\{\interval \mid \left( A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})[\interval], \ba_{N_{i} \setminus \{n\}}\right) \in \bigcup_{i \leq s\leq k} \Pi_{N_{i}} R_{N_s} \right\}
        \end{align*}
        \item[output] a range sum $\bigoplus_{\interval \in [\open+1, \close]} \formula_n\left(A_0(\Pi_{U \setminus \{n\}} \ba_{N_{i} \setminus \{n\}})[\interval], \; \ba_{N_{i} \setminus \{n\}} \right)$, (or $\zerobf$ if $\open = \close$).
    \end{description}    
\end{theorem}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Stashed Demos %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bigskip
% \bigskip
% \highlight{the upper level: $\nonterm_n(\bx_{N^-_2}) \derive \formula_n(\bx_{S_1}) \otimes \nonterm_n(\bx_{N_1}) \yield \formula_n(\bx_{S_1}) \otimes (R_N(\bx_{N_1}) \vdash \nonterm_n(\bx_{U})) $}

% \introparagraph{\textcolor{blue}{the $N_1$ case}}
% Now for $\nonterm_n(\bx_{N_1}) \yield R_N(\bx_{N_1}) \vdash \nonterm_n(\bx_{U})$, we will build an oracle $\Oracle_n( \bx_{N_1 \setminus \{n\}})$, using the oracle $\Oracle_n( \bx_{U \setminus \{n\}})$ we have just built for $\nonterm_n(\bx_{U})$. We start by building a hashtable $\Oracle_n( \bx_{N_1 \setminus \{n\}})$ with $\bx_{N_1 \setminus \{n\}}$ as its key, where each entry $\bx_{U \setminus \{n\}} = \ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$ is intialized as an empty array decomposition, written as $\Oracle_n( \ba_{N_1 \setminus \{n\}})$. 
% We distinguish for each $\ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$, whether $\Pi_{U \setminus \{n\}}\ba_{N_1 \setminus \{n\}} \in \Pi_{U \setminus \{n\}} R_U$ or not.

% \begin{itemize}
%     \item for each $\ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$ such that $\Pi_{U \setminus \{n\}}\ba_{N_1 \setminus \{n\}} \notin \Pi_{U \setminus \{n\}} R_U$, we observe that $R_U$ will not constribute to the aggregations of $x_n$. Thus, we can build trivial array decompositions as in the case for $\nonterm_n(\bx_{U})$.
%     \item otherwise, $\ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$ such that $\Pi_{U \setminus \{n\}}\ba_{N_1 \setminus \{n\}} \in R_U$. 
%     Then, for every distinct $\ba_{U \setminus \{n\}} \in \Pi_{U \setminus \{n\}} R_{N_1}$, we will scan the array $\Oracle_n( \ba_{U \setminus \{n\}})$. 
    
%     Say for a fixed $\ba_{U \setminus \{n\}}$, we initialize two scanning pointers $\open = \close = 1$ and all empty array decompositions $\Oracle_n( \ba_{N_1 \setminus \{n\}})$ such that $\ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$ and $\Pi_{U \setminus \{n\}}\ba_{N_1 \setminus \{n\}} = \ba_{U \setminus \{n\}}$ are to be filled. In particular, as we scan the array $\Oracle_n( \ba_{U \setminus \{n\}})$ (by move $\close$ forward to the next break point) at its $\close$-th element. Let $a_n$ be the $\close$-th value of the $x_n$ in the array. If there are some tuple(s) $(a_n, \ba_{N_i \setminus \{n\}}) \in R_{N_i}$ such that $\Pi_{N_1 \setminus \{n\}}\ba_{N_i \setminus \{n\}} = \ba_{N_1 \setminus \{n\}}$, for some $i \in [k]$, then $\close$ should be a break point. Thus, we ask the oracle $\Oracle_n( \bx_{U \setminus \{n\}})$ one query with input $(\ba_{U \setminus \{n\}}, [\open, \close - 1])$ and it tells a sum $\bigoplus_{\interval \in [\open, \close - 1]} \nonterm_n(x_n, \ba_{U \setminus \{n\}})[\interval]$.
%     Then by getting the answers, we can fill the corresponding array decomposition $\Oracle_n( \ba_{N_1 \setminus \{n\}})$ with two pairs, 
%     \begin{align*}
%         \left( [\open, \close - 1], \bigoplus_{\interval \in [\open, \close - 1]} \nonterm_n(x_n, \ba_{U \setminus \{n\}})[\interval] \right) \quad \text{and} \quad \left( [\close, \close], \; R_{N_1}(a_n, \ba_{N_1 \setminus \{n\}}) \right)
%     \end{align*}
%     Then we update $\open = \close$ and continue scanning until we exhaust the array $\Oracle_n( \ba_{U \setminus \{n\}})$. As a brief recap, by scanning over the array $\Oracle_n( \ba_{U \setminus \{n\}})$ once, we fill in all array decompositions $\nonterm_n(x_n, \ba_{N_1 \setminus \{n\}})$ such that $\ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$ and $\Pi_{U \setminus \{n\}}\ba_{N_1 \setminus \{n\}} = \ba_{U \setminus \{n\}}$. 
% \end{itemize}


% \highlight{recall the upper level: $\nonterm_n(\bx_{N^-_2}) \derive \formula_n(\bx_{S_1}) \otimes \nonterm_n(\bx_{N_1}) \yield \formula_n(\bx_{S_1}) \otimes (R_N(\bx_{N_1}) \vdash \nonterm_n(\bx_{U})) $}

% \highlight{the upper level: $\nonterm_n(\bx_{N^-_3}) \derive \formula_n(\bx_{S_2}) \otimes \nonterm_n(\bx_{N_2}) \yield \formula_n(\bx_{S_2}) \otimes (R_N(\bx_{N_2}) \vdash \nonterm_n(\bx_{N^-_2})) $}

% \medskip
% \introparagraph{\textcolor{blue}{the $N_2$ case}}
% Now for $\nonterm_n(\bx_{N_2}) \yield R_N(\bx_{N_2}) \vdash \nonterm_n(\bx_{N^-_2}) \derive R_N(\bx_{N_2}) \vdash \formula_n(\bx_{S_1}) \otimes \nonterm_n(\bx_{N_1})$, we build an oracle $\Oracle_n( \bx_{N_2 \setminus \{n\}})$, using the oracle $\Oracle_n( \bx_{N_1 \setminus \{n\}})$ we have just built for $\nonterm_n(\bx_{N_1})$. We start by building a hashtable $\Oracle_n( \bx_{N_2 \setminus \{n\}})$ with $\bx_{N_2 \setminus \{n\}}$ as its key, where each entry $\bx_{U \setminus \{n\}} = \ba_{N_2 \setminus \{n\}} \in \Pi_{N_2 \setminus \{n\}} R_{N_2}$ is intialized as an empty array decomposition, written as $\Oracle_n( \ba_{N_2 \setminus \{n\}})$. 

% We distinguish the tuples $\ba_{N_2 \setminus \{n\}} \in \Pi_{N_2 \setminus \{n\}} R_{N_2}$ into the following 3 cases:
% \begin{itemize}
%     \item if $\Pi_{N_1 \setminus \{n\}} \ba_{N_2 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$, then $\Oracle_n( \bx_{N_1 \setminus \{n\}})$ will be the oracle to be queried for the array decomposition $\Oracle_n( \ba_{N_2 \setminus \{n\}})$. 
%     \textcolor{orange}{Now for every distinct $\ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$, we will scan the array decomposition $\Oracle_n( \ba_{N_1 \setminus \{n\}})$ and fill in all array decompositions $\Oracle_n( \ba_{N_2 \setminus \{n\}})$ such that $\Pi_{N_1 \setminus \{n\}}\ba_{N_2 \setminus \{n\}} = \ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_1}$. So for every distinct $\ba_{N_1 \setminus \{n\}}$, we will scan the array decomposition $\Oracle_n( \ba_{N_1 \setminus \{n\}})$ once. \\
%     Say for a fixed $\ba_{N_1 \setminus \{n\}}$, we initialize two scanning pointers $\open = \close = 1$ and all empty array decompositions $\Oracle_n( \ba_{N_2 \setminus \{n\}})$ such that $\Pi_{N_1 \setminus \{n\}}\ba_{N_2 \setminus \{n\}} = \ba_{N_1 \setminus \{n\}}$ are to be filled in.
%     In particular, as we scan the array decomposition $\Oracle_n( \ba_{N_1 \setminus \{n\}})$ (by move $\close$ to the next break point). Let $a_n$ be the $\close$-th valuation of $x_n$ in $\ba_{N_1 \setminus \{n\}}$. If there are some tuple(s) $(a_n, \ba_{N_i \setminus \{n\}}) \in R_{N_i}$, for $2 \leq i \leq k$, such that $\Pi_{N_1 \setminus \{n\}}\ba_{N_i \setminus \{n\}} = \ba_{N_1 \setminus \{n\}}$, then we ask the oracle $\Oracle_n( \ba_{N_1 \setminus \{n\}})$ one query with inputs $(\ba_{N_1 \setminus \{n\}}, [\open, \close])$. Then by getting the answer, we can fill the corresponding array decomposition $\Oracle_n( \ba_{N_2 \setminus \{n\}})$ with two pairs 
%     \begin{align*}
%         \left( [\open, \close - 1], \bigoplus_{\interval \in [\open, \close - 1]} \Oracle_n( \ba_{N_1 \setminus \{n\}})[\interval] \right) \quad \text{and} \quad \left( [\close, \close], \; R_{N_2}(a_n, \ba_{N_2 \setminus \{n\}})  \right)
%     \end{align*}
%     Then we update $\open = \close + 1$ and continue scanning until we exhaust the array decomposition $\Oracle_n( \ba_{N_1 \setminus \{n\}})$. 
%     }
%     \highlight{As a sanity check, how many times we ask the oracle? We ask the oracle for a fixed $\ba_{N_1 \setminus \{n\}}$, 
%     $ \sum_{2 \leq i \leq k} \left| R_{N_i}(x_n, \bx_{N_i \setminus N_1}, \ba_{N_1 \setminus \{n\}}) \right|$ times. And we scan it for every $\ba_{N_1 \setminus \{n\}} \in \Pi_{N_1 \setminus \{n\}} R_{N_2}$}
%     \item otherwise, if $\Pi_{U \setminus \{n\}}\ba_{N_2 \setminus \{n\}} \in \Pi_{U \setminus \{n\}} R_U$, then $\Oracle_n( \bx_{U \setminus \{n\}})$ is the oracle to be queried for the array decomposition $\Oracle_n( \ba_{N_2 \setminus \{n\}})$.
%     Then, for every distinct $\ba_{U \setminus \{n\}} \in \Pi_{U \setminus \{n\}} R_{N_2}$, we will scan the array $\Oracle_n( \ba_{U \setminus \{n\}})$. 
    
%     Say for a fixed $\ba_{U \setminus \{n\}}$, we initialize two scanning pointers $\open = \close = 1$ and all empty array decompositions $\Oracle_n( \ba_{N_2 \setminus \{n\}})$ such that $\ba_{N_2 \setminus \{n\}} \in \Pi_{N_2 \setminus \{n\}} R_{N_2}$ and $\Pi_{U \setminus \{n\}}\ba_{N_2 \setminus \{n\}} = \ba_{U \setminus \{n\}}$ are to be filled. In particular, as we scan the array $\Oracle_n( \ba_{U \setminus \{n\}})$ at its $\close$-th element. Let $a_n$ be the $\close$-th valuation of $x_n$ of the array. If there are some tuple(s) $(a_n, \ba_{N_i \setminus \{n\}}) \in R_{N_i}$ such that $\Pi_{U \setminus \{n\}} \ba_{N_i \setminus \{n\}} = \ba_{U \setminus \{n\}}$, for some $2 \leq i \leq k$, then $\close$ should be a break point. Thus, we ask the oracle $\Oracle_n( \bx_{U \setminus \{n\}})$ one query with inputs $(\ba_{U \setminus \{n\}}, [\open, \close - 1])$ and it tells a sum $\bigoplus_{\interval \in [\open, \close - 1]} \nonterm_n(x_n, \ba_{U \setminus \{n\}})[\interval]$.
%     Then by getting the answers, we can fill the corresponding array decomposition $\Oracle_n( \ba_{N_2 \setminus \{n\}})$ with two pairs, 
%     \begin{align*}
%         \left( [\open, \close - 1], \bigoplus_{\interval \in [\open, \close - 1]} \Oracle_n( \ba_{U \setminus \{n\}})[\interval] \right) \quad \text{and} \quad \left( [\close, \close], \; R_{N_2}(a_n, \ba_{N_2 \setminus \{n\}}) \right)
%     \end{align*}
%     Then we update $\open = \close + 1$ and continue scanning until we exhaust the array $\Oracle_n( \ba_{U \setminus \{n\}})$. As a brief recap, by scanning over the array $\Oracle_n( \ba_{U \setminus \{n\}})$ once, we fill in all array decompositions $\Oracle_n( \ba_{N_2 \setminus \{n\}})$ such that $\Pi_{U \setminus \{n\}}\ba_{N_2 \setminus \{n\}} = \ba_{U \setminus \{n\}} \in \Pi_{U \setminus \{n\}} R_U$. 
%     \highlight{As a sanity check, how many times we ask the oracle? We ask the oracle for such a fixed $\ba_{U \setminus \{n\}}$, $\sum_{2 \leq i \leq k} \left| R_{N_i}(x_n, \bx_{N_i \setminus U}, \ba_{U \setminus \{n\}})  \right|$ times.}
%     \item otherwise, we have $\Pi_{U \setminus \{n\}}\ba_{N_2 \setminus \{n\}} \notin \Pi_{U \setminus \{n\}} R_U$ and $\Pi_{N_1 \setminus \{n\}} \ba_{N_2 \setminus \{n\}} \notin \Pi_{N_1 \setminus \{n\}} R_{N_1}$, then $\nonterm_n(\bx_{N_1}) \yield R_N(\bx_{N_1}) \vdash \nonterm_n(\bx_{U})$ will not constribute to the aggregations of $x_n$. Thus, we can build a trivial array decomposition $\Oracle_n( \bx_{N_2 \setminus \{n\}})$.
% \end{itemize}

% \hangdong{1. How to find all the intervals of $T(x, y, z, w, u)$ at the start? for each $y \in A$, we scan $A(\cdot, y)$ once and when scanning at $x$, if $T(x, y, z, w, u)$ for all $(z, w, u)$ such that $(y, z, w, u) \in T$, tag a new interval - $O(T + A)$ time for getting all intervals of $T$ ready for calling the lower level oracle $S$.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Stashed Demos %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{example}
%     Let $\mH = ([8], \mE^+, \mE^-)$ be a $\pn$-acyclic signed hypergraph, where $\mE^+ = \{\{1\}, \{6, 8\}, \{2, 3, 5, 6\}, \{2, 3, 4, 5\} \}$ and $\mE^- = \{\{1, 2, 3, 6, 8\}, \{2, 6, 8\}, \{3, 4, 5\}, \{4, 5\}, \{3, 7\}\}$. It is easy to see that it accepts a $\pn$-elimination sequence $(x_1, x_2, \ldots, x_8)$. We use the following $\nestfaqneg$ as a running example:

%     \begin{align*}
%         %% format the positive factors in the first line, negative factors in the second line
%         \varphi() & = \bigoplus_{\bx_{[8]}} R_1(\bx_1) \otimes R_{68}(\bx_{68}) \otimes R_{2367}(\bx_{2367}) \otimes R_{2345}(\bx_{2345}) \otimes \\
%         & \qquad (R_{12368} \oplus \indicator{\neg R_{12368}} \otimes \onebf) \otimes (R_{268} \oplus \indicator{\neg R_{268}} \otimes \onebf) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes (R_{37} \oplus \indicator{\neg R_{37}} \otimes \onebf)
%     \end{align*}
%     Following the $\pn$-elimination sequence $(x_1, x_2, \ldots, x_8)$, we first eliminate $x_8$ and rewrite $\varphi$ in the following way:

%     \hangdong{step 1 ($\alpha$-step at topmost). factor out those without $x_8$ and appoint the pivot factor (eat smaller factors containing $x_8$)}

%     \begin{align*}
%         %% factors that doesn't have x_8
%         \varphi() & = \bigoplus_{\bx_{[7]}} R_1(\bx_1) \otimes R_{2367}(\bx_{2367}) \otimes R_{2345}(\bx_{2345}) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes (R_{37} \oplus \indicator{\neg R_{37}} \otimes \onebf) \otimes \textcolor{blue}{I(\bx_{68 \setminus 8})} \otimes \\
%         %% factor that has x_8
%         & \qquad \bigoplus_{x_8}  R_{68}(\bx_{68}) \otimes (R_{12368} \oplus \indicator{\neg R_{12368}} \otimes \onebf) \otimes (R_{268} \oplus \indicator{\neg R_{268}} \otimes \onebf)
%     \end{align*}

%     \hangdong{step 2 ($\beta$-steps top-down). Indentify the biggest negative factor and nest $R_{68}$ and the other negative subtrees as its children, this effectively pushes down the aggregation into the lower level of the AST}

%     \begin{align*}
%         %% factors that doesn't have x_8
%         \varphi() & = \bigoplus_{\bx_{[7]}} R_1(\bx_1) \otimes R_{2367}(\bx_{2367}) \otimes R_{2345}(\bx_{2345}) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes (R_{37} \oplus \indicator{\neg R_{37}} \otimes \onebf) \otimes \textcolor{blue}{I(\bx_{68 \setminus 8})} \otimes \\
%         %% factor that has x_8
%         & \qquad \left[ R_{12368 \setminus 8}(\bx_{12368 \setminus 8}) \oplus \indicator{\neg R_{12368 \setminus 8}} (\bx_{12368 \setminus 8}) \otimes 
%         \bigoplus_{x_8}  R_{68}(\bx_{68}) \otimes (R_{268} \oplus \indicator{\neg R_{268}} \otimes \onebf) \right]
%     \end{align*}

%     \hangdong{step 3 ($\alpha$-step the subtree). factor out those without $x_7$ and appoint the pivot factor (eat smaller factors containing $x_7$)}

%     \hangdong{step 4 ($\beta$-steps top-down). Indentify the biggest negative factor and nest $R_{68}$ and the other negative subtrees as its children, this effectively pushes down the aggregation into the lower level of the AST}

%     \begin{align*}
%         %% factors that doesn't have x_8
%         \varphi() & = \bigoplus_{\bx_{[7]}} R_1(\bx_1) \otimes R_{2367}(\bx_{2367}) \otimes R_{2345}(\bx_{2345}) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes (R_{37} \oplus \indicator{\neg R_{37}} \otimes \onebf) \otimes \textcolor{blue}{I(\bx_{68 \setminus 8})} \otimes \\
%         %% factor that has x_8
%         & \qquad 
%         \left[ 
%             R_{12368 \setminus 8}(\bx_{12368 \setminus 8}) \oplus \indicator{\neg R_{12368 \setminus 8}} (\bx_{12368 \setminus 8}) \otimes  
%             \left[
%                 R_{268 \setminus 8} \oplus \indicator{\neg R_{268 \setminus 8}} \otimes \bigoplus_{x_8}  R_{68}(\bx_{68}) 
%             \right]
%         \right]
%     \end{align*}

%     \hangdong{continue to eliminate $x_7$}
%     \begin{align*}
%         %% factors that doesn't have x_7
%         \varphi() & = \bigoplus_{\bx_{[6]}} R_1(\bx_1) \otimes R_{2345}(\bx_{2345}) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes \textcolor{blue}{I(\bx_{68 \setminus 8})} \otimes \\
%         %% factor that has x_7
%         & \qquad 
%         \left[ 
%             R_{12368 \setminus 8}(\bx_{12368 \setminus 8}) \oplus \indicator{\neg R_{12368 \setminus 8}} (\bx_{12368 \setminus 8}) \otimes 
%             \left[
%                 R_{268 \setminus 8} \oplus \indicator{\neg R_{268 \setminus 8}} \otimes R_{68 \setminus 8}(\bx_{68 \setminus 8}) 
%             \right]
%         \right] \\
%         & \qquad \bigoplus_{x_7} R_{2367}(\bx_{2367}) \otimes (R_{37} \oplus \indicator{\neg R_{37}} \otimes \onebf)  
%     \end{align*}

%     \hangdong{continue to eliminate $x_6$}
%     \begin{align*}
%         %% factors that doesn't have x_6
%         \varphi() & = \bigoplus_{\bx_{[5]}} R_1(\bx_1) \otimes R_{2345}(\bx_{2345}) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes \\
%         %% factor that has x_6
%         & \qquad \bigoplus_{x_6} 
%         \left[ 
%             R_{12368 \setminus 8}(\bx_{12368 \setminus 8}) \oplus \indicator{\neg R_{12368 \setminus 8}} (\bx_{12368 \setminus 8}) \otimes 
%             \left[
%                 R_{268 \setminus 8} \oplus \indicator{\neg R_{268 \setminus 8}} \otimes R_{68 \setminus 8}(\bx_{68 \setminus 8}) 
%             \right] 
%         \right] \otimes R_{2367 \setminus 7}(\bx_{2367 \setminus 7}) \otimes \textcolor{blue}{I(\bx_{68 \setminus 8})} 
%     \end{align*}

%     \hangdong{it ends up with}
%     \begin{align*}
%         %% factors that doesn't have x_6
%         \varphi() & = \bigoplus_{\bx_{[5]}} R_1(\bx_1) \otimes R_{2345}(\bx_{2345}) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes  \textcolor{blue}{I(\bx_{2367 \setminus 67})}   \\
%         %% factor that has x_6
%         & \qquad \bigoplus_{x_6} 
%         \left[ 
%             R_{12368 \setminus 8}(\bx_{12368 \setminus 8}) \oplus \indicator{\neg R_{12368 \setminus 8}} (\bx_{12368 \setminus 8}) \otimes 
%             \left[
%                 R_{268 \setminus 8} \oplus \indicator{\neg R_{268 \setminus 8}} \otimes R_{68 \setminus 8}(\bx_{68 \setminus 8}) 
%             \right] 
%         \right] \otimes R_{2367 \setminus 7}(\bx_{2367 \setminus 7}) 
%     \end{align*}

%     \begin{align*}
%         %% factors that doesn't have x_6
%         \varphi() & = \bigoplus_{\bx_{[5]}} R_1(\bx_1) \otimes R_{2345}(\bx_{2345}) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes  \textcolor{blue}{I(\bx_{2367 \setminus 67})}  \otimes \\
%         %% factor that has x_6
%         & \qquad R_{12368 \setminus 68}(\bx_{12368 \setminus 68}) \oplus \indicator{\neg R_{12368 \setminus 68}} (\bx_{12368 \setminus 68}) \otimes 
%             \bigoplus_{x_6}  R_{2367 \setminus 7}(\bx_{2367 \setminus 7}) \otimes
%             \left[
%                 R_{268 \setminus 8} \oplus \indicator{\neg R_{268 \setminus 8}} \otimes R_{68 \setminus 8}(\bx_{68 \setminus 8}) 
%             \right] 
%     \end{align*}

%     \begin{align*}
%         %% factors that doesn't have x_6
%         \varphi() & = \bigoplus_{\bx_{[5]}} R_1(\bx_1) \otimes R_{2345}(\bx_{2345}) \otimes (R_{345} \oplus \indicator{\neg R_{345}} \otimes \onebf) \otimes (R_{45} \oplus \indicator{\neg R_{45}} \otimes \onebf) \otimes  \textcolor{blue}{I(\bx_{2367 \setminus 67})}  \otimes \\
%         %% factor that has x_6
%         & \qquad R_{12368 \setminus 68}(\bx_{12368 \setminus 68}) \oplus \indicator{\neg R_{12368 \setminus 68}} (\bx_{12368 \setminus 68}) \otimes 
%         \left[
%         R_{268 \setminus 68} \oplus \indicator{\neg R_{268 \setminus 68}}  
%                 \underbrace{\bigoplus_{x_6}  R_{2367 \setminus 7}(\bx_{2367 \setminus 7})  \otimes R_{68 \setminus 8}(\bx_{68 \setminus 8})}_{R_{2367 \setminus 67}}
%         \right]
%     \end{align*}
% \end{example}

% Now we prsent the $\cdelay$ algorithm for $\varphi$.

% \begin{example}
%     Let us use the aggregation step as an example:
%     %% write an equation here
%     \begin{align*}
%         \bigoplus_{x} \mathsf{R}(x) & \otimes \textcolor{red}{\left(\mathsf{A}(x, y, z, w, u) \oplus \indicator{\neg \mathsf{A}(x, y, z, w, u)} \otimes \left(\mathsf{B}(z,  u) \oplus \indicator{\neg \mathsf{B}(z, u)} \otimes a\right) \otimes \left(\mathsf{C}(w, u) \oplus \indicator{\neg \mathsf{C}(w, u)} \otimes b\right)\right) } \\
%         & \otimes \textcolor{olive}{\left(\mathsf{D}(x, y, z, w) \oplus \indicator{\neg \mathsf{D}(x, y, z, w)} \otimes \left(\mathsf{E}(x, z) \oplus \indicator{\neg \mathsf{E}(x, z)} \otimes \left(\mathsf{F}(x) \oplus \indicator{\neg \mathsf{F}(x)} \otimes c\right)\right) \right)}  \\
%         & \otimes  \textcolor{purple}{\left(\mathsf{G}(x, y, z) \oplus \indicator{\neg \mathsf{G}(x, y, z)} \otimes \left(\mathsf{H}(y, z) \oplus \indicator{\neg \mathsf{H}(y, z)} \otimes \left(\mathsf{I}(y) \oplus \indicator{\neg \mathsf{I}(y)} \otimes \mathsf{S}(v)\right)\right) \right)} 
%     \end{align*}
% \end{example}

 
%% draw a tree in latex using tikz package, put it in the center of the page, and add some text above and below the tree

% \begin{tikzpicture} 
%     %% root is \bigotimes, 2nd level are \bigooplus nodes, 3rd level are \bigotimes nodes, 4th level are relation nodes
%     %% root
%     \node (root) at (0, 0) {$\bigotimes$};

%     %% 2nd level
%     \node (oplus1) at (-2, -1) {$\bigoplus$};
%     \node (oplus2) at (2, -1) {$\bigoplus$};
%     \node (oplus3) at (0, -1) {$\bigoplus$};

%     %% 3rd level
%     \node (otimes1) at (-3, -2) {$\bigotimes$};
%     \node (otimes2) at (-1, -2) {$\bigotimes$};
%     \node (otimes3) at (1, -2) {$\bigotimes$};

%     %% 4th level
%     \node (R1) at (-3.5, -3) {$R_1$};
%     \node (R2) at (-2.5, -3) {$R_2$};
%     \node (R3) at (-1.5, -3) {$R_3$};

%     %% finish the tree
%     \draw (root) -- (oplus1);
%     \draw (root) -- (oplus2);
%     \draw (root) -- (oplus3);
    
%     \draw (oplus1) -- (otimes1);
%     \draw (oplus1) -- (otimes2);
%     \draw (oplus2) -- (otimes3);

%     \draw (otimes1) -- (R1);
%     \draw (otimes2) -- (R2);
%     \draw (otimes3) -- (R3);
% \end{tikzpicture}



% \begin{algorithm}[t]
% \caption{$\mathsf{Preprocess}(\varphi, \mH)$}
% \label{alg:faqneg-preprocessing}
% \KwIn{a free-connex $\pn$-acyclic $\nestfaqneg$ query $\varphi(\bx_{F})$ with signed hypergraph $\mH = ([n], \mE^+, \mE^-)$, a set of free variables $F = [f]$}
% \KwOut{succinct data structures $\mL_i$ for every $i\in[f]$ 
% }
% $(1, 2, \dots, f, f+1, \dots, n) \leftarrow$ a $\pn$-elimination sequence of $\mH' = ([n], \mE^+, \mE^- \cup \{F\})$ \\
% $\mH_n \leftarrow ([n], \mE^+_n, \mE^-_n)$, where $\mE^+_n = \mE^+$ and $\mE^-_n = \mE^-$ \\
% $\varphi_n \leftarrow \varphi$ \\ 
% \ForEach{$i = n, n-1, \dots, 1$}{
% 	$U\leftarrow$ a pivot hyperedge for the $\pn$-leaf $i$ in $\mH_i$\\
% 	Update the factor $R_U(\bx_{U}) \leftarrow \bigotimes_{K \in \mE^+_i, K \subseteq U} R_K(\bx_{K}) \otimes \bigotimes_{K \in \mE^-_i, K \subseteq U} \indicator{R_{K}(\bx_{K}) = 0}$\\
% 	\ForEach{$K_1, K_2, \dots, K_m \in \mE^-$ such that $U \subseteq K_1 \subseteq K_2 \subseteq \dots \subseteq K_m$}{
% 		\xiating{\dots}
% 	}
% 	\If{$i \leq f$}{
% 		$\mL_{i}[x_1, x_2, \dots, x_{i-1}] \leftarrow \{x_i \in \dom(X_i) \mid \varphi_i(\bx_{[i]}) = \varphi_i(x_1, x_2, \dots, x_i) \neq \zerobf\}$
% 	}
% 	$\mH_{i-1} = \removeleaf{\mH_i}{i}$	 \\
% 	\xiating{A projection step, where the 01 semiring might be used.} \\
% 	$\varphi_{i-1} \leftarrow$ the $\nestfaqneg$ query induced by $\mH_{i-1}$
% }
% \end{algorithm}


% \begin{proposition}
% For every $i \in \{f, f+1, \dots, n\}$ in the preprocessing phase, $\varphi_i(\bx_{F}) = \varphi(\bx_{F})$ and the factors in $\varphi_i$ can be computed in linear time. 
% \end{proposition}

% \begin{proposition}
% For every $i\in[f]$ and $\bx_{[i]} \in \prod_{1 \leq j \leq i}\dom(X_j)$, the nonempty sets $\mL_i[x_1, x_2, \dots, x_{i-1}]$ can be constructed in linear time.
% \end{proposition}

% \subsection{Enumeration phase}
% \label{sec:enumeration}

% \begin{algorithm}[t]
% \caption{$\mathsf{Enumerate}(\varphi, \mH)$}
% \label{alg:faqneg-enumerate}
% \KwIn{the data structures computed from the preprocessing phase}
% \KwOut{an enumeration of the answers of $\varphi$}
% \ForEach{$x_1 \in \mL_{1}$}{
% 	\ForEach{$x_2 \in \mL_{2}[x_1]$}{
% 		\dots\\
% 		\ForEach{$x_f \in \mL_{f}[x_1,x_2,\dots,x_{f-1}]$}{
% 			$\bx_{[F]} = (x_1, x_2, \dots, x_f)$ \\
% 			\textbf{output} $\varphi_{f}(\bx_{[F]})$
% 		}
% 	}
% }
% \end{algorithm}




\subsection{The $\pn$-elimination step: a summary} \label{sec:putting_things_together}
In this section, we put together the discussions in Appendix~\ref{sec:rewriting}, Appendix~\ref{sec:oracle} and Appendix~\ref{sec:aggregation} to prove the main theorem for the $\pn$-elimination sequence, i.e. \autoref{thm:faqneg-main}. First, we give a proof for \autoref{thm:aggregation-main}, now equipped with the $\RangeSumOracle$ described in \autoref{sec:oracle}.

\begin{proof} [Proof of Theorem \ref{thm:aggregation-main}]
    The aggregation algorithm follows \eqref{eq:derivation-aggregate} line-by-line and ``pushes'' the aggregation operator $\bigoplus_{x_n}$ into the inner-most parenthesis, therefore costing time $O(|\formula_n|)$ to scan over the derivation of $\formula_n(\bx_{[n]})$. Factoring out the term $\formula_n(\bx_{S_i})$, where $i = 0, \ldots, k = d(n)$ and $n \notin S_i$ is a pure syntactic step. The last step aggregates out $x_n$ from the pivot factor and gets a new positive factor $R_{U \setminus \{n\}}(\bx_{U \setminus \{n\}})$ in $O(|R_U|)$ time and space. 

    The only tricky step in \eqref{eq:derivation-aggregate} for pushing the aggregation operator $\bigoplus_{x_n}$ into the inner-most parenthesis is to efficiently compute the list representation of $R_{N_i \setminus \{n\}}(\bx_{N_i \setminus \{n\}})$, where $i = 1, \ldots, k = d(n)$, and by definition,
    \begin{align*}
        R_{N_i \setminus \{n\}}(\ba_{N_i \setminus \{n\}})  = 
        \begin{cases} \bigoplus_{x_n}  \formula_n (x_n, \ba_{N_i \setminus \{n\}})  & \text { if } \ba_{N \setminus \{n\}} \in \Pi_{N \setminus \{n\}} R_N \\ \zerobf & \text { otherwise } \end{cases}
    \end{align*}
    where $ \formula_n (x_n, \ba_{N_i \setminus \{n\}}) =  R_{N_i}({x_n, \ba_{N \setminus \{n\}}}) \oplus \indicator{\neg R_{N_i}}({x_n, \ba_{N_i \setminus \{n\}}}) \otimes \formula_n({x_n, \ba_{N^-_i \setminus \{n\}}})$. Now we apply \autoref{thm:oracle-main} to get the oracles $\Oracle_i(\bx_{N_i \setminus \{n\}})$ for each $i = 1, \ldots, k$. Then, the weight $R_{N_i \setminus \{n\}}(\ba_{N_i \setminus \{n\}})$ can be obtained in $O(\ackfunc{\db_n})$ time, for each $\ba_{N_i \setminus \{n\}} \in \Pi_{N_i \setminus \{n\}} R_{N_i}$, by calling the oracle $\Oracle_i(\bx_{N_i \setminus \{n\}})$ with inputs $\left(\ba_{N_i \setminus \{n\}}, [1, \bot] \right)$. Indeed, the oracle runs in time $O(\ackfunc{\db_n})$ and returns the range sum
    \begin{align*}
        \bigoplus_{\interval \in [1, \bot]} \formula_n \left(A_0(\Pi_{U \setminus \{n\}} \ba_{N_i \setminus \{n\}})[\interval], \; \ba_{N_i \setminus \{n\}}\right) = \bigoplus_{x_n \in \dom(x_n)} \formula_n (x_n, \ba_{N_i \setminus \{n\}}) = R_{N_i \setminus \{n\}}(\ba_{N_i \setminus \{n\}})
    \end{align*}
    Therefore, the list representation of the new factor $R_{N_i \setminus \{n\}}$ can be computed in $O(|R_{N_i}| \cdot \ackfunc{\db_n})$ time and is of size $O(|R_{N_i}|)$. The overall time complexity of the aggregation algorithm is $O(d(n) \cdot |\db_n| \cdot \ackfunc{\db_n})$ since there are $d(n)$ steps in the derivation of $\formula_n(\bx_{[n]})$ that requires the construction of a new factor $R_{N_i \setminus \{n\}}$ and each construction takes at most $O(|\db_n| \cdot \ackfunc{\db_n})$ time (to further push the aggregation operator $\bigoplus_{x_n}$ into the nested subexpression). After we aggregate out the variable $x_n$ from $\formula_n(\bx_{[n]})$, we automatically get a new $\nestfaqneg$ expression $\formula_{n-1}(\bx_{[n-1]})$. Since we keep the derivation of $\formula_n(\bx_{[n]})$ intact, we have $|\formula_{n-1}| = O(|\formula_n|)$ and $\formula_{n-1}(\bx_{[n-1]})$ is indeed a $\nestfaqneg$ expression recognized by $\CFG_{n-1}$. Moreover, as all the new factors $R_{N_i \setminus \{n\}}$ are still of size $O(|R_{N_i}|)$, we have $|\db_{n-1}| = O(|\db_n|)$.
\end{proof}



We finally prove the main theorem \autoref{thm:faqneg-main} for free-connex $\pn$-acyclic $\nestfaqneg$ queries.

% \begin{theorem}
%     Let $\varphi$ be a free-connex $\pn$-acyclic $\nestfaqneg$ query with free variables $F$ over a commutative semiring $\bS$. Then, there is an algorithm that can enumerate the answers of $\varphi$ in $O(|\varphi|)$ delay, after a $O(|\varphi|^3 + |\varphi| \cdot |\db| \cdot \ackfunc{\db})$ preprocessing time.
% \end{theorem}

\begin{proof} [Proof of \autoref{thm:faqneg-main}]
    Recall that for a $\pn$-leaf, say $n$, we run the following algorithms in order:
    \begin{enumerate}
        \item first, by \autoref{thm:rewrite}, we apply the $\Rewrite$ algorithm in time $O(|\formula|^2 + d(n) \cdot |\db|)$, where $d(n)$ is the number of hyperedges in $\mH$ that contain $n$, to transform $(\formula(\bx_{[n]}), \db)$ into a $\nestfaqneg$ expression $\formula_n(\bx_{[n]})$ recognized by $\CFG_n$ \eqref{eq:cfg_n} and a database instance $\db_n$ such that $\formula_n(\bx_{[n]}) = \formula(\bx_{[n]})$. Moreover, we have that $|\formula_n| \leq |\formula|$ and $|\db_n| \leq |\db|$. 
        \item next, we run the oracle-construction algorithm described in Appendix~\ref{sec:oracle} for $\formula_n(\bx_{[n]})$. By \autoref{thm:oracle-main}, the construction of oracles takes $O(|\formula_n| + |\db_n| \cdot \ackfunc{\db_n})$ time.
        \item finally, we apply the aggregation algorithm on $(\formula_n(\bx_{[n]}), \db_n)$ and by \autoref{thm:aggregation-main}, we obtain in $O(|\formula_n| + d(n) \cdot |\db_n| \cdot \ackfunc{\db_n})$ time the tuple $(\formula_{n-1}(\bx_{[n-1]}), \db_{n-1})$, where $\formula_{n-1}(\bx_{[n-1]})$ is a $\nestfaqneg$ expression associated with $\mH_{n-1} = \removeleaf{\mH_n}{n-1}$ and $\db_{n-1}$ is its database instance such that $\formula_{n-1}(\bx_{[n-1]}) = \bigoplus_{\bx_{[n] \setminus F} \in \dom(\bx_{[n] \setminus F})} \; \formula_n(\bx_{[n]})$. By \autoref{thm:aggregation-main}, we have that $|\formula_{n-1}| \leq |\formula_n|$ and $|\db_{n-1}| \leq |\db_n|$. Thereafter, recall that $\formula_{n-1}(\bx_{n-1})$ is recognized by the following $\CFG_{n-1}$ \eqref{eq:cfg_n-1}
        %%%%%%%%%%%%%%%%%%%%%%%% the old CFG_{n-1} %%%%%%%%%%%%%%%%%%%%%%%%
        % \begin{equation*} 
        %     \begin{aligned}
        %         \CFG_{n-1} \qquad \qquad \; \\
        %         \text{ for all } S \subseteq [n-1], \\
        %         \nonterm_{n-1}(\bx_{\emptyset}) &::= \; e  
        %         && \text{ where }  S = \emptyset \text{ and } e \in \boldsymbol{D} \setminus \{\zerobf\}   \\
        %         \nonterm_{n-1}(\bx_{S}) &::= \; R_U(\bx_U) 
        %         && \text{ where } S = U \setminus \{n\} \\
        %         & \; \; \mid \; R_K(\bx_K) \otimes \nonterm_{n-1}(\bx_{S^-}) 
        %         && \text{ where } S = K \cup S^- \text{ and } K \in \{K \in \mE^+ \mid n \notin K\}   \\
        %         & \; \; \mid \; (R_{N}(\bx_{N}) \vdash \nonterm_{n-1}(\bx_{N^-}))
        %         && \text{ where } S = N \text{ and } N^- \subseteq N \in \{N \setminus \{n\} \mid N \in \mE^-, n \in U \subset N \}  \\
        %         & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_{n-1}(\bx_{N^-})) \otimes \nonterm_{n-1}(\bx_{S^-}) 
        %         && \text{ where } S = N \cup S^- \text{ and } N^- \subseteq N \in \{N \in \mE^- \mid n \notin N\} 
        %     \end{aligned}
        % \end{equation*}
        \begin{equation} 
            \begin{aligned}
               \framebox{$\CFG_{n-1}$} \qquad \qquad \; \\
                \text{ for all } S \subseteq [n-1], \\
                    \nonterm_{n-1}(\bx_{\emptyset}) &::= \; e  
                    && \text{ where } e \in \boldsymbol{D} \setminus \{\zerobf\}  \\
                    \nonterm_{n-1}(\bx_{S}) &::= \; R_K(\bx_K) \otimes \nonterm_{n-1}(\bx_{S^-}),  
                    && \text{ where } K \in \mE^+_{n-1}, S^- \subseteq S \text{ such that } S = K \cup S^- \\
                    & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm_{n-1}(\bx_{N^-})) \otimes \nonterm_{n-1}(\bx_{S^-}), 
                    && \text{ where } N \in \mE^-_{n-1}, N^- \subseteq N, S^- \subseteq S \text{ such that } S = N \cup S^-
            \end{aligned}
        \end{equation}
    \end{enumerate}
    Thus, the $\pn$-elimination step on $n$ takes $O(|\formula|^2 + d(n) \cdot |\db| \cdot \ackfunc{\db})$ time in total. 

    Now we are ready for the next $\pn$-elimination step for $n-2$ with $\pn$-leaf $n-1$. We keep repeating the $\pn$-elimination step for $i = n-2, \dots, f$ and every intermediate $\nestfaqneg$ expression $\formula_{i}(\bx_{[i]})$ and its corresponding database instance $\db_i$ have their sizes bounded by $O(|\formula|)$ and $O(|\db|)$, respectively. In the end, we obtain a full $\nestfaqneg$ expression $\formula_f(\bx_{[f]})$ and a database instance $\db_f$ as desired, i.e.
    \begin{align*}
        \varphi(\bx_F) = \bigoplus_{\bx_{[n] \setminus F} \in \dom(\bx_{[n] \setminus F})} \; \formula(\bx_{[n]}) = \bigoplus_{\bx_{[n-1] \setminus F} \in \dom(\bx_{[n-1] \setminus F})} \; \formula_{n-1}(\bx_{[n-1]}) = \cdots = \formula_f(\bx_{[f]}).
    \end{align*}
    Therefore, the total time for the $\pn$-elimination sequence (for $i = n-1, \dots, f$) is bounded by (by definition, $|\varphi| = |\formula|$)
    \begin{align*}
        \sum_{i = f}^{n-1} O(|\formula|^2 + d(i) \cdot |\db| \cdot \ackfunc{\db}) = O(|\formula|^3 + |\formula| \cdot |\db| \cdot \ackfunc{\db}).
    \end{align*}
    From now on, we follow the enumeration algorithm for full $\nestfaqneg$ queries proposed in Appendix~\ref{sec:enum-full-faqneg} and by Appendix~\ref{cor:enum-full-faqneg}, thus we close the proof.
\end{proof}







% \begin{equation}
%     \begin{aligned}
%         \CFG: \qquad \qquad \quad \; \\
%         \text{ for all } S \subseteq [n], \\
%         \nonterm(\bx_{\emptyset}) &::= \; e 
%         && \text{ where } e \in \boldsymbol{D} \\
%         \nonterm(\bx_{S}) &::= \; R_K(\bx_K) \otimes \nonterm(\bx_{S^-})
%         && \text{ where } K \in \mE^+ \text{ and } S^- \subseteq S \text{ such that } S = K \cup S^- \\
%         & \; \; \mid \; (R_N(\bx_N) \vdash \nonterm(\bx_{N^-})) \otimes \nonterm(\bx_{S^-})
%         && \text{ where } N \in \mE^-, N^- \subseteq N \text{ and } S^- \subseteq S \text{ such that } S = N \cup S^-
%     \end{aligned}
% \end{equation}

==> border.tex <==

\section{Main results}


==> characterization.tex <==

\section{Characterizations of the condition $\mathcal{C}$}

The notions of a nest point variable and a projected atom are crucial.

\begin{definition}[Nest point variable]
Let $q$ be a signed BCQ. A variable $x$ in $q$ is a \emph{nest point variable} if all the atoms in $q$ that contain $x$ can be linearly ordered by $\subseteq$.
In particular, a variable $x$ is an \emph{isolated variable} if there is only one atom in $q$ that contains $x$.
\end{definition}

\begin{definition}[Projected atom]
Let $q$ be a signed BCQ. An atom $R(\vec{u})$ in $q$ is a \emph{projected atom} if there is another positive atom $S(\vec{w})$ in $q$ with $\vars{\vec{u}} \subseteq \vars{\vec{w}}$.
\end{definition}

We show that the removal of nest point variables or projected atoms preserves $\mathcal{C}$. 

\begin{lemma}
\label{lemma:c-nest-points}
Let $q$ be a signed BCQ. Let $x$ be a variable in $q$. Let $q'$ be the resulting query obtained by removing $x$ from every atom in $q$ that contains $x$. 
If $q$ satisfies $\mathcal{C}$, then $q'$ satisfies $\mathcal{C}$.
\end{lemma}
\begin{proof}
Let $q' = q_x^+, q_x^-$, and consider any signed BCQ $q_x^* = q_x^+, p_x^-$ where $p_x^- \subseteq q_x^-$.
It suffices to show that $q_x^*$ is $\alpha$-acyclic. 
By construction of $q'$, there exists a subquery $p^- \subseteq q^-$ such that $q_x^+$ and $p_x^-$ are obtained by removing $x$ from $q^+$ and $p^-$ respectively. 
Since $q$ satisfies $\mathcal{C}$, $q^{*} = q^+, p^-$ is $\alpha$-acyclic, and let $T$ be the join tree of $q^{*}$.
Then, consider the tree $T_x$ obtained by removing $x$ from every tree node that contains $x$ in $T$. 
We have that $T_x$ is a join tree of $q_x^*$, since it by construction contains every atom as its tree node and for every variable $u(\neq x)$ in $q_x^*$, the tree nodes containing $u$ must be connected in $T_x$ since they are connected in $T$, as desired.
\end{proof}


% We recall how isolated variables and projected atoms are relevant in $\alpha$-acyclic and $\beta$-acyclic queries. 

% \begin{proposition}
% Every $\alpha$-acyclic BCQ $q$ with no negated atom contains either an isolated variable or a projected atom.
% \end{proposition}
% \begin{proof}
% Let $T$ be a join tree of $q$ and consider the atom $R(\vec{u})$ that appears as a leaf in $T$. 
% Let $S(\vec{w})$ be the only neighbor of $R(\vec{u})$ in $T$.
% Assume that $R(\vec{u})$ contains no isolated variables. 
% Let $x \in \vars{\vec{u}}$.
% Since $x$ is not an isolated variable and $T$ is a join tree, we must have $x \in \vars{\vec{w}}$. 
% Hence $\vars{\vec{u}} \subseteq \vars{\vec{w}}$ and $R(\vec{u})$ is a projected atom, as desired.
% \end{proof}

To show that the removal of projected atoms preserves $\mathcal{C}$, we need the following property of $\alpha$-acyclicity.

\begin{lemma}
\label{lemma:alpha-contained-set}
Let $q$ be a signed BCQ.
Let $R(\vec{u})$ and $S(\vec{w})$ be two distinct positive or negated atoms with $\vars{\vec{u}} \subseteq \vars{\vec{w}}$.
Let $q' = q \setminus \{R(\vec{u})\}$. 
If $q$ is $\alpha$-acyclic, then $q'$ is $\alpha$-acyclic. 
\end{lemma}
\begin{proof}
Assume that $q$ is $\alpha$-acyclic and let $T$ be a join tree of $q$.
Let $V_R$ be the node for the atom $R$ in $T$ and let $T_1, T_2, \dots, T_k$ be the connected components of $T - V_R$, and assume that $V_R$ is adjacent to $V_{A_i}$ in $T_i$ for each $1 \leq i \leq k$.
Assume without loss of generality that $V_S$ is in $T_k$.

Consider the tree $T'$ obtained by removing $V_R$ from $T$, and connect every $V_{A_i}$ to $V_S$ for each $1 \leq i < k$. 

We argue that $T'$ is a join tree of $q'$. Consider any variable $x$ in $q'$ and let $T_x$ be the set of all tree nodes whose corresponding atoms in $q'$ contain the variable $x$.
Consider $I = \{i \mid 1 \leq i \leq k, T_i \cap T_x \neq \emptyset\}$.

If $I = \{i\}$ for some index $1 \leq i \leq k$, then $T_x$ is properly contained in $T_i$, and since $T_i$ is a join tree, $T_x$ is connected. 
Otherwise, $\card{I} \geq 2$, and in this case, $x \in \vars{A_i}$ and thus $x \in \vars{R} = \vars{\vec{u}} \subseteq \vars{\vec{w}}$. 
Therefore, $x$ is contained in any node $V_P$ on the unique path from $V_R$ to $V_S$ in $T$. Hence $T_x$ would remain connected in $T'$, as desired.
\end{proof}

We remark that Lemma~\ref{lemma:alpha-contained-set} does not necessarily require that every variable in the resulting query $q'$ is bounded. 
Lemma~\ref{lemma:alpha-contained-set} can be extended to show that the removal of projected atoms also preserves $\mathcal{C}$.

\begin{lemma}
\label{lemma:c-projected-atoms}
Let $q$ be a signed BCQ.
Let $R(\vec{u})$ be a projected atom in $q$
Let $q' = q \setminus \{R(\vec{u})\}$. 
If $q$ satisfies $\mathcal{C}$, then $q'$ satisfies $\mathcal{C}$. 
\end{lemma}

\begin{proof}
We write $q = q^+, q^-$. Assume that there is a positive atom $S(\vec{w})$ such that $\vars{\vec{u}} \subseteq \vars{\vec{w}}$. 
We consider the sign of the atom $R(\vec{u})$.
\begin{itemize}
\item Case that $\lnot R(\vec{u})$ is negated, that is, $\lnot R(\vec{u}) \in q^-$.
We show that $q'$ satisfies $\mathcal{C}$. Consider any $q^* = q^+, p^-$ where $p^- \subseteq q^- \setminus \{\lnot R(\vec{u})\} \subseteq q^-$. 
Since $q$ satisfies $\mathcal{C}$, we have $q^*$ is $\alpha$-acyclic, as desired.

\item Case that $R(\vec{u})$ is positive, that is, $R(\vec{u}) \in q^+$. Let $p^+ = q^+ \setminus \{R(\vec{u})\}$
and we have $q' = p^+, q^-$.
We show that $q'$ satisfies $\mathcal{C}$. Consider any $q^* = p^+, p^-$ where $p^- \subseteq q^-$. 
Note that $q^{**} = q^+, p^-$ is $\alpha$-acyclic since $q$ satisfies $\mathcal{C}$. 
Then $q^*$ is $\alpha$-acyclic by Lemma~\ref{lemma:alpha-contained-set}.
\end{itemize}
This completes the proof.
\end{proof}

We conclude this section with a key result.

\begin{lemma}
\label{lemma:always-proceed}
If a signed BCQ $q$ satisfies $\mathcal{C}$, then $q$ contains either a nest point variable or a projected atom. 
\end{lemma}

In fact, we can show a stronger result.

\begin{lemma}
\label{lem:two-nest-points}
Let $q$ be a signed BCQ satisfying $\mathcal{C}$ with at least two variables.
If $q$ does not contain projected atoms, then $q$ contains two nest point variables that are not contained in any atom $R(\vec{u})$ in $q$ where $\vars{\vec{u}} \subsetneq \vars{q}$.
\end{lemma}
\begin{proof}
We use induction on the sum $k$ of all arities of atoms in $q$.

\begin{description}
\item[Basis $k = 2$.] 
In this case, we have $q = R(x_1, x_2)$ or $q = R(x_1), S(x_2)$, and the lemma holds for both cases.

\item[Inductive step.]
Let $q$ be a signed BCQ query satisfying $\mathcal{C}$ and let $\vars{q} = \{x_1, x_2, \dots, x_n\}$.
Assume that $q$ does not contain projected atoms.
Let $k$ be the sum of arities of all atoms in $q$ and assume that the lemma holds for any sum of arities between $2$ and $k-1$.


\begin{itemize}
\item Case that there is an atom $R(x_1, x_2, \dots, x_n)$ in $q$. 

(i) Case that $R(x_1, x_2, \dots, x_n) \in q$. In this case, we must have $q = R(x_1, x_2, \dots, x_n)$ and $n = k$, since any atom in $q$ other than $R(x_1, x_2, \dots, x_n)$ would be a projected atom, a contradiction. The lemma thus follows.

(ii) Case that $\lnot R(x_1, x_2, \dots, x_n) \in q$. Let $q' = q \setminus \{\lnot R(x_1, x_2, \dots, x_n)\}$. We must have that $\vars{q'} = \vars{q}$, or otherwise there is some variable $x$ only appearing in the negated atom $\lnot R(x_1, x_2, \dots, x_n)$ in $q$, a contradiction to that every variable in $q$ is bounded.

Let $k' = k - n$, the sum of all atom arities in $q'$. If $2 \leq k' \leq n$, then by the inductive hypothesis, there exist two nest point variables $x$ and $y$ in $q'$ not contained in any atom $R(\vec{u})$ in $q'$ where $\vars{\vec{u}} \subsetneq \vars{q'} = \vars{q}$. The lemma then follows. If $k' = 1$, then we have 
$q = A(x_1), \lnot R(x_1, x_2, \dots, x_{n})$. Since $q$ is bounded, we must have $q = A(x_1), \lnot R(x_1)$ where $\lnot R(x_1)$ is a projected atom, a contradiction.


\item Case that there is no atom in $q$ containing $\vars{q}$. 
A variable $x$ in $q$ is an \emph{$\alpha$-variable} if there exists an atom $R(\vec{u})$ such that for any atom $S(\vec{v})$ with $x \in \vars{\vec{v}}$, $\vars{\vec{v}} \subseteq \vars{\vec{u}}$.


\begin{claim}
\label{cl:alpha-variable}
The query $q$ has an $\alpha$-variable.
\end{claim}
\begin{proof}
Since $q$ satisfies $\mathcal{C}$, $q$ is $\alpha$-acyclic. 
\end{proof}


\begin{claim}
\label{cl:alpha-to-beta}
Let $x$ be an $\alpha$-variable in $q$. Then $q$ contains a nest point variable $y$ such that there is no atom $R(\vec{u})$ in $q$ with $x, y \in \vars{\vec{u}} \subsetneq \vars{q}$.
\end{claim}
\begin{proof}
Let $R(\vec{u})$ be the atom in $q$ such that for any atom $S(\vec{v})$ in $q$ with $x \in \vars{\vec{v}}$, $\vars{\vec{v}} \subseteq \vars{\vec{u}}$.

Let $q'$ be the query obtained by removing every occurence of $x$ from $q$. Let $R(\vec{w})$ be the resulting atom in $q'$ obtained from $R(\vec{u})$.
By Lemma~\ref{lemma:c-nest-points}, $q'$ satisfies $\mathcal{C}$ and contains at least two variables. 
By the inductive hypothesis, $q'$ contains two nest point variables $y$ and $z$ such that there is no atom 
$S'(\vec{z})$ in $q'$ with $y, z \in \vars{\vec{z}} \subsetneq \vars{q}$.
Therefore, either $y \notin \vars{\vec{w}}$ or $z \notin \vars{\vec{w}}$, and assume that $y \notin \vars{\vec{w}}$. 
Hence $y$ is a nest point variable in $q$. Suppose for contradiction that there is some atom $S(\vec{v})$ such that $x, y \in \vars{v}$. Since $S(\vec{v})$ contains $x$, we have that $\vars{\vec{v}} \subseteq \vars{\vec{u}}$ and thus both $R(\vec{u})$ in $q$ and $R(\vec{w})$ in $q'$ contains $y$, but $y \notin \vars{\vec{w}}$, a contradiction. 
\end{proof}


By Claim~\ref{cl:alpha-variable}, let $x$ be an $\alpha$-variable of $q$.
Then by Claim~\ref{cl:alpha-to-beta}, there is a nest point variable $y$ such that there is no atom $R(\vec{u})$ in $q$ with $x, y \in \vars{\vec{u}} \subsetneq \vars{q}$. 
Since $y$ is a nest point variable, $y$ is also an $\alpha$-variable, and by Claim~\ref{cl:alpha-to-beta}, there is a nest point variable $z$ such that there is no atom $S(\vec{v})$ in $q$ with $y, z \in \vars{\vec{u}} \subsetneq \vars{q}$. 
Then $y$ and $z$ are two nest point variables in $q$, as desired.
\end{itemize}

\end{description} 


The proof is now complete.
\end{proof}



==> enumeration.tex <==


% \xiating{Two things to follow:
% \begin{enumerate}
% \item Extension to non-full queries: we simply skip the data structure step;
% \item Extension to general semirings (very rough example below\dots)
% \end{enumerate}
% }

% Next, consider following $\faqneg$ query $\varphi$ with aggregations. 
% \begin{align*}
% \varphi(x_1, x_2, x_3) &= \bigoplus_{x_4 \in \dom(X_4)} \bigoplus_{x_5 \in \dom(X_5)} A(x_1) \otimes B(x_2) \otimes C(x_3, x_4) \otimes D(x_4, x_5) \otimes \indicator{R(x_1, x_2, x_3, x_4) = \zerobf} \otimes \indicator{S(x_2, x_3, x_5) = \zerobf} \\
% &= \bigoplus_{x_4 \in \dom(X_4)} \formula{A(x_1) \otimes B(x_2) \otimes C(x_3, x_4) \otimes \indicator{R(x_1, x_2, x_3, x_4) = \zerobf} } \otimes \bigoplus_{x_5 \in \dom(X_5)} \formula{D(x_4, x_5) \otimes \indicator{S(x_2, x_3, x_5) = \zerobf}}
% \end{align*}
% Our goal is to construct factors $\factorleq{D}{4}$ and $\factorleq{S}{4}$ in linear time such that 
% $$\factorleq{D}{4}(x_4) \otimes \indicator{\factorleq{S}{4}(x_2, x_3) = \zerobf} = \bigoplus_{x_5 \in \dom(X_5)} \formula{D(x_4, x_5) \otimes \indicator{S(x_2, x_3, x_5) = \zerobf}}$$
% and thus we yield
% \begin{align*}
% \varphi(x_1, x_2, x_3) 
% &= \bigoplus_{x_4 \in \dom(X_4)} A(x_1) \otimes B(x_2) \otimes C(x_3, x_4)  \otimes \factorleq{D}{4}(x_4) \otimes \indicator{\factorleq{S}{4}(x_2, x_3) = \zerobf}\otimes \indicator{R(x_1, x_2, x_3, x_4) = \zerobf} \\
% &=  A(x_1)   \otimes B(x_2) \otimes \indicator{\factorleq{S}{4}(x_2, x_3) = \zerobf}    \bigoplus_{x_4 \in \dom(X_4)} \formula{C(x_3, x_4)  \otimes   \factorleq{D}{4}(x_4) \otimes \indicator{R(x_1, x_2, x_3, x_4) = \zerobf}},
% \end{align*}

% Subsequently, we want to construct factors $\factorleq{C}{3}$, $\factorleq{R}{3}$ such that 
% $$\factorleq{C}{3}(x_3) \otimes \indicator{\factorleq{R}{3}(x_1, x_2, x_3) = \zerobf} = \bigoplus_{x_4 \in \dom(X_4)} C(x_3, x_4)  \otimes \factorleq{D}{4}(x_4) \otimes \indicator{R(x_1, x_2, x_3, x_4) = \zerobf},$$
% and we yield
% \begin{align*}
% \varphi(x_1, x_2, x_3) 
% &= \bigoplus_{x_4 \in \dom(X_4)} A(x_1) \otimes B(x_2) \otimes C(x_3, x_4)  \otimes \factorleq{D}{4}(x_4) \otimes \indicator{\factorleq{S}{4}(x_2, x_3) = \zerobf}\otimes \indicator{R(x_1, x_2, x_3, x_4) = \zerobf} \\
% &=  A(x_1)   \otimes B(x_2) \otimes \factorleq{C}{3}(x_3)  \otimes \indicator{\factorleq{S}{4}(x_2, x_3) = \zerobf}  \otimes \indicator{\factorleq{R}{3}(x_1, x_2, x_3) = \zerobf}.
% \end{align*}

% Now, note that $\varphi(x_1, x_2, x_3)$ does not contain any aggregation, and we reduce to the case of computing $\psi(x_1, x_2, x_3)$ introduced at the beginning. 

==> old-pn-acyclic.tex <==
\section{$\pn$-acyclicity}
\label{sec:pn-acyclic}

In this section, we study the properties of $\pn$-acyclicity. Some results have been carefully studied in Chapter 6 of Brault-Baron's thesis~\cite{DBLP:phd/hal/BraultBaron13}.

\begin{definition}[$\pn$-leaf]
Given a signed hypergraph $\mH = (\mV, \mE^+, \mE^-)$, a vertex $x \in \mV$ is a $\pn$-leaf of $\mH$ if there exists a hyperedge $R_x \in \mE^+$ that contains $x$ such that  
\begin{itemize}
\item $R \subseteq R_x$ for every edge $R \in \mE^+$ that contains $x$; and
\item the set $\negatedN{x}{\mH} = \{N \in \mE^- \mid x \in N, N \not\subseteq R_x\} \cup \{R_x\}$ can be linearly ordered by $\subseteq$ with $R_x$ being the minimal element.
\end{itemize}
The hyperedge $R_x$ is called the \emph{pivot edge} of the $\pn$-leaf $x$ in $\mH$. 
\end{definition}
% \xiating{Note that this definition intentionally and explicitly merges the properties of $\alpha$-leaf and $\beta$-leaf together for the sake of having some $\pn$-leaf.
% However, the later expositions may be complicated.
% We could also define two independent operations: (i) remove an atom $R(\vec{u})$ if $R(\vec{u}) \subseteq S(\vec{v}) \in \positiveatoms{q}$ and (ii) remove a nest point variable $x$.
% }

% \xiating{Well, we need to generalize our algorithm for free-connex SCQs.}

It can be verified that the notion of $\pn$-leaf degenerates to an $\alpha$-leaf when $\mE^- = \emptyset$ and reduces to a $\beta$-leaf when $\mH^+$ contains only singleton hyperedges.
Recall that every $\alpha$-acyclic hypergraph has an $\alpha$-leaf and every $\beta$-acyclic hypergraph has a $\beta$-leaf. 
We show a similar result for $\pn$-acyclicity.



\begin{proposition}
\label{prop:pn-acyclic-leaf}
Every $\pn$-acyclic signed hypergraph contains a $\pn$-leaf.
\end{proposition}


Let $\mH = (\mV, \mE^+, \mE^-)$ be a $\pn$-acyclic signed hypergraph and let $x$ be a $\pn$-leaf in $\mH$. We define a procedure $\removeleaf{\mH}{x}$ as follows:

\begin{itemize}
\item $\removeleaf{\mH}{x}$: Let $R_x \in \mE^+$ be the pivot hyperedge of the $\pn$-leaf $x$ in $\mH$. 
We define $S_x = \{K \in \mE^+ \cup \mE^- \mid K \neq R_x, K \subseteq R_x\}$ and $\mH' = (\mV, \mE^+ \setminus S_x, \mE^- \setminus S_x)$ and return the hypergraph $\rmvertex{\mH'}{x}$.
\end{itemize}

\begin{proposition}
\label{prop:remove-pn-leaf-still-pn}
Let $x$ be a $\pn$-leaf of a signed hypergraph $\mH$. If $\mH$ is $\pn$-acyclic, then $\removeleaf{\mH}{x}$ is also $\pn$-acyclic.
\end{proposition}


\begin{definition}[$\pn$-elimination sequence]
Let $\mH = (\mV, \mE^+, \mE^-)$ be a $\pn$-acyclic signed hypergraph. A sequence $\sigma = (v_1, v_2, \dots, v_n)$ of all variables in $\mV$ is a $\pn$-elimination sequence of $\mH$ if there exists a sequence of hypergraphs $\{\mH_{i}\}_{0 \leq i \leq n}$ such that 
\begin{itemize}
\item $\mH_{0} = \mH$ and $\mH_{n}$ is empty; and
\item for every $i \in \{1, \dots, n\}$, $v_i$ is a $\pn$-leaf in $\mH_{i-1}$ and $\mH_{i} = \removeleaf{\mH_{i-1}}{v_i}$.
\end{itemize}
\end{definition}

\begin{proposition}
\label{prop:removal-sequence}
Let $\mH = (\mV, \mE^+, \mE^-)$ be a $\pn$-acyclic signed hypergraph. Let $R^- = \{u_1, u_2, \dots, u_k\}$ be any hyperedge in $\mE^-$. Then $\mH$ has a $\pn$-acyclic elimination sequence $v_1, v_2, \dots, v_{n-k}, u_1, u_2, \dots, u_k$.
\end{proposition}



\subsection{Proof of Proposition~\ref{prop:pn-acyclic-leaf} and~\ref{prop:remove-pn-leaf-still-pn} and~\ref{prop:removal-sequence}}

We first need some structural properties on $\pn$-acyclicity.

\begin{lemma}
\label{lemma:remove-var-or-atom}
Let $\mH = (\mV, \mE)$ be an $\alpha$-acyclic hypergraph. Then we have 
\begin{enumerate}
\item the hypergraph $\rmvertex{\mH}{x}$ is $\alpha$-acyclic for every vertex $v \in \mV$; and
\label{it:rmvertex}
\item the hypergraph $\mH' = (\mV, \mE \setminus \{R\})$ is $\alpha$-acyclic for every two distinct hyperedges $R$ and $S$in $\mH$ such that $R \subseteq S$. 
\label{it:rmatom}
\end{enumerate}
\end{lemma}
\begin{proof}
Let $\mT$ be the join tree of $\mH$ witnessed by the bijection mapping $\chi : \mE \rightarrow V(\mT)$.
Consider two items.

\framebox{(\ref{it:rmvertex})}
We have that $\rmvertex{\mH}{x} = (\mV\setminus \{x\}, \rmvertex{\mE}{x})$.
Consider the new mapping $\chi' : \rmvertex{\mE}{x} \rightarrow V(\mT)$ such that $\chi'(K \setminus \{x\}) = \chi(K)$ for every $K \in \mE$. 
It is easy to verify that for every variable $v \in \mV\setminus\{x\}$, the set of nodes $\{\chi'(K \setminus \{x\}) \mid K \setminus \{x\} \in \rmvertex{\mE}{x}\}$ induces a connected component in $\mT$ since the set of nodes $\{\chi(K) \mid K \in \mE\}$ does.


\framebox{(\ref{it:rmatom})}
Let $R$ and $S$ be two distinct hyperedges in $\mH$ such that $R \subseteq S$. 
Let $\mT_1, \mT_2, \dots, \mT_k$ be the connected components of $\mT - \chi(R)$, the tree obtained by removing the node $\chi(R)$ and all edges incident to $\chi(R)$ from $\mT$. 
Assume that $\chi(R)$ is adjacent to $\chi({A_i})$ in $\mT_i$ for each $i\in[k]$ and without loss of generality that $\chi(S)$ is contained in $\mT_k$.
Consider the tree $\mT'$ obtained by removing $\chi(R)$ from $\mT$ and adding an edge between every $\chi({A_i})$ to $\chi(S)$ for each $i\in[k-1]$. 

We argue that $\mT'$ is a join tree of $\mH'$. Consider any vertex $x$ in $\mH'$ and let $K_x = \{\chi(K) \mid x \in K, K \in \mE \setminus \{R\}\}$. The goal is to show that $K_x$ induces a connected component in $\mT'$.

Consider $I = \{i \in [k] \mid V(\mT_i) \cap K_x \neq \emptyset\}$, the indices of all subtrees $\mT_i$ that contains some hyperedge containing $x$.
If $I = \{i\}$ for some index $i \in[k]$, then $K_x$ is properly contained in $\mT_i$, and since $\mT_i$ is a join tree, $\mT_x$ induces a connected component in $\mT_i$ and thus $\mT'$. 
Otherwise, $\card{I} \geq 2$. In this case, we must have $A_i \in K_x$ for every $i \in I$ and thus $x \in R \subseteq S$.
Therefore, $K_x \setminus V(\mT_k)$ induces a connected component in $\mT'$. By construction, every $\chi(A_i)$ is connected to $\chi(S)$ in $\mT'$ and $\chi(S) \in K_x$. Note that $K_x \cap V(\mT_k)$ also induces a connected component in $\mT_k$ and $\chi(S) \in K_x \cap V(\mT_k)$, $K_x$ induces a connected component in $\mT'$.
\end{proof}

\begin{corollary}
\label{coro:remove-var-or-atom-pn}
Let $\mH = (\mV, \mE^+, \mE^-)$ be an $\pn$-acyclic signed hypergraph. Then we have 
\begin{enumerate}
\item the hypergraph $\rmvertex{\mH}{x}$ is $\pn$-acyclic; and
\label{it:rmvertex-pn}
\item let $R\in \mE^+ \cup \mE^-$ and $S \in \mE^+$ be two distinct hyperedges with $R \subseteq S$, and we have $\mH' = (\mV, \mE^+ \setminus\{R\}, \mE^- \setminus \{R\})$ is $\pn$-acyclic.
\label{it:rmatom-pn}
\end{enumerate}
\end{corollary}
\begin{proof}
We again consider two items.

\framebox{(\ref{it:rmvertex-pn})}
Let $\mE = \mE^+ \cup \mE^-$ and we have that $\rmvertex{\mH}{x} = (\mV \setminus \{x\}, \rmvertex{\mE^+}{x}, \rmvertex{\mE^-}{x})$.
Let $\mE_x' \subseteq \rmvertex{\mE^-}{x}$ and consider the hypergraph $\mH_x' = (\mV \setminus \{x\}, \rmvertex{\mE^+}{x} \cup \mE_x')$.
By construction, we must have some $\mE' \subseteq \mE^-$ such that $\mE_x' = \rmvertex{\mE^-}{x}$.
Since $\mH$ is $\pn$-acyclic, we have that the hypergraph $\mH' = (\mV, \mE^+ \cup \mE')$ is $\alpha$-acyclic.
Then $\rmvertex{\mH'}{x} = (\mV\setminus\{x\}, \rmvertex{\mE^+}{x} \cup \rmvertex{\mE'}{x}) = (\mV\setminus\{x\}, \rmvertex{\mE^+}{x} \cup \mE'_x) = \mH'_x$ is also $\alpha$-acyclic by Lemma~\ref{lemma:remove-var-or-atom}, as desired.
 
\framebox{(\ref{it:rmatom-pn})}
The claim is straightforward if $R \in \mE^-$. 
Assume that $R \in \mE^+$.
Consider any hypergraph $\mH' = (\mV, (\mE^+  \cup \mE') \setminus \{R\})$ where $\mE' \subseteq \mE^-$.
Note that the hypergraph $\mH'' =  (\mV, \mE^+  \cup \mE')$ is $\alpha$-acyclic since $\mH$ is $\pn$-acyclic. 
Since $\mH''$ is $\alpha$-acyclic, $R \subseteq S$ and $S \in \mE^+$, by Lemma~\ref{lemma:remove-var-or-atom}, $\mH'$ is $\alpha$-acyclic, as desired.
\end{proof}


\begin{proof}[Proof of Proposition~\ref{prop:remove-pn-leaf-still-pn}]
Immediate from Corollary~\ref{coro:remove-var-or-atom-pn}.
\end{proof}



Our proof for Proposition~\ref{prop:pn-acyclic-leaf} is inspired from the proof of Theorem~7 in~\cite{10.1145/2983573}.
Some additional definitions are required.
Two vertices $x$ and $y$ are non-neighbors in a signed hypergraph $\mH = (\mV, \mE^+, \mE^-)$ if there is no hyperedge $R \in \mE^+ \cup \mE^-$ such that $R \subset \mV$ and $x, y \in R$.



\begin{lemma}
\label{lemma:two-beta-leaf}
Let $\mH = (\mV, \mE^+, \mE^-)$ be a $\pn$-acyclic signed hypergraph with at least two variables. If for every hyperedge $R \in \mE^+ \cup \mE^-$, there is no other hyperedge $S \in \mE^+$ such that $R \subseteq S$, then $\mH$ contains two non-neighbor $\beta$-leaf.
\end{lemma}
\begin{proof}
We define the size of a signed hypergraph as the sum of the size of each hyperedge in it. 
We use an induction on the size $k$ of the $\pn$-acyclic signed hypergraph $\mH$, satisfying the \emph{minimal property}, i.e. for every hyperedge $R \in \mE^+ \cup \mE^-$, there is no other hyperedge $S \in \mE^+$ such that $R \subseteq S$.


\begin{description}
\item[Basis $k = 2$.] In this case, we can only have $\mH = (\{x, y\}, \{\{x\}, \{y\}\}, \emptyset)$ or $\mH = (\{x, y\}, \{\{x, y\}\}, \emptyset)$ and the claim follows.

\item[Inductive step.] Assume that the claim holds for any $\pn$-acyclic signed hypergraph with size between $2$ and $k-1$ satisfying the minimal property.
Let $\mH = (\mV, \mE^+, \mE^-)$ be a $\pn$-acyclic signed hypergraph with size $k$ satisfying the minimal property.

Assume first that there is some hyperedge $R$ in $\mH$ such that $R = \mV$.
If $R \in \mE^+$, since $q$ satisfies the minimal property, we must have $\mH = (\mV, \{R\}, \emptyset)$, and the lemma follows. 
If $R \in \mE^-$, consider $\mH' = (\mV, \mE^+, \mE^- \setminus \{R\})$. Note that $\mH'$ is also $\pn$-acyclic, and thus by the inductive hypothesis, contains two non-neighbor $\beta$-leaves $x$ and $y$. 
Then $x$ and $y$ are also non-neighbor $\beta$-leaves in $\mH$, since the hyperedge $R$ contains $x$ and $y$ and for any hyperedge $S$ in $\mH$, $S \subseteq R = \mV$.

In what follows, we assume that $\mH$ contains no hyperedge $R$ with $R = \vars{q}$ and has at least 3 variables.

\begin{claim}
\label{cl:alpha-to-pn}
If $x$ is a $\alpha$-leaf in $\mH$, then there exists a $\beta$-leaf $y$ in $\mH$ such that $x$ and $y$ are non-neighbors in $\mH$. 
\end{claim}
\begin{proof}
Assume that $x$ is an $\alpha$-leaf in $\mH$. Let $R_x \in \mE^+ \cup \mE^-$ be an hyperedge containing $x$ in $\mH$ such that for any other hyperedge $S\in\mE^+ \cup \mE^-$ containing $x$ in $q$, $S \subseteq R$.

Consider the signed hypergraph $\rmvertex{\mH}{x} = (\mV\setminus\{x\}, \rmvertex{\mE^+}{x}, \rmvertex{\mE^-}{x})$. 
Let $\mH'$ be the signed hypergraph obtained by repeated removing hyperedges $R$ from $\rmvertex{\mE^+}{x}$ and $\rmvertex{\mE^-}{x}$ if there exists another $S\in\rmvertex{\mE^+}{x}$ with $R \subseteq S$.
By Proposition~\ref{prop:remove-pn-leaf-still-pn}, $\rmvertex{\mH}{x}$ and $\mH'$ are also $\pn$-acyclic with size less than $k$. 
By the inductive hypothesis, $\mH'$ contains two non-neighbor $\beta$-leaves $y$ and $z$.
Either $y$ or $z$ is not contained in $R_x\setminus\{x\}$ and we assume that $y$ is not contained in $R_x \setminus \{x\}$.
We argue that there is no hyperedge $S$ in $\mH$ that can contain both variables $x$ and $y$. 
Indeed, if not, assume that $S$ contains both $x$ and $y$ in $\mH$. 
By definition of $R_x$, we have that $S \subseteq R_x$, and we would have $y \in R_x$, a contradiction to our choice of $y$.

Let $R_1, R_2, \dots, R_n$ be all hyperedges in $\mH'$ such that $y \in R_i$ for each $i \in [n]$ and $R_i \subseteq R_{i+1}$ for each $i \in [n-1]$.
Then $x\notin R_i$ for each $i\in[n]$, and thus $R_i \in \mE^+ \cup \mE^-$. 
Every hyperedge $K$ in $\mH$ that contains $y$ must be included in every $R_i$, since otherwise $K$ would contain $x$, a contradiction.
Hence $y$ is a $\beta$-leaf in $\mH$.
\end{proof}

Since $\mH$ is $\pn$-acyclic, $\mH$ is $\alpha$-acyclic and thus contains an $\alpha$-leaf $x$. 
By Claim~\ref{cl:alpha-to-pn}, there is a $\beta$-leaf $y$ in $\mH$. Then $y$ is also an $\alpha$-leaf in $\mH$, and by Claim~\ref{cl:alpha-to-pn} again, there is a $\beta$-leaf $z$ in $\mH$. Hence $y$ and $z$ are non-neighbor $\beta$-leaves in $\mH$, as desired.
\end{description}
This concludes the proof.
\end{proof}


\begin{lemma}
\label{lemma:two-pn-leaves}
Let $\mH$ be a $\pn$-acyclic signed hypergraph. If $\mH$ contains at least two vertices, then $\mH$ contains two non-neighbor $\pn$-leaves.
\end{lemma}
\begin{proof}
Let $\mH = (\mV, \mE^+, \mE^-)$ be a $\pn$-acyclic signed hypergraph. Let $\mH' = (\mV, \mE'_+, \mE'_-)$ be the hypergraph obtained by repeatedly removing a hyperedge $R \in \mE^+ \cup \mE^-$ from $\mH$ if there is some hyperedge $S \in \mE^+$ with $R \subseteq S$.\xiating{Need to change to two leaves.}

If $\mH'$ contains only one vertex $x$, then Proposition~\ref{prop:pn-acyclic-leaf} holds since it is only possible that $\mH' = (\{x\}, \{\{x\}\}, \emptyset)$ and $\mH = (\{x\}, \{\{x\}\}, \mE^-)$ where $\mE^- \subseteq \{\{x\}\}$. 
In either case $x$ is a $\pn$-leaf of $\mH$. 

Otherwise, $\mH'$ contains at least two vertices. By Lemma~\ref{lemma:remove-var-or-atom}, $\mH'$ is $\pn$-acyclic. Then by Lemma~\ref{lemma:two-beta-leaf}, $\mH'$ contains a $\beta$-leaf $x$. 
Let $R_1, R_2, \dots, R_n$ be all hyperedges in $\mH'$ such that $x \in R_i$ for $i\in[n]$ and $R_i\subseteq R_{i+1}$ for each $i \in [n-1]$.

We argue that $R_1 \in \mE'_+$ and for every $i \in \{2, 3, \dots, n-1\}$, $R_i \in \mE'_-$. 
Let $i$ be the smallest index such that $R_i \in \mE'_+$. 
Such an $i$ must exist, since otherwise otherwise we have $x \in \bigcup_{K \in \mE'_-} K$ but $x \notin \bigcup_{K \in \mE'_+} K$, a contradiction to $\bigcup_{K\in \mE'_-}K \subseteq \bigcup_{K \in \mE'_+}K$.
If $i > 1$, since $R_1 \subseteq R_i$, then $R_1$ would have been removed from $\mH'$, a contradiction.
Finally, if there is any $j \in \{2, 3, \dots, n-1\}$ such that $R_j \in \mE'_+$, since $R_1 \subseteq R_j$, $R_1$ would have been removed from $\mH'$, a contradiction.

We show that $x$ is a $\pn$-leaf in $\mH$. Let $R \in \mE^+$ with $x \in R$.
If $R \notin \mE'_+$, then by construction of $\mH'$ we have $R \subseteq R_1$; and if $R \in \mE'_+$ we must have $R= R_1$.
The proof is concluded by noting that $\negatedN{x}{\mH} = \{R_i \mid i \in [n]\} \cup \{R\}$, and $R$ is the minimal element in $\negatedN{x}{\mH}$ with respect to $\subseteq$.
\end{proof}


\begin{proof}[Proof of Proposition~\ref{prop:pn-acyclic-leaf}]
Let $\mH$ be a $\pn$-acyclic signed hypergraph. If $\mH$ contains only one vertex, then that vertex is a $\pn$-leaf.
Otherwise, the claim follows by Lemma~\ref{lemma:two-pn-leaves}.
\end{proof}

\begin{proof}[Proof of Proposition~\ref{prop:removal-sequence}]
Let $\mH = (\mV, \mE^+, \mE^-)$ be a $\pn$-acyclic signed hypergraph and let $R = \{u_1, u_2, \dots, u_k\}\in \mE^-$.
By Proposition~\ref{prop:pn-acyclic-leaf} and~\ref{prop:remove-pn-leaf-still-pn}, $\mH$ always has a $\pn$-acyclic elimination sequence.
The claim follows if $R =\mV$ or $\mH$ contains only one vertex.
Otherwise, we let $\mH_0 = \mH$ construct a sequence $v_1, v_2, \dots, v_{n-k}$ such that for each $i \in [n-k]$, $v_i$ is a $\pn$-leaf in $\mH_{i-1}$ such that $v_i \notin R$ and $\mH_{i} = \removeleaf{\mH_{i-1}}{v_i}$.
This is feasible because each $\mH_i$ contains at least two vertices and must contain two $\pn$-leaves by Lemma~\ref{lemma:two-pn-leaves}, and thus there must be one that does not contain $v_i$.
\end{proof}





==> related.tex <==
\section{Related work}

==> upperbound.tex <==

\section{A linear time algorithm}

Let $q$ be a signed BCQ satisfying $\mathcal{C}$. Let $\db$ be a database instance. We first present our algorithm, that involves iteratively reducing the query and the database while preserving the query answer.

\begin{enumerate}
\item[] Algorithm: $\texttt{Evaluate}(q, \db)$
\item[] Input: a signed BCQ $q$ and a database instance $\db$
\item[] Output: does $\db$ satisfies $q$
\item \textbf{while } $q$ contains at least two atoms:
\item  \hspace{1cm} \textbf{if } for some positive atom $S(\vec{w})$ in $q$, the relation $S$ is empty in $\db$:
\item  \hspace{2cm} \textbf{return } false
\item \hspace{1cm} \textbf{if } $q$ contains a nest point variable $x$:
\item \hspace{2cm} $q, \db \leftarrow \rmnest{q}{x}{\db}$
\item \hspace{1cm} \textbf{if } $q$ contains a projected atom $R(\vec{u})$:
\item \hspace{2cm} $q, \db \leftarrow \rmatom{q}{R(\vec{u})}{\db}$
\item \textbf{return whether } $\db$ satisfies $q$ 
\end{enumerate}

The procedures $\rmnest{q}{x}{\db}$ and $\rmnest{q}{R(\vec{u})}{\db}$ are introduced below.

\begin{enumerate}
\item[] Algorithm: $\rmnest{q}{x}{\db}$
\item[] Input: a signed BCQ $q$, a nest point variable $x$ and a database instance $\db$
\item[] Output: a signed BCQ $q'$ and a database instance $\db'$
\item $q' \leftarrow$ remove the variable $x$ from every atom in $q$ that contains $x$
\item let $R_1(x, \vec{v_1})$, $R_2(x, \vec{v_2})$, $\dots$, $R_n(x, \vec{v_n})$ be positive or negated atoms in $q$ with 
$\vars{\vec{v_1}} \subseteq \vars{\vec{v_2}} \subseteq \dots \subseteq \vars{\vec{v_n}}$
\item $i \leftarrow $ the largest in $\{1, 2, \dots, n\}$ such that $R_i(x, \vec{v_i})$ is a positive atom
\item \textbf{for each } $j = 1, 2, \dots, i$:
\item \hspace{1cm} \textbf{if } $R_i(x, \vec{v_i})$ is a positive atom:
\item \hspace{2cm} \dots
\item \hspace{1cm} \textbf{else } 
\item \hspace{2cm}	\dots
\item \textbf{for each } $j = i+1, i+2, \dots, n$:
\item \hspace{1cm} \textbf{if } $R_i(x, \vec{v_i})$ is a positive atom:
\item \hspace{2cm} 	\dots
\item \hspace{1cm} \textbf{else } 
\item \hspace{2cm}	\dots
\item $\db' = \formula{\db \setminus \bigcup_{1 \leq i \leq n} R_i} \cup \bigcup_{1 \leq i \leq n} R_i'$
\item \textbf{return } $q', \db'$
\end{enumerate}

\begin{enumerate}
\item[] Algorithm: $\rmatom{q}{R(\vec{u})}{\db}$
\item[] Input: a signed BCQ $q$, a projected atom $R(\vec{u})$ and a database instance $\db$
\item[] Output: a signed BCQ $q'$ and a database instance $\db'$
\item $q' \leftarrow q \setminus \{R(\vec{u})\}$
\item Let $S(\vec{w})$ be a positive atom in $q$ such that $\vars{\vec{u}} \subseteq \vars{\vec{w}}$
\item \textbf{ if } $R(\vec{u})$ is a positive atom in $q$:
\item \hspace{1cm} $S' = S \ltimes R$
\item \textbf{ else }
\item \hspace{1cm} $S' = S \setminus \formula{S \ltimes R}$
\item $\db' \leftarrow \formula{\db \setminus S} \cup S'$
\item \textbf{ return } $q', \db'$
\end{enumerate}

We compare our algorithm with the Yannakakis algorithm and the algorithm in~\cite{Baron12}.
When $q^- = \emptyset$, this alternating algorithm coincides with the Yannakakis algorithm, by processing each leaf nodes in the join tree of $q$ iteratively. 
When $q^+$ contains only the singleton atoms (or is an NCQ, as coined in~\cite{Baron12}), it is easy to see that $q$ satisfies $\mathcal{C}$ if and only if $q$ is $\beta$-acyclic, which ensures that repeated applications of $\rmatom{q}{x}{\db}$ is possible by following the \emph{nest point elimination sequence} of $q$ at each step as in~\cite{Baron12}. 


\begin{lemma}
\label{lemma:invariant-nest}
Let $q$ be a signed BCQ with a nest point variable $x$.
Let $\db$ be a database instance of size $N$ \textcolor{red}{such that the relations involved in $q^+$ are nonempty}.
Let $q'$ and $\db'$ be the output of $\rmnest{q}{x}{\db}$. 
Then $\db$ satisfies $q$ if and only if $\db'$ satisfies $q'$, and $\rmnest{q}{x}{\db}$ runs in $O(N)$.
\end{lemma}
\begin{proof}
\xiating{The second item requires the Hangdong-Paris hashing arguments in \texttt{CQneg.pdf}.
The red assumption is to avoid the following incorrect claims:
\begin{quote}
$q_0=R(x, y, z)$ is true on $\db_0 = \emptyset$ if and only if $q_1 = R(x, y)$ is true on $\db_1$ if and only if $q_n=\emptyset$ is true on $\db_n = \emptyset$ (which is a tautology).
\end{quote}
}
% \austen{The presentation logic here could also be like this: we first define the algorithm for performing $\rmnest{q}{x}{\db}$, i.e. explain how to construct $q'$ and $\db'$, and then prove the resulting $q'$ and $\db'$ satisfy the conditions.\xiating{Absolutely, and currently I am only certain about the construction of $\db'$ in Lemma~\ref{lemma:invariant-atom}, but not Lemma~\ref{lemma:invariant-nest}.}}
\end{proof}

\begin{lemma}
\label{lemma:invariant-atom}
Let $q$ be a signed BCQ with a projected atom $R(\vec{u})$.
Let $\db$ be a database instance of size $N$ such that the relations involved in $q^+$ are nonempty.
Let $q'$ and $\db'$ be the output of $\rmatom{q}{R(\vec{u})}{\db}$. 
Then $\db$ satisfies $q$ if and only if $\db'$ satisfies $q'$, and $\rmatom{q}{R(\vec{u})}{\db}$ runs in $O(N)$.
\end{lemma}
\begin{proof}
Consider two directions.

\framebox{$\Longrightarrow$}
Assume that $\db$ satisfies $q$. 
Then there is a valuation $\mu$ such that for any positive atom $P(\vec{x})$ in $q$, $\mu(\vec{x}) \in P$ and for every negated atom $\lnot N(\vec{y})$ in $q$, $\mu(\vec{y}) \notin N$. 

It remains to show that $\mu(\vec{w}) \in S'$. 
Consider two cases. If $R(\vec{u})$ is a positive atom, then we have $\mu(\vec{u}) \in R$, and thus $\mu(\vec{w}) \in S'$ by construction. If $\lnot R(\vec{u})$ is a negated atom, then we have $\mu(\vec{u}) \notin R$, and thus $\mu(\vec{w}) \in S'$ by construction. It follows that $\db'$ satisfies $q'$.

\framebox{$\Longleftarrow$}
Assume that $\db'$ satisfies $q'$. 
Then there is a valuation $\mu$ such that for any positive atom $P(\vec{x})$ in $q'$, $\mu(\vec{x}) \in P$ and for every negated atom $\lnot N(\vec{y})$ in $q'$, $\mu(\vec{y}) \notin N$. 

Since $\mu(\vec{w}) \in S'$, we have that the valuation $\mu$ satisfies the atom $R(\vec{u})$.
Therefore, we have (i) $R(\vec{u})$ is a positive atom and $\mu(\vec{u}) \in R$ or (ii) $\lnot R(\vec{u})$ is a negated atom and $\mu(\vec{u}) \notin R$. This implies that $\db$ satisfies $q$, witnessed by the valuation $\mu$.

The proof is now complete.
\end{proof}


We may now prove the upper bound of Conjecture~\ref{conj:main}.


\begin{proposition}
Let $q$ be a signed BCQ. If $q$ satisfies $\mathcal{C}$, then $\bcqneg{q}$ is in linear time.
\end{proposition}
\begin{proof}
Assume that $q$ satisfies $\mathcal{C}$. 
Let $\db$ be a database of size $N$.
If the algorithm returns at line 3, the algorithm would return the correct result. Now assume that line 2 is always true and thus the algorithm never executes line 3.
By Lemma~\ref{lemma:c-nest-points} and~\ref{lemma:c-projected-atoms}, every intermediate queries $q$ satisfies $\mathcal{C}$, and the algorithm would terminate since either line 4 or line 6 holds by Lemma~\ref{lemma:always-proceed}.
Let $\{(q_i, \db_i)\}_{0 \leq i \leq n}$ be the sequence of query $q$ and $\db$ throughout the execution of the algorithm.
Here $n$ is a fixed constant which depends only on the query $q$.
By Lemma~\ref{lemma:invariant-nest} and~\ref{lemma:invariant-atom}, $\db$ satisfies $q$ if and only if $\db_n$ satisfies $q_n$, and thus the algorithm also returns the correct result.

Our algorithm runs in linear time since it proceeds in constant number of iterations, and each iteration can be implemented in linear time.
\end{proof}



\begin{comment}
\begin{definition}[Reduction sequence]
Let $q$ be a signed BCQ. A sequence of variables $x_0, x_1, \dots, x_{n-1}$ is a \emph{reduction sequence} of $q_0 = q$ if for every $0 \leq i \leq n-1$,
\begin{enumerate}
\item $x_i$ is a nest point variable in $q_{i}$,
\item $q_{i+1} = \texttt{Reduce}(q_{i}, x_{i})$,
\end{enumerate}
and $q_n$ is $\alpha$-acyclic and contains \emph{at most one} negated atom.
\end{definition}



\begin{conjecture}
\label{conj:reduction-sequence}
% Let $q() :- R_1(\vec{x_1}), R_2(\vec{x_2}), \dots, R_n(\vec{x_n}), \lnot S_1(\vec{y_1}), \lnot S_2(\vec{y_2}), \dots, S_m(\vec{y_m})$.
% where $\bigcup_{1 \leq i \leq m} \vars{\vec{y_i}} \subseteq \bigcup_{1 \leq i \leq n} \vars{\vec{x_i}}$. 
If a BCQ with negated atoms $q$ admits a reduction sequence, then $\bcqneg{q}$ is in linear time.
\end{conjecture}

\xiating{I am not sure about the lower bounds though.}

\begin{example}
Every $\alpha$-acyclic BCQ with at most one negated atom has the empty sequence as its reduction sequence, since the base case is vacuously satisfies the base case.

Every $\beta$-acyclic NCQ\footnote{An NCQ is a BCQ with negated atoms in which all positive atoms have arity $1$.} has a nested point elimination sequence, and any such sequence is a reduction sequence since it ends up with $q_n$ being an empty query.

\end{example}



The following lemma demonstrates an iterative step.
\begin{conjecture}
\label{lemma:nest-point}
Let $q$ be a BCQ with negated atoms.
Let $\db$ be a database instance of size $N$.
Let $x$ be a nest point variable in $q$ and let $q' = \texttt{Reduce}(q, x)$.
Then there exists a database instance $\db'$ of size at most $N$ that can be constructed in $O(N)$ time such that
$\db$ satisfies $q$ if and only if $\db'$ satisfies $q'$.
\end{conjecture}


We show that Conjecture~\ref{lemma:nest-point} implies Conjecture~\ref{conj:reduction-sequence}.

\begin{proof}[Proof of Conjecture~\ref{conj:reduction-sequence}]
Assume that $q$ has a reduction sequence $x_0, x_1, \dots, x_{n-1}$. 
Let $q_0 = q$.
By Conjecture~\ref{lemma:nest-point}, for each $0 \leq i \leq n-1$, let $q_{i+1} = \texttt{Reduce}(q_i, x_i)$, and there exists a database $\db_{i+1}$ such that $\db_{i+1}$ satisfies $q_{i+1}$ if and only if $\db_{i}$ satisfies $q_i$.
It follows that $\db$ satisfies $q$ if and only if $\db_n$ satisfies $q_n$ and the size of $\db_n$ is at most the size of $\db_0$.
Deciding whether $\db_n$ satisfies $q_n$ can be solved in $O(N)$ by Corollary~\ref{coro:at-most-one-negated-atom} if $q_n$ is $\alpha$-acyclic and contains at most one negated atom.


Note that here $n$ is a fixed constant since it is at most the number of variable in $q$. Thus the database $\db$ can be constructed in $O(n \cdot N) = O(N)$ time.  Therefore, $\bcqneg{q}$ is in $O(N)$ time.
\end{proof}


\begin{proof}[Proof of Conjecture~\ref{lemma:nest-point}]
Let $x$ be a nest point variable in $q$ and let $R_1(x, \vec{x_1}), R_2(x, \vec{x_2}), \dots, R_n(x, \vec{x_n})$ be (either positive or negated) atoms in $q$.

Let $k$ be the largest such that $R_k(x, \vec{x_k})$ is a positive atom. Such an index must exist since otherwise the variable $x$ would be unbounded since it only appears in negated atoms, a contradiction. 

For each relation $R_i$ in $\db$ with arity $d+1 > 1$, we define a new relation $R_i'$ with arity $d$ as follows:
\begin{itemize}
\item for every $1 \leq i \leq k$, 
\begin{itemize}
\item if $R_i(x, \vec{x_i})$ is a positive atom, then 
$$R_i' := \{\vec{c} \in \Pi_{\vec{x_i}} R_i \mid \exists \theta: \formula{\theta(x, \vec{x_k}) \in R_k \land \theta(\vec{x_i}) = \vec{c} \land \theta(x, \vec{x_i}) \in R_i} \},$$
\item if $R_i(x, \vec{x_i})$ is a negated atom, then 
$$R_i' := \{\vec{c} \in \Pi_{\vec{x_i}} R_i \mid \forall \theta: \formula{\theta(x, \vec{x_k}) \in R_k \land \theta(\vec{x_i}) = \vec{c}} \rightarrow \formula{\theta(x, \vec{x_i}) \in R_i} \},$$
\end{itemize}
\item for every $k < i \leq n$, we have $R_i(x, \vec{x_i})$ is a negated atom,  
$$R_i' := \{\vec{c} \in \Pi_{\vec{x_i}} R_i \mid \forall \theta: \formula{\theta(x, \vec{x_k}) \in R_k \land \theta(\vec{x_i}) = \vec{c}} \rightarrow \formula{\bigvee_{k+1 \leq j \leq i} \theta(x, \vec{x_j}) \in R_j}\}.$$
\end{itemize}

Consider the database $\db'$ obtained by replacing each relation $R_i$ with $R_i'$. By construction, the size of $\db'$ is at most that of $\db$.


We show that $\db$ satisfies $q$ if and only if $\db'$ satisfies $q'$. We write $q = q^*, q_x$ and $q' = q^*, q_x'$ where 
$$q_x() :- R_1(x, \vec{x_1}), R_2(x, \vec{x_2}), \dots, R_n(x, \vec{x_n}).$$

\framebox{$\Longrightarrow$}
Assume that $\db$ satisfies $q$. Then, there is a valuation $\mu$ such that $\mu(q^*) \subseteq \db$ and $\mu(q_x) \subseteq \db$. 
Since $q^*$ does not contain the variable $x$, the relations involved in $q^*$ in $\db'$ remains the same as those $\db$, and thus $\mu(q^*) \subseteq \db'$.

\begin{itemize}
\item Let $R_i(x, \vec{x_i})$ be any positive atom with $1 \leq i \leq k$. 
We argue that $\mu(\vec{x_i}) \in R_i'$. For the valuation $\mu$, we have $\mu(x, \vec{x_k}) \in R_k$ and $\mu(x, \vec{x_i}) \in R_i$. Hence $\mu(\vec{x_i}) \in R_i'$.

\item Let $R_i(x, \vec{x_i})$ be any negative atom with $1 \leq i \leq k$. 
We argue that $\mu(\vec{x_i}) \notin R_i'$. For the valuation $\mu$, we have $\mu(x, \vec{x_k}) \in R_k$, but $\mu(x, \vec{x_i}) \notin R_i$. Hence $\mu(\vec{x_i}) \notin R_i'$.

\item Let $R_i(x, \vec{x_i})$ be any negative atom with $i > k$. 
We argue that $\mu(\vec{x_i}) \notin R_i'$. For the valuation $\mu$, we have $\mu(x, \vec{x_k}) \in R_k$, but we have 
$$\bigwedge_{k+1 \leq j \leq i} \mu(x, \vec{x_j}) \notin R_j.$$
Hence $\mu(\vec{x_i}) \notin R_i'$. 
\end{itemize}
\xiating{The arguments in this directions are very loose \dots hopefully the set constructors defined above help us merging the valuations together.}

\framebox{$\Longleftarrow$}
Assume that $\db'$ satisfies $q'$. Let $\mu$ be a valuation such that $\mu(q') \subseteq \db'$. 
We have that $\mu(q^*) \subseteq \db$. 

% Since $R_k(\vec{x_k})$ is a positive atom, there is a valuation $\theta^+$ such that 
% $\theta^{+}(x, \vec{x_k}) \in R_k$, $\theta^+(\vec{x_k}) = \mu(\vec{x_k})$ and $\theta^{+}(x, \vec{x_k}) \in R_k$.


% \begin{itemize}
% \item For every positive atom $R_i'(\vec{x_i})$ with $1 \leq i \leq k$ in $q'$, we have that $\mu(\vec{x_i}) \in R_i'$. Let $\theta_i^{+}$ be a valuation such that $\theta_i^{+}(x, \vec{x_k}) \in R_k$, $\theta_i^{+}(\vec{x_i}) = \mu(\vec{x_i})$ and $\theta_i^{+}(x, \vec{x_i}) \in R_i$.
% \item For every negated atom $\lnot R_i'(\vec{x_i})$ with $1 \leq i \leq k$ in $q'$, we have that $\mu(\vec{x_i}) \notin R_i'$. Let $\theta_i^{-}$ be a valuation such that $\theta_i^{-}(x, \vec{x_k}) \in R_k$, $\theta_i^{-}(\vec{x_i}) = \mu(\vec{x_i})$ and $\theta_i^{-}(x, \vec{x_i}) \notin R_i$.
% \item For every negated atom $\lnot R_i'(\vec{x_i})$ with $i > k$ in $q'$, we have that $\mu(\vec{x_i}) \notin R_i'$. Let $\theta_i^{-,\geq}$ be a valuation such that $\theta_i^{-,\geq}(x, \vec{x_k}) \in R_k$, $\theta_i^{-,\geq}(\vec{x_i}) = \mu(\vec{x_i})$ and $\theta_i^{-,\geq}(x, \vec{x_j}) \notin R_j$ for any $k+1 \leq j \leq i$.
% \end{itemize}

% Consider the valuation $\xi$ defined as 
% $$
% \xi(z) = 
% \begin{cases}
% \mu(z) & \text{ if } z \in \vars{q^*} \\
% \theta_i^{+}(z) & \text{ if } z \in \vars{\vec{x_i}}, i \leq k, R_i \text{ is positive} \\
% \theta_i^{-}(z) & \text{ if } z \in \vars{\vec{x_i}}, i \leq k, R_i \text{ is negated} \\
% \theta_i^{-,\geq}(z) & \text{ if } z \in \vec{\vars{x_i}}, i > k, R_i \text{ is negated}
% \end{cases}
% $$

% We first argue that the valuation $\xi$ is well defined. Assume that 

% Lastly, observe that $\xi(q^*) = \mu(q^*) \in \db$, and for each positive atom $R_i(x, \vec{x_i})$, we have 
% $$\mu$$

\xiating{Merging the valuations together\dots}


\medskip
Finally, we show that each relation $R_i'$ can be computed in linear time \xiating{using the Hangdong-Paris hashing arguments\dots}
\end{proof}

\end{comment}




